Precision phenomenology of the PDF-BSM interplay

The Standard Model (SM) is one of the most successful theories ever conceived, representing a triumph of human intellect and collaboration. The SM provides a very good description of visible matter, with the proton being a central part of this understanding. The structure of the proton can be parametrised in terms of parton distribution functions (PDFs), essential inputs for theoretical predictions at the Large Hadron Collider (LHC) which cannot be computed from first principles and must be obtained from fits to experimental data. Despite the remarkable success of the SM, many fundamental questions remain unanswered, motivating the search for physics beyond the Standard Model (BSM). These searches often rely on precise comparisons between theoretical predictions and experimental measurements. However, a significant challenge arises because PDFs are typically determined under SM assumptions. This approach can introduce potential biases and inconsistencies in BSM searches. Additionally, signals of BSM physics may be absorbed by the PDFs during the fitting procedure, further complicating the interpretation of the results. This PhD thesis explores the interplay between PDFs and BSM physics. We introduce the open-source release of SIMUnet, a deep learning framework designed to perform simultaneous fits of PDFs and BSM parameters, as well as to assess the potential absorption of BSM signals by the PDFs. We study the PDF-BSM interplay in the top sector and in a global dataset, and assess the absorption of BSM physics in widely used models. Additionally, we explore how BSM effects can alter the evolution of PDFs, and demonstrate the potential of interpretable machine learning techniques in symbolic regression for collider physics in general.

==> Chapters/Contamination/files_to_delete/_region_.tex <==
\message{ !name(sec-intro.tex)}
\message{ !name(sec-intro.tex) !offset(-2) }
\section{Introduction}

Two crucial questions are still unanswered and should be addressed at the LHC. First, how can one assess whether new physics effects are inadvertently absorbed into the flexible parametrisation of the non-perturbative proton structure, as the high-energy tails of the distributions are used to determine the PDFs of the proton? And second, how are the bounds on the SMEFT coefficients modified if the PDFs used as input to determine such bounds had been fitted using a consistent BSM framework? Despite a lot of concentrated effort from a wide community in both PDF and SMEFT fields separately, and despite a recent indication of their significant interplay.

The inconsistencies between data which enter a global PDF determination can distort the statistical interpretation of PDF uncertainties. In particular, the inconsistency of any individual dataset with the bulk of the global fit may suggest that its understanding, either from the theoretical or experimental point of view, is not complete. First, we will extend the statistical definition of inconsistency given in [22], by accounting also for theory uncertainties and model uncertainties.

% From Mangano's email

% \begin{itemize}
%   \item You mention one very briefly at the end of the paper, namely the measurement of fwd W and Z production in LHCb. I think it’s useful to elaborate on this further: Forward DY production will mostly be driven by q qbar (fwd being in the direction of the q. In the following I assume that the first parton comes from the “left”, the second parton comes from the “right”, where the LHCb detector is located). qbar q will be much suppressed. At large x, q is rather well known already. So the mass spectrum alone will not be very powerful in probing qbar. What could help more is the charge-dependent lepton spectrum in W production. For example, in u dbar -> e+ nu, the EW spin correlation will send the neutrino forward, and the positron will stay at smaller eta. Looking at positrons in the most forward eta region, will therefore strongly enhance the dbar u initial state, and hopefully help improving the dbar knowledge at large x. For the ubar it is slightly more complicated, since here it’s the antineutrino that goes fwd, the electron is produced more centrally, and the two eta solutions for the nubar compete with each other. (as an aside: as you know there are now two neutrino detectors approved for the LHC, FASERnu and SND. They do have some acceptance for neutrinos from W decays, especially SND. I wonder whether a possible measurement of an antineutrino -- the detectors have magnets, so can tell the charge of the lepton from the CC neutrino interaction -- can say something about large-x ubar…) \LM{I do not completely understand the idea here... I guess we would like to probe more the qbar component of the proton, but aren't these observables already included in the NNPDF fit? Also I think there is possible confusion in the text because he mentions that positrons are central as opposed to electrons, but then he says that also electrons are central.}
% \item Another useful handle is the angular distribution of the large mass dileptons. In the highest mass bins there won’t be much statistics, but the impact of EFTs starts building up earlier, and there could be a sweet-spot in mll where the distortions induced on the angular spectrum could start being visible. More in general, the leptonic angular distributions (in the W or DY rest frame, to reduce PDF dependence) should be a good SM monitor.
% \item The best SM control sample, in my view, would be high statistics data at 7 or 8 TeV. This goes along the lines of Ref.~\cite{Mangano:2012mh}  If at 13 or 14 TeV you see the DY spectrum deviate from the SM at, say, mll=3 TeV, then one could check the spectrum in 7 or 8 TeV data at mll~1.5 TeV. This probes the PDFs in the same range of x. I believe the extrapolation to mll=3 TeV at 14 TeV would have a very small systematics, smaller than anything else in the game. Notice that, since we’re doing a shape comparison, the luminositty uncertainties (which at the two energies are not correlated) will be irrelevant. Of course we do not have good statistics at 7 or 8 TeV. However, if a discrepancy is found in the future at 13-14 TeV, we shall need to answer the question: what is the most robust way to find out whether it’s BSM or systematics? If it turned out that the best way is to use one year of HL-LHC running to get 100fb-1 of 7 TeV data, that’s an interesting observation to make. So I think it’s worth keeping this opportunity in mind when doing a phenomenological study like yours.
% \item You have all the tools available to explore the ideas above in great detail, I believe it would be a very useful investment on your side to do at least a preliminary investigation. Even a LO study would be helpful, it could suggest that none of the above is really useful, and then you don’t waste much time. If you see some hope, then you may decide to move to a full-fledged study.
% \end{itemize}
The idea is to do everything with MC pseudo-data and
\begin{enumerate}
\item Generate MC pseudo-data of observables that are typically included in a PDF fit with SM theory, do a PDF fit of these pseudodata and create our baseline PDF set
\item Generate MC pseudo-data with some BSM theory injected in the data (something that affects the high-energy data that are usually included in PDF fits) and do a PDF fit of these "contaminated" pseudo-data using SM theory
\item Generate a conservative version of the PDF set above, that excludes the contaminated data.
\item How can we disentangle EFT manifestations of new physics effects from PDF effects? In the PDF set generated in (2) have we absorbed new physics? To answer these questions the idea is that we look at an observable in which we should see signs of the new physics that we are assuming exists in Nature. If we use the PDF set (2) that was obtained from contaminated pseudo-data and we do not "see" new physics it means that PDFs have absorbed new physics. What if we use the PDF set (3)? This should disentangle EFT manifestations of new physics and PDF effects.
 \end{enumerate}

\noindent Plan:
\begin{itemize}
\item We must identify a number of interesting new physics scenarios, that have to do with the data included in a PDF fit. A tentative list is given in Section 2.
\item We must generate MC pseudo-data for all observables we include in our PDF fits (plus some extra interesting ones). The uncertainty should be the one of current data but the central values are the ones we get from the MC.
\item We must identify test observables that allow us to assess whether we can disentangle the effects
\end{itemize}


\subsection{Detailed plan proposal (LM and MM)}

\begin{enumerate}
\item Select a PDF set and a UV completion of the SM. These will be "God-given" and represent the laws of physics that we want
to extract.
    \begin{itemize}
    \item We are free to choose a PDF set that we want in principle, it just represents a functional description of the proton
    structure that we assume to be the real one.
    \item Regarding the UV completion, we need a model with a scale of NP considerably higher than the energy scales probed by the data.
    This way we expect just a perturbation in the tails of the distributions and we can also match the UV description to a SMEFT
    parametrisation.
    \item From the SMEFT perspective, we should study the validity of the EFT, finding the region in the Wilson coefficient parameter
    space that provides a good description of the UV effects at linear level in the EFT power expansion.
    \item A simple option could be a UV completion that generates the $W$ and $Y$ parameters, this way we could take advantage of previous studies  and previously implemented calculations, although it might be too narrow and not affect observables like jets ot top observables.
    \end{itemize}
\item Produce the pseudo-data with new-physics contamination.
    \begin{itemize}
    \item Ideally we would do so in the SMEFT, having previously established the region of validity. This would give us more
    flexibility if we want to vary the coefficients without having to regenerate all the data from scratch.
    \item Once we decide the subset of the NNPDF 4.0 dataset~\cite{Ball:2021leu} that we want to include, we need to generate pseudo-data
    for all the observables. One simple way to proceed could be to exploit the predictions in NNPDF, using the K-factors
    approximation. This way we could take advantage of the already implemented SMEFT predictions in DIS and DY, while we might have to
    compute predictions for top-quark observables. If something is missing we can compute it with madgraph, making sure that we
    are consistent with the theoretical settings (same PDF and same input parameters).
    \item If some observables are not expected to be modified by NP effects, we can avoid to compute the corrections but we need to
    make sure that that is the case, checking with madgraph that the corrections are indeed negligible for the region of Wilson
    coefficients that we consider. We will however compute the pseudo-data for that with NNPDF (or madgraph if not implemented), in order to be consistent across the board.
    \item The prediction generated will be used to determine the central value of the pseudo data, while we will associate to those numbers the experimental uncertainties (already implemented in NNPDF).
    \end{itemize}
\item Extrapolate SM PDFs from the pseudo-data: we perform a fit assuming the SM. Can we fit away the NP effects? How do we check that?
    \begin{itemize}
    \item If the $\chi^2$ is reasonable and it suggests that the NP effects have been absorbed, can we prove that by doing a
    fixed PDF fit of the Wilson coefficients on new data we end up having bounds without a clear pull towards NP? Can we even end up excluding the NP scenario that was actually used to generate the pseudo-data?
    \item If we are in the aforementioned case, can we add observables to the fit that would probe the PDF but not NP, and this would disentangle the effects? (For example, introducing in the PDF fit observables that probe high-x but not high energy, as suggested by MLM)
    \item If instead we are in the scenario in which NP is not fitted away, can we understand why that happened? Was the
    pollution from NP too strong and the PDFs could not accommodate it? Is there data with a heavy weight in the fit that being not polluted
    is helping us to disentangle the PDFs and the NP effects?
    \end{itemize}

\item We can use the PDFs extracted from the pseudo-data fit to perform SMEFT fits on other observables (pseudo-data) which do not
      enter in the fit but are affected by NP.
      \begin{itemize}
      \item For example, in the scenario of $Z'$ which affects $DY$, we could fit pseudo-data polluted with NP effects including also data of
            top and DIS. Then we could perform a fixed PDF fit for other observables such as $ZH$, $ttZ$ and diboson, which are
            all affected by the $Z'$.
      \item We might see that we do not find NP in these observables or maybe we do but we find a shift in the measured coupling
      due to the absorbed NP in the PDFs.
      \end{itemize}
\end{enumerate}

\subsection{First shot}

MU's proposal. With current data expect mild effects. Including HL-LHC expect big effect.
\begin{itemize}
\item Take contaminated PDFs with Y=-0.0004 or Y=0.0003.
\item Test 1: Use these PDFs to make a fit of Y coefficient using DY data.  Do we get an interval that includes the true value?
\item Test 2: Generate LHCb on-shell rapidity distribution for W and Z with God-given theory (baseline PDF set and Y=whatever). Perform predictions using contaminated PDFs. Do we get wrong prediction compared to God-given one? 
\end{itemize}

\message{ !name(sec-intro.tex) !offset(-92) }


==> Chapters/Contamination/sec-intro.tex <==
\section{Introduction}
\label{sec:intro}

The LHC data places significant constraints on the PDFs, with Drell-Yan high-mass distributions providing a strong handle on the 
light quark and antiquark distributions in the medium and large-$x$ regions~\cite{Jing:2023isu}, and the high-$E_T$ jet and top data constraining 
the gluon in the large-$x$ region~\cite{Nocera:2017zge}. Despite the wealth of constraints coming from LHC data, the large-$x$ 
region still displays the largest PDF uncertainty, thus limiting the discovery potential for BSM signatures 
in the multi-TeV mass region. 
It is therefore paramount to devise and include new observables that can give us a robust understanding of PDFs and their uncertainties 
at large-$x$, such as, for example, the Drell-Yan forward-backward asymmetry~\cite{Accomando:2019vqt,Fiaschi:2021okg,Fiaschi:2022wgl,Ball:2022qtp,Fu:2023rrs}.  

In this chapter, we assess the potential contamination of PDFs by new physics in the large-$x$ region, by means of a contamination procedure that can be obtained via the \simunet{} methodology applied to Drell-Yan and DIS data. In this study, after identifying two showcase scenarios in which  
contamination might happen, we explore two natural follow-up
questions. First, if we were using a ``contaminated'' PDF set, would we miss
other signals of new physics that Nature would exhibit in other observables
(typically not included in a PDF fit)?
Second, are there suitable observables that constrain the large-$x$ region but
are unaffected by new physics, which would uncover the inconsistency of the
tails of the distributions that we include in a PDF fit? These datasets
would help us preventing the contamination of the PDFs from occurring. 
Alternatively, we could ask whether a targeted analysis of the data included in a 
PDF fit would help detecting an inconsistency due to the presence of new physics and distinguish it from 
an inconsistency that has a different source.  

The structure of this chapter is as follows. 
In Sect.~\ref{sec:scenarios} we present two UV scenarios and their low-energy 
SMEFT parametrisation, determining  the region of the EFT validity in each of the scenarios that we consider. 
In Sect.~\ref{sec:dy} we present the main results of this chapter. We show that in one of the two scenarios that we consider, namely in 
a flavour-universal $W'$ model, contamination does happen, and we identify the phenomenological consequences of the contamination. 
Finally in Sect.~\ref{sec:solution} we explore several ways to disentangle contamination. 
We summarise our results and highlight how users can utilise the tools developed here to 
explore other BSM scenarios in Sect.~\ref{sec:summary}.
Technical details of the analysis are collected in the appendices. App.~\ref{app:fit} contains the details about the 
quality of the various fits presented in this analysis, App.~\ref{app:pdfs} shows the effect of new physics contamination on 
individual partons, while App.~\ref{app:random} explores the dependence of the 
results on the random fluctuation of the Monte Carlo data that we produce in this analysis, proving the stability and robustness of the results.


==> Chapters/Contamination/sec-summary.tex <==
\section{Conclusion}
\label{sec:summary}

In this chapter we have analysed two concrete new physics scenarios
that would distort the high energy Drell-Yan invariant mass distributions that
enter PDF fits. We considered scenarios of flavour universal NP, manifested in the form of a heavy 
$Z^\prime$ and $W^\prime$ coupled to both quarks and leptons. For simplicity, we parametrised the modified interactions
by means of an EFT, where the corresponding Wilson coefficients are denoted $\hat{Y}$ and $\hat{W}$ respectively.
By generating pseudodata in different benchmark scenarios, we assessed the ability of the PDF fitting framework to
absorb the modified interactions in the PDF parametrisation, effectively hiding NP inside the modelling of the proton.
For this exploratory study we chose values of the Wilson coefficients that are not strongly disfavoured from global EFT fits.
In terms of data, we considered the state-of-the-art {\tt NNPDF4.0} dataset and its extension with
future HL-LHC projections. 

The first important conclusion from our study is that current Drell-Yan data is
not precise enough to lead to a contaminated PDF set. The uncertainties on the Drell-Yan tails of the distribution
are big enough to render the NP effects sub-leading corrections with respect to the PDF uncertainty.
On the other had, when HL-LHC projections are included, we see that more interesting effects occur.
In particular, while the heavy $Z'$ scenario does not 
lead to any contamination, a flexible enough PDF parametrisation would be able to fit away signs of a heavy $W'$ boson when performing a global PDF determination and thus
introduce spurious contamination in the large-$x$ structure of the proton. 

In particular, this has been assessed by 
looking at possible contamination in both the neutral and charged currents,
finding that it is when both charged current and neutral current observables are effected by NP
that we have the highest freedom
of parametrisation. This is ultimately traced back to the lack of data constraining the large-$x$
antiquark PDFs, in particular the $\bar{d}$ PDF. For this reason, we observe that, when
data are contaminated with the presence of a $W^\prime$, we generally find good fits and are able to accommodate
even large deviations from the SM. It is however worth noting that
the leading source of contaminated data are the high-statistics data expected from the HL-LHC, as present data would not be as susceptible to the $W^\prime$ effects.

One could argue that, for a safe use of  PDFs in the context of searches for new physics, 
datasets possibly susceptible to contamination from new physics should be systematically left out of PDF fits. 
But this would be naive: if a deviation from a SM projection based on available PDF fits were found in the large-$x$ tails of some distribution, 
the first systematics to double check would be the robustness of the PDF parametrisation in the region of the anomaly. 
This should be assessed by means such as those presented in this work, namely checking whether the deviation can be washed 
away by modifying the PDFs in a way that does not significantly impact the overall quality of the global fit. 
If it can, the deviation should be attributed to the PDF systematics, rather than to new physics. 

We discussed possible consequences of having a contaminated PDF set, finding that such NP contamination would have consequences
in the interpretation of the LHC data. On the one hand, by computing predictions with the aforementioned set of PDFs, one would likely hinder searches for new physics
affected by the presence of the $W^\prime$, leading to biased exclusion bounds. On the other hand, one would also potentially see deviations
from the SM predictions in processes not affected by the presence of the heavy state, purely as a consequence of the spurious
behaviour of the PDFs at large-$x$.

We discussed possible strategies to disentangle the NP effects from the PDF determination. In particular, we verified that a post-fit sliding invariant mass cut on the data entering the $\chi^2$ calculation would not highlight any trend, indicating that the PDF set describes the high invariant mass data-points across the dataset well. We also checked whether the contaminated PDF set could be flagged by HL-LHC projections of on-shell forward $Z/W$ production, an observable that would 
probe high-$x$ but not high-$Q$. However, as previously mentioned, the contamination seems to be related more to the flexibility in the antiquark PDF flavours, which in the case of forward EW boson production are mostly probed in the low-$x$ regime.

However, a more effective strategy of disentangling PDFs and NP is given by the study of the ratio of differential cross sections. By exploiting the fact that different processes might be dependent on the same parton luminosity channels, one could devise observables that remove the dependence on the PDF set by taking ratios of cross sections in similar kinematical regions. In the case of $W^\prime$ contamination, a promising test would be to take for instance the ratio of neutral/charged current Drell-Yan against neutral/charged diboson production.  We found that this test could in principle ascertain the presence of NP independently of the PDF set, with the ultimate caveat that the source of the deviation could either be affecting the numerator, the denominator or both.

Finally, we discussed the potential for low-energy observables to provide complementary constraints on the large-$x$ sea quarks. Such low-energy observables would not be as susceptible to the effects of new physics, and could therefore show a tension with the NP-affected high-energy data.  We found that, although the PDF fit 
includes low-energy observables that exhibit a large correlation with the large-$x$ $\bar{d}$ and $\bar{u}$ PDFs, the precision offered by these measurements is not sufficient to create a tension with the high-energy data. Future precision measurements of the large-$x$ sea quarks, for example the EIC programme, will provide important inputs in PDF fits to avoid the contamination studied here.

To conclude, in this work we tackled the problem of inconsistent data in PDF determination.
Although it is well known that inconsistencies between experimental data entering
a global PDF determination can distort the statistical interpretation of
PDF uncertainties and although there are mechanisms to select
a sufficiently consistent bulk of data to use as an input of a global PDF analysis,
the inconsistency of any individual dataset with the bulk of the global fit may suggest that its understanding, 
either from the theoretical or experimental point of view, is not complete. How can we establish whether the inconsistency 
comes from missing higher order uncertainties, data inconsistencies or unaccounted new physics effects?
In this work we tackled the latter, trying to take advantage of the fact that NP contamination has a different 
energy-scaling behaviour compared to effects that might arise from missing higher orders or from experimental inconsistencies. 
We tackled it by setting up a set of tools and analyses built on statistical closure tests in a specific and simple 
test-case scenario. 

We have provided a concrete example of the issues that can emerge from possible new physics effects 
in the data used in a fit of PDFs, and how to possibly address those issues, when trying to expose new physics from 
departures of SM predictions in the tails of kinematical distributions at large energy. 


==> Chapters/Contamination/tables/tab_chi2_hllhc.tex <==
\begin{table}[t!]
        \small
        \centering
        \begin{tabular}{l|c|c|c|c|c|}
                \toprule
       & \multicolumn{2}{c}{HL-LHC} & \multicolumn{2}{c}{Stat. improved}\\
          \midrule
       Dataset  & $\chi^2/n_{\rm dat}$ &  $n_\sigma$ & $\chi^2/n_{\rm dat}$ & $n_\sigma$ \\
          \midrule
 $W^+ H$         & 1.17 & 0.41 & 1.77 & 1.97 \\
 $W^- H$         & 1.08 & 0.19 & 1.08 & 0.19 \\
 $W^+ Z$         & 1.08 & 0.19 & 1.49 & 1.20\\
 $W^- Z$         & 0.99 & -0.03 & 1.02 & 0.05\\
 $Z H$           & 1.19 & 0.44 & 1.67 & 1.58\\
 $W^+ W^-$       & 2.19 & 3.04 & 2.69 & 4.31\\
 VBF $\to$ H        & 0.70 & -0.74 & 0.62 & -0.90\\
                \bottomrule
        \end{tabular}
        \caption{Values of the \(\chi^2\) and $n_\sigma$ for the projected observables at HL-LHC in the EW sector. In the left column we report the values from a realistic estimate of the statistical uncertainties, while in the right columns we show what would be obtained if statistics were to improve by a factor $10$. \label{tab:chi2_hllhc}}
\end{table}


==> Chapters/Contamination/tables/tab_chi2_w.tex <==
\begin{table}[t]
        \tiny
        \centering
\begin{tabular}{lrrrrrrrr}
\toprule
 & \multicolumn{2}{r}{baseline} & \multicolumn{2}{r}{W=3e-5} & \multicolumn{2}{r}{W=8e-5} & \multicolumn{2}{r}{W=15e-5} \\
 & $\chi^2$ & $n_\sigma$ & $\chi^2$ & $n_\sigma$ & $\chi^2$ & $n_\sigma$ & $\chi^2$ & $n_\sigma$ \\
\midrule
NMC $d/p$ & 1.02 & 0.14 & 1.01 & 0.04 & 1.04 & 0.31 & 1.05 & 0.42 \\
NMC $p$ & 1.03 & 0.26 & 1.03 & 0.27 & 1.02 & 0.22 & 1.03 & 0.28 \\
SLAC $p$ & 1.02 & 0.06 & 1.02 & 0.07 & 1.01 & 0.03 & 1.02 & 0.06 \\
SLAC $d$ & 1.00 & -0.01 & 0.98 & -0.07 & 0.99 & -0.05 & 1.00 & 0.02 \\
BCDMS $p$ & 1.02 & 0.20 & 1.01 & 0.07 & 1.02 & 0.24 & 1.01 & 0.11 \\
BCDMS $d$ & 1.01 & 0.07 & 1.00 & 0.01 & 1.01 & 0.10 & 1.00 & 0.02 \\
CHORUS $\sigma_{CC}^{\nu}$ & 1.00 & 0.02 & 1.00 & -0.07 & 1.00 & 0.06 & 1.00 & 0.04 \\
CHORUS $\sigma_{CC}^{\bar{\nu}}$ & 0.99 & -0.13 & 0.99 & -0.13 & 1.00 & -0.00 & 1.00 & -0.02 \\
NuTeV $\sigma_{c}^{\nu}$ & 0.99 & -0.06 & 0.99 & -0.05 & 1.01 & 0.05 & 1.00 & 0.01 \\
NuTeV $\sigma_{c}^{\bar{\nu}}$ & 0.96 & -0.19 & 1.02 & 0.09 & 1.06 & 0.27 & 1.47 & 2.03 \\
HERA I+II inclusive NC $e^-p$ & 1.00 & -0.02 & 1.01 & 0.13 & 1.00 & 0.03 & 1.02 & 0.19 \\
HERA I+II inclusive NC $e^+p$ 460 GeV & 1.01 & 0.08 & 1.01 & 0.12 & 1.01 & 0.12 & 1.02 & 0.20 \\
HERA I+II inclusive NC $e^+p$ 575 GeV & 0.98 & -0.21 & 1.00 & 0.01 & 0.98 & -0.18 & 1.01 & 0.10 \\
HERA I+II inclusive NC $e^+p$ 820 GeV & 1.00 & -0.00 & 1.01 & 0.07 & 1.00 & -0.02 & 1.02 & 0.10 \\
HERA I+II inclusive NC $e^+p$ 920 GeV & 1.02 & 0.29 & 1.06 & 0.76 & 1.04 & 0.54 & 1.09 & 1.23 \\
HERA I+II inclusive CC $e^-p$ & 0.99 & -0.05 & 1.03 & 0.13 & 1.00 & -0.00 & 1.03 & 0.15 \\
HERA I+II inclusive CC $e^+p$ & 1.02 & 0.08 & 1.02 & 0.08 & 1.04 & 0.19 & 1.10 & 0.45 \\
HERA comb. $\sigma_{c\bar c}^{\rm red}$ & 1.00 & 0.02 & 1.02 & 0.08 & 1.01 & 0.02 & 1.01 & 0.04 \\
HERA comb. $\sigma_{b\bar b}^{\rm red}$ & 1.12 & 0.43 & 1.13 & 0.45 & 1.13 & 0.48 & 1.13 & 0.47 \\
DYE 866 $\sigma^d_{\rm DY}/\sigma^p_{\rm DY}$ & 1.14 & 0.40 & 1.07 & 0.20 & 1.40 & 1.11 & 1.72 & 1.98 \\
DY E886 $\sigma^p_{\rm DY}$ & 1.02 & 0.14 & 1.02 & 0.16 & 1.13 & 0.87 & 1.48 & 3.20 \\
DY E605 $\sigma^p_{\rm DY}$ & 1.08 & 0.53 & 1.07 & 0.44 & 1.07 & 0.47 & 1.08 & 0.50 \\
DYE 906 $\sigma^d_{\rm DY}/\sigma^p_{\rm DY}$ & 1.80 & 1.39 & 1.44 & 0.77 & 1.96 & 1.66 & 2.20 & 2.08 \\
CDF $Z$ rapidity (new) & 1.06 & 0.21 & 1.03 & 0.12 & 1.06 & 0.22 & 1.02 & 0.07 \\
D0 $Z$ rapidity & 1.03 & 0.10 & 1.02 & 0.07 & 1.04 & 0.16 & 1.02 & 0.07 \\
D0 $W\to \mu\nu$ asymmetry & 1.23 & 0.50 & 1.16 & 0.33 & 1.24 & 0.50 & 1.82 & 1.73 \\
ATLAS $W,Z$ 7 TeV 2010 & 1.05 & 0.20 & 1.04 & 0.17 & 1.06 & 0.22 & 1.05 & 0.18 \\
ATLAS HM DY 7 TeV & 1.02 & 0.04 & 1.05 & 0.12 & 1.01 & 0.04 & 1.03 & 0.06 \\
ATLAS low-mass DY 2011 & 0.90 & -0.17 & 1.04 & 0.07 & 0.87 & -0.23 & 0.99 & -0.02 \\
ATLAS $W,Z$ 7 TeV 2011 Central selection & 1.06 & 0.28 & 1.07 & 0.35 & 1.06 & 0.28 & 1.08 & 0.37 \\
ATLAS $W,Z$ 7 TeV 2011 Forward selection & 0.91 & -0.25 & 1.33 & 0.90 & 0.90 & -0.29 & 1.31 & 0.84 \\
ATLAS DY 2D 8 TeV high mass & 1.02 & 0.11 & 1.03 & 0.14 & 1.02 & 0.10 & 1.04 & 0.20 \\
ATLAS DY 2D 8 TeV low mass & 1.03 & 0.16 & 1.00 & 0.00 & 1.03 & 0.16 & 0.99 & -0.04 \\
ATLAS $W,Z$ inclusive 13 TeV & 1.07 & 0.09 & 1.07 & 0.09 & 1.09 & 0.11 & 1.08 & 0.10 \\
ATLAS $W^+$+jet 8 TeV & 1.17 & 0.46 & 0.96 & -0.10 & 1.17 & 0.48 & 0.96 & -0.12 \\
ATLAS $W^-$+jet 8 TeV & 1.19 & 0.51 & 0.97 & -0.10 & 1.21 & 0.58 & 0.98 & -0.06 \\
ATLAS $Z$ $p_T$ 8 TeV $(p_T^{ll},M_{ll})$ & 1.01 & 0.03 & 0.98 & -0.07 & 1.01 & 0.03 & 0.99 & -0.05 \\
ATLAS $Z$ $p_T$ 8 TeV $(p_T^{ll},y_{ll})$ & 0.98 & -0.10 & 0.94 & -0.29 & 0.99 & -0.06 & 0.96 & -0.21 \\
ATLAS $\sigma_{tt}^{\rm tot}$ & 1.03 & 0.02 & 1.14 & 0.10 & 1.04 & 0.03 & 1.17 & 0.12 \\
ATLAS $\sigma_{tt}^{\rm tot}$ 8 TeV & 1.31 & 0.22 & 1.12 & 0.09 & 1.30 & 0.21 & 1.13 & 0.09 \\
ATLAS $\sigma_{tt}^{\rm tot}$ 13 TeV Run II full lumi & 0.92 & -0.06 & 0.93 & -0.05 & 0.93 & -0.05 & 0.97 & -0.02 \\
ATLAS $t\bar{t}$ $y_t$ & 1.03 & 0.05 & 1.06 & 0.09 & 1.03 & 0.04 & 1.06 & 0.08 \\
ATLAS $t\bar{t}$ $y_{t\bar{t}}$ & 1.04 & 0.05 & 1.04 & 0.06 & 1.05 & 0.08 & 1.09 & 0.12 \\
ATLAS $t\bar{t}$ normalised $|y_t|$ & 1.13 & 0.21 & 1.13 & 0.21 & 1.14 & 0.22 & 1.18 & 0.28 \\
ATLAS jets 8 TeV, R=0.6 & 0.83 & -1.53 & 0.94 & -0.57 & 0.83 & -1.53 & 0.94 & -0.54 \\
ATLAS dijets 7 TeV, R=0.6 & 1.03 & 0.19 & 1.00 & 0.00 & 1.03 & 0.18 & 1.01 & 0.10 \\
ATLAS direct photon production 13 TeV & 0.97 & -0.16 & 1.03 & 0.14 & 0.98 & -0.13 & 1.03 & 0.16 \\
ATLAS single top $R_{t}$ 7 TeV & 1.14 & 0.10 & 1.25 & 0.18 & 1.06 & 0.04 & 1.16 & 0.11 \\
ATLAS single top $R_{t}$ 13 TeV & 0.91 & -0.07 & 1.01 & 0.01 & 0.94 & -0.04 & 1.05 & 0.03 \\
ATLAS single top $y_t$ (normalised) & 0.94 & -0.07 & 1.07 & 0.09 & 0.94 & -0.08 & 1.04 & 0.04 \\
ATLAS single antitop $y$ (normalised) & 0.92 & -0.10 & 0.91 & -0.11 & 0.94 & -0.07 & 0.98 & -0.03 \\
CMS $W$ asymmetry 840 pb & 0.99 & -0.03 & 0.99 & -0.02 & 0.97 & -0.08 & 1.05 & 0.12 \\
CMS $W$ asymmetry 4.7 fb & 0.97 & -0.07 & 0.97 & -0.06 & 0.97 & -0.06 & 0.97 & -0.06 \\
CMS Drell-Yan 2D 7 TeV 2011 & 1.01 & 0.05 & 1.01 & 0.07 & 1.01 & 0.04 & 1.01 & 0.08 \\
CMS $W$ rapidity 8 TeV & 1.06 & 0.21 & 1.11 & 0.38 & 1.07 & 0.25 & 1.11 & 0.38 \\
CMS $Z$ $p_T$ 8 TeV $(p_T^{ll},y_{ll})$ & 1.03 & 0.12 & 1.03 & 0.12 & 1.04 & 0.13 & 1.06 & 0.21 \\
CMS dijets 7 TeV & 0.97 & -0.15 & 1.05 & 0.24 & 0.97 & -0.13 & 1.05 & 0.28 \\
CMS jets 8 TeV & 0.99 & -0.11 & 1.00 & -0.02 & 0.99 & -0.05 & 1.01 & 0.06 \\
CMS $\sigma_{tt}^{\rm tot}$ 7 TeV & 0.86 & -0.10 & 0.95 & -0.03 & 0.86 & -0.10 & 0.99 & -0.00 \\
CMS $\sigma_{tt}^{\rm tot}$ 8 TeV & 1.18 & 0.13 & 1.08 & 0.06 & 1.22 & 0.16 & 1.07 & 0.05 \\
CMS $\sigma_{tt}^{\rm tot}$ 13 TeV & 0.98 & -0.01 & 1.11 & 0.08 & 0.99 & -0.01 & 1.13 & 0.09 \\
CMS $t\bar{t}$ rapidity $y_{t\bar{t}}$ & 1.06 & 0.12 & 1.04 & 0.08 & 1.03 & 0.07 & 1.02 & 0.05 \\
CMS $\sigma_{tt}^{\rm tot}$ 5 TeV & 0.86 & -0.10 & 0.77 & -0.16 & 0.81 & -0.13 & 0.73 & -0.19 \\
CMS $t\bar{t}$ double differential $(m_{t\bar{t}},y_{t\bar{t}})$ & 0.99 & -0.04 & 1.01 & 0.02 & 1.01 & 0.04 & 1.03 & 0.08 \\
CMS $t\bar{t}$ absolute $y_t$ & 1.01 & 0.03 & 1.02 & 0.04 & 1.02 & 0.04 & 1.05 & 0.11 \\
CMS $t\bar{t}$ absolute $|y_t|$ & 0.98 & -0.05 & 0.99 & -0.03 & 0.98 & -0.05 & 0.96 & -0.10 \\
CMS single top $\sigma_{t}+\sigma_{\bar{t}}$ 7 TeV & 0.93 & -0.05 & 0.91 & -0.06 & 0.88 & -0.09 & 0.86 & -0.10 \\
CMS single top $R_{t}$ 8 TeV & 0.64 & -0.26 & 1.21 & 0.15 & 0.65 & -0.25 & 1.15 & 0.10 \\
CMS single top $R_{t}$ 13 TeV & 1.50 & 0.35 & 1.44 & 0.31 & 1.46 & 0.32 & 1.40 & 0.28 \\
LHCb $Z$ 940 pb & 1.08 & 0.17 & 0.95 & -0.10 & 1.12 & 0.25 & 0.96 & -0.08 \\
LHCb $Z\to ee$ 2 fb & 1.03 & 0.08 & 1.04 & 0.12 & 1.01 & 0.02 & 1.01 & 0.03 \\
LHCb $W,Z \to \mu$ 7 TeV & 0.98 & -0.07 & 0.96 & -0.17 & 1.07 & 0.26 & 1.13 & 0.48 \\
LHCb $W,Z \to \mu$ 8 TeV & 1.08 & 0.32 & 1.12 & 0.45 & 1.17 & 0.65 & 1.32 & 1.22 \\
LHCb $Z\to \mu\mu$ & 1.09 & 0.26 & 1.05 & 0.14 & 1.10 & 0.28 & 1.05 & 0.15 \\
LHCb $Z\to ee$ & 1.07 & 0.19 & 1.03 & 0.08 & 1.08 & 0.22 & 1.04 & 0.11 \\
CMS HM DY 8 TeV & 0.98 & -0.09 & 0.98 & -0.08 & 0.99 & -0.05 & 1.00 & -0.02 \\
CMS HM DY 13 TeV - combined channel & 0.97 & -0.14 & 0.97 & -0.16 & 0.97 & -0.14 & 0.97 & -0.12 \\
HL-LHC HM DY 14 TeV - neutral current - electron channel & 1.01 & 0.03 & 1.03 & 0.08 & 1.04 & 0.10 & 1.21 & 0.53 \\
HL-LHC HM DY 14 TeV - neutral current - muon channel & 1.02 & 0.04 & 1.03 & 0.07 & 1.02 & 0.06 & 1.20 & 0.49 \\
HL-LHC HM DY 14 TeV - charged current - electron channel & 1.01 & 0.02 & 1.00 & -0.00 & 1.15 & 0.42 & 2.97 & 5.56 \\
HL-LHC HM DY 14 TeV - charged current - muon channel & 0.97 & -0.09 & 0.98 & -0.07 & 1.11 & 0.31 & 2.75 & 4.94 \\
\bottomrule
\end{tabular}
\caption{\label{tab:chi2_w} Fit quality in fits contaminated with the $\hat{W}$ parameter.}
\end{table}


==> Chapters/Contamination/tables/tab_chi2_w8.tex <==
\begin{table}[t]
        \tiny
        \centering
        \begin{tabular}{lc|c|c|c|c|c|}
                \toprule
       & & \multicolumn{2}{c}{SM} & \multicolumn{2}{c}{$W=8\cdot 10^{-5}$}\\
          \midrule
       Dataset  & $n_{\rm dat}$ & $\chi^2$ &  $n_\sigma$ & $\chi^2$ & $n_\sigma$ \\
          \midrule
 NMC $F^d_2/F^p_2$         & 121 & 0.90 & -0.78 & 0.94 &-0.47 \\
 NMC $\sigma^{\rm NC,p}$ & 204 & 0.93 & -0.71 & 0.93 &-0.71 \\
 SLAC $F^p_2$                   & 33 & 0.52 & -1.95 & 0.55 & -1.83 \\
SLAC $F^d_2$                   & 34 & 1.12 & +0.49 &  1.12 & +0.49 \\
BCDMS $F^p_2$                & 333 & 1.04 & +0.51 &1.03 &+0.39 \\
BCDMS $F^d_2$                & 248 & 0.93 & -0.78 & 0.93 &-0.78 \\
CHORUS $\sigma^\nu_{\rm CC}$ & 416 & 0.98 &-0.28&0.98 &-0.28 \\
CHORUS $\sigma^{\bar\nu}_{\rm CC}$& 416 & 0.95 &-0.72&0.95 &-0.72 \\
NuTeV $\sigma^\nu_{\rm CC}$ (dimuon) & 39 & 0.85 &-0.66& 0.87 &-0.57 \\
NuTeV $\sigma^{\bar\nu}_{\rm CC}$ (dimuon) & 37 & 0.48&-2.23& 0.59&-1.76 \\
                    \midrule
HERA I+II $\sigma^p_{\rm NC} e^-$ & 159 & 1.01&+0.09& 1.02&+0.18 \\
HERA I+II $\sigma^p_{\rm NC} e^+$ (460 GeV) & 204 &0.95&-0.51& 0.95&-0.51 \\
HERA I+II $\sigma^p_{\rm NC} e^+$ (575 GeV) & 254 &1.12 &+1.35&1.12 &+1.35 \\
HERA I+II $\sigma^p_{\rm NC} e^+$ (820 GeV) & 70 &0.89 &-0.65&0.90 &-0.59 \\
HERA I+II $\sigma^p_{\rm NC} e^+$ (920 GeV) & 377 & 0.94&-0.82&0.95 &-0.69 \\
          HERA I+II $\sigma^p_{\rm CC} e^+$ & 42 & 1.22&+1.01&1.22 &+1.01 \\
          HERA I+II $\sigma^p_{\rm CC} e^+$ & 39 & 1.06 &+0.26&1.03 &+0.13\\
          HERA I+II $\sigma^c_{\rm NC}$    & 37 & 0.83 &-0.73&0.84 &-0.69 \\
         HERA I+II $\sigma^b_{\rm NC}$     & 26 & 1.15 &+0.54&1.15&+0.54 \\
                \midrule
                \textbf{Total DIS} & \textbf{3089} & \textbf{0.98} &-0.79&\textbf{0.98} & -0.79 \\
                \midrule
           E886 \(\sigma^p\) (NuSea) & 89 & 1.02&+0.13&0.97 &-0.20 \\
           E886 \(\sigma^{d}/2\sigma^p\) (NuSea) & 15 & 1.17 &+0.46& 1.42&+1.15 \\
           E605 \(\sigma^p\) & 85 & 0.38&-4.04 &0.37 & -4.11\\
           E906 \(\sigma^{d}/2\sigma^p\) (SeaQuest) & 6 & 0.59&-0.71&0.67 &-0.57 \\
          \midrule
           CDF $Z$ differential & 28 & 1.02 &+0.07&1.00 &+0.00\\
           D0  $Z$ differential & 28 & 0.98 &-0.07& 1.00&+0.00\\
           D0  $W$ muon asymmetry & 9 &1.23 &+0.48&1.48 &+1.02\\
                \midrule
         ATLAS low-mass DY 7\,TeV & 6 &1.21 &+0.36&1.21 &+0.36 \\
         ATLAS \(W, Z\) 7 TeV (${\cal L}=35\,{\rm pb}^{-1}$) & 30 & 0.78&-0.85& 0.78&-0.85 \\
         ATLAS \(W, Z\) 7 TeV (${\cal L}=4.6\,{\rm fb}^{-1}$) central& 46 & 1.39&+1.87& 1.44&+2.11\\
         ATLAS \(W, Z\) 7 TeV (${\cal L}=4.6\,{\rm fb}^{-1}$) forward&15 & 0.91&-0.25& 0.92&-0.22 \\
         ATLAS low-mass DY 2D 8 TeV&60 & 0.87&-0.71& 0.86&-0.77 \\
        ATLAS $\sigma^{\rm tot}_{W,Z}$13 TeV & 3 &0.38 &-0.76&0.40&-0.73 \\
        ATLAS $W^+$+jet 8 TeV   &15&1.26&+0.71 &1.24 &+0.66 \\       
        ATLAS $W^-$ +jet 8 TeV   &15&1.02&+0.05 &0.98 &-0.05 \\       

          ATLAS $Z$ $p_T$ 8 TeV $(p_T , m_{ll})$& 44 &0.91 &-0.42&0.91 &-0.42 \\
          ATLAS $Z$ $p_T$ 8 TeV $(p_T , y_Z)$ & 48 &0.70 &-1.47&0.68 &-1.57 \\
                \midrule
CMS $W$ electron asymmetry 7 TeV & 11 &1.48&+1.13&1.50 &+1.17 \\
CMS $W$ muon asymmetry 7 TeV & 11 &1.22 &+0.52&1.28 &+0.66 \\
CMS $W$ rapidity 8 TeV& 22 &1.36 &+1.19& 1.37&+1.23 \\
 CMS  \(Z_{p_T}\) 8 TeV  & 28 &0.83&-0.64&0.82&-0.67\\
                \midrule
LHCb \(Z\rightarrow ee\)  7\,TeV & 9 &0.69&-0.66&0.69&-0.66 \\
LHCb \(W,Z\rightarrow\mu\) 7\,TeV & 29 &0.99&-0.04&0.94&-0.23 \\
LHCb \(Z\rightarrow ee\)  8\,TeV &17  &1.24&+0.70&1.24&+0.70 \\
LHCb \(W,Z\rightarrow\mu\) 8\,TeV &30&0.85&-0.58&0.74&-1.0\\
LHCb \(Z\rightarrow ee\)  13\,TeV & 15 &1.58&+1.59&1.60&+1.64 \\
LHCb \(Z\rightarrow\mu\) 13\,TeV & 16 &1.36&+1.02&1.37&+1.05 \\
                \midrule
                \textbf{Total DY (excl. HM)} & \textbf{670} & \textbf{xx} & \textbf{xx}& & \\
                \midrule
                ATLAS high-mass DY 7 TeV (${\cal L}=49\,{\rm fb}^{-1}$)& 13 &0.40 &-1.53& 0.40&-1.53 \\
                ATLAS high-mass DY 2D 8 TeV & 46 & 0.94&-0.29&0.94&-0.29 \\
                CMS high-mass DY 2D 7 TeV & 117 &0.92&-0.61&0.92&-0.61 \\
                CMS high-mass DY 8 TeV & 41 &1.30 &+1.36&1.29 &+1.31 \\
                CMS high-mass DY 13 TeV & 43 &1.06 &+0.28&1.07 &+0.32 \\
                \midrule
                \textbf{Total DY (HM only)} & \textbf{260} & \textbf{xx} & \textbf{xx}& & \\
                \midrule
%                \textbf{Total (excl. HL-LHC)} & \textbf{4715} & \textbf{xx} & \textbf{xx}& & \\
%                \midrule
                HL-LHC CC \(e\)& 16 & 0.79 &-0.60 & 1.00 & +0.0 \\ %% SM vs  Wcont   | Wcont vs SM
                HL-LHC CC \(\mu\)& 16 & 0.55 & -1.27 & 0.74 & -0.74\\
                HL-LHC NC \(e\)& 12 & 1.63 & +1.54 & 1.61 &+1.49 \\
                HL-LHC NC \(\mu\)& 12 & 0.81 &-0.46 & 0.79 &-0.51  \\
                \midrule
                \textbf{Total HL-LHC only} & \textbf{56} &\textbf{0.92} &-0.42 & \textbf{1.03} &+0.16 \\
                \midrule
                \textbf{Total} & \textbf{4771} & \textbf{0.97} & -1.41 & \textbf{0.96} &-1.89 \\
                \bottomrule
        \end{tabular}
        \caption{Values of the \(\chi^2\) per data point across all datasets
        used in this study. We tabulate values for the baseline PDF set as well
        as those obtained in the contaminated PDF fit. \label{tab:chi2w000008}}
\end{table}


==> Chapters/Contamination/tables/tab_chi2_weighted.tex <==
\begin{table}[t]
        \tiny
        \centering
        \begin{tabular}{lc|c|c|c|c|c|}
                \toprule
       & & \multicolumn{2}{c}{SM} & \multicolumn{2}{c}{$W=8\cdot 10^{-5}$}\\
          \midrule
       Dataset  & $n_{\rm dat}$ & $\chi^2$  & $\chi^2$ (weighted) & $\chi^2$ & $\chi^2$ (weighted) \\
          \midrule
           E866 (NuSea) & 89 & 0.80 & 0.81 & 0.98 & 1.14 \\
           D0  $W$ muon asymmetry & 9 & 2.38 & 2.76 & 3.05  & 3.82\\
         ATLAS \(W, Z\) 7 TeV (${\cal L}=4.6\,{\rm fb}^{-1}$) central & 46 & 0.81 & 0.82 & 0.82 & 0.82\\
         ATLAS \(W, Z\) 7 TeV (${\cal L}=4.6\,{\rm fb}^{-1}$) forward & 15 & 1.82 & 1.80 & 1.81 & 1.80 \\
%                \midrule
%                ATLAS high-mass DY 7 TeV (${\cal L}=49\,{\rm fb}^{-1}$)& 13 & 0.85  & 0.85 & 0.87 & 0.84 \\
%                ATLAS high-mass DY 2D 8 TeV & 46 & 0.86 & 0.85 & 0.88 & 0.86 \\
%                CMS high-mass DY 2D 7 TeV & 117 & 0.90 & 0.90 & 0.91 & 0.90 \\
%                CMS high-mass DY 8 TeV & 41 & 0.84 & 0.84 & 0.85 & 0.84 \\
%                CMS high-mass DY 13 TeV & 43 & 1.12 & 1.12 &1.13 & 1.13 \\
                \midrule
                HL-LHC NC \(e\)& 16 & 1.98 & 1.79 & 2.21 & 1.83 \\
                HL-LHC NC \(\mu\)& 16 & 1.10 & 1.04 & 1.17 & 1.05\\
                HL-LHC CC \(e\)& 12 & 0.75 & 0.74 & 1.14 & 0.77\\
                HL-LHC CC \(\mu\)& 12 & 0.65 & 0.64 & 1.16 & 0.63  \\
                \midrule
                \textbf{Total} & \textbf{4771} & \textbf{0.97} & -1.41 & \textbf{0.96} &-1.89 \\
                \bottomrule
        \end{tabular}
        \caption{\label{tab:chi2weighted} Values of the \(\chi^2\) per data point  in the baseline and in the $\hat{W}=8\cdot 10^{-5}$ contaminated fit 
        in the regular fit and in a weighted fit in which high-mass Drell-Yan data are given a larger weight according to Eq.~\eqref{eq:wgts}.}
\end{table}

==> Chapters/Contamination/tables/tab_chi2_y.tex <==
\begin{table}[t]
        \tiny
        \centering
\label{tab:chi2_y}
\begin{tabular}{lrrrrrrrr}
\toprule
 & \multicolumn{2}{r}{baseline} & \multicolumn{2}{r}{Y=5e-5} & \multicolumn{2}{r}{Y=15e-5} & \multicolumn{2}{r}{Y=25e-5} \\
 & $\chi^2$ & $n_\sigma$ & $\chi^2$ & $n_\sigma$ & $\chi^2$ & $n_\sigma$ & $\chi^2$ & $n_\sigma$ \\
\midrule
NMC $d/p$ & 1.02 & 0.14 & 1.02 & 0.12 & 1.03 & 0.24 & 1.06 & 0.45 \\
NMC $p$ & 1.03 & 0.26 & 1.02 & 0.23 & 1.02 & 0.18 & 1.02 & 0.18 \\
SLAC $p$ & 1.02 & 0.06 & 1.01 & 0.05 & 1.01 & 0.03 & 1.02 & 0.07 \\
SLAC $d$ & 1.00 & -0.01 & 0.98 & -0.07 & 0.99 & -0.02 & 0.99 & -0.04 \\
BCDMS $p$ & 1.02 & 0.20 & 1.00 & 0.06 & 1.02 & 0.21 & 1.01 & 0.11 \\
BCDMS $d$ & 1.01 & 0.07 & 1.00 & 0.01 & 1.01 & 0.08 & 1.00 & 0.03 \\
CHORUS $\sigma_{CC}^{\nu}$ & 1.00 & 0.02 & 1.00 & -0.06 & 1.00 & 0.06 & 1.00 & 0.01 \\
CHORUS $\sigma_{CC}^{\bar{\nu}}$ & 0.99 & -0.13 & 0.99 & -0.13 & 1.00 & -0.03 & 0.99 & -0.08 \\
NuTeV $\sigma_{c}^{\nu}$ & 0.99 & -0.06 & 0.99 & -0.05 & 0.99 & -0.02 & 1.00 & 0.02 \\
NuTeV $\sigma_{c}^{\bar{\nu}}$ & 0.96 & -0.19 & 0.98 & -0.08 & 1.00 & 0.00 & 1.05 & 0.23 \\
HERA I+II inclusive NC $e^-p$ & 1.00 & -0.02 & 1.01 & 0.12 & 1.00 & 0.02 & 1.02 & 0.17 \\
HERA I+II inclusive NC $e^+p$ 460 GeV & 1.01 & 0.08 & 1.01 & 0.12 & 1.01 & 0.13 & 1.02 & 0.18 \\
HERA I+II inclusive NC $e^+p$ 575 GeV & 0.98 & -0.21 & 1.00 & 0.01 & 0.99 & -0.17 & 1.01 & 0.07 \\
HERA I+II inclusive NC $e^+p$ 820 GeV & 1.00 & -0.00 & 1.01 & 0.07 & 1.00 & -0.01 & 1.01 & 0.09 \\
HERA I+II inclusive NC $e^+p$ 920 GeV & 1.02 & 0.29 & 1.05 & 0.63 & 1.03 & 0.35 & 1.05 & 0.67 \\
HERA I+II inclusive CC $e^-p$ & 0.99 & -0.05 & 1.03 & 0.13 & 0.99 & -0.03 & 1.03 & 0.15 \\
HERA I+II inclusive CC $e^+p$ & 1.02 & 0.08 & 1.02 & 0.07 & 1.03 & 0.11 & 1.04 & 0.18 \\
HERA comb. $\sigma_{c\bar c}^{\rm red}$ & 1.00 & 0.02 & 1.02 & 0.09 & 1.01 & 0.05 & 1.03 & 0.11 \\
HERA comb. $\sigma_{b\bar b}^{\rm red}$ & 1.12 & 0.43 & 1.13 & 0.45 & 1.14 & 0.49 & 1.13 & 0.48 \\
DYE 866 $\sigma^d_{\rm DY}/\sigma^p_{\rm DY}$ & 1.14 & 0.40 & 1.04 & 0.12 & 1.22 & 0.59 & 1.34 & 0.94 \\
DY E886 $\sigma^p_{\rm DY}$ & 1.02 & 0.14 & 1.02 & 0.13 & 1.04 & 0.26 & 1.05 & 0.36 \\
DY E605 $\sigma^p_{\rm DY}$ & 1.08 & 0.53 & 1.07 & 0.43 & 1.06 & 0.42 & 1.06 & 0.39 \\
DYE 906 $\sigma^d_{\rm DY}/\sigma^p_{\rm DY}$ & 1.80 & 1.39 & 1.14 & 0.25 & 1.41 & 0.70 & 1.46 & 0.80 \\
CDF $Z$ rapidity (new) & 1.06 & 0.21 & 1.03 & 0.12 & 1.06 & 0.21 & 1.01 & 0.06 \\
D0 $Z$ rapidity & 1.03 & 0.10 & 1.02 & 0.08 & 1.04 & 0.17 & 1.03 & 0.11 \\
D0 $W\to \mu\nu$ asymmetry & 1.23 & 0.50 & 1.06 & 0.13 & 1.32 & 0.69 & 1.18 & 0.38 \\
ATLAS $W,Z$ 7 TeV 2010 & 1.05 & 0.20 & 1.04 & 0.17 & 1.05 & 0.20 & 1.05 & 0.20 \\
ATLAS HM DY 7 TeV & 1.02 & 0.04 & 1.05 & 0.12 & 1.01 & 0.02 & 1.03 & 0.09 \\
ATLAS low-mass DY 2011 & 0.90 & -0.17 & 1.04 & 0.07 & 0.87 & -0.22 & 1.01 & 0.01 \\
ATLAS $W,Z$ 7 TeV 2011 Central selection & 1.06 & 0.28 & 1.07 & 0.36 & 1.07 & 0.31 & 1.07 & 0.35 \\
ATLAS $W,Z$ 7 TeV 2011 Forward selection & 0.91 & -0.25 & 1.33 & 0.90 & 0.90 & -0.29 & 1.32 & 0.87 \\
ATLAS DY 2D 8 TeV high mass & 1.02 & 0.11 & 1.03 & 0.13 & 1.02 & 0.08 & 1.03 & 0.12 \\
ATLAS DY 2D 8 TeV low mass & 1.03 & 0.16 & 1.00 & 0.00 & 1.02 & 0.13 & 0.99 & -0.04 \\
ATLAS $W,Z$ inclusive 13 TeV & 1.07 & 0.09 & 1.08 & 0.10 & 1.09 & 0.11 & 1.13 & 0.16 \\
ATLAS $W^+$+jet 8 TeV & 1.17 & 0.46 & 0.96 & -0.11 & 1.17 & 0.48 & 0.95 & -0.13 \\
ATLAS $W^-$+jet 8 TeV & 1.19 & 0.51 & 0.97 & -0.09 & 1.20 & 0.56 & 0.97 & -0.08 \\
ATLAS $Z$ $p_T$ 8 TeV $(p_T^{ll},M_{ll})$ & 1.01 & 0.03 & 0.98 & -0.07 & 1.01 & 0.04 & 0.99 & -0.05 \\
ATLAS $Z$ $p_T$ 8 TeV $(p_T^{ll},y_{ll})$ & 0.98 & -0.10 & 0.94 & -0.31 & 0.98 & -0.10 & 0.93 & -0.36 \\
ATLAS $\sigma_{tt}^{\rm tot}$ & 1.03 & 0.02 & 1.14 & 0.10 & 1.05 & 0.03 & 1.19 & 0.14 \\
ATLAS $\sigma_{tt}^{\rm tot}$ 8 TeV & 1.31 & 0.22 & 1.12 & 0.08 & 1.27 & 0.19 & 1.08 & 0.06 \\
ATLAS $\sigma_{tt}^{\rm tot}$ 13 TeV Run II full lumi & 0.92 & -0.06 & 0.93 & -0.05 & 0.97 & -0.02 & 0.98 & -0.01 \\
ATLAS $t\bar{t}$ $y_t$ & 1.03 & 0.05 & 1.06 & 0.08 & 1.04 & 0.06 & 1.04 & 0.05 \\
ATLAS $t\bar{t}$ $y_{t\bar{t}}$ & 1.04 & 0.05 & 1.04 & 0.05 & 1.06 & 0.08 & 1.05 & 0.07 \\
ATLAS $t\bar{t}$ normalised $|y_t|$ & 1.13 & 0.21 & 1.13 & 0.20 & 1.15 & 0.24 & 1.17 & 0.26 \\
ATLAS jets 8 TeV, R=0.6 & 0.83 & -1.53 & 0.94 & -0.58 & 0.83 & -1.55 & 0.94 & -0.60 \\
ATLAS dijets 7 TeV, R=0.6 & 1.03 & 0.19 & 1.00 & -0.00 & 1.04 & 0.24 & 1.01 & 0.09 \\
ATLAS direct photon production 13 TeV & 0.97 & -0.16 & 1.03 & 0.14 & 0.98 & -0.11 & 1.04 & 0.21 \\
ATLAS single top $R_{t}$ 7 TeV & 1.14 & 0.10 & 1.26 & 0.18 & 1.05 & 0.03 & 1.15 & 0.11 \\
ATLAS single top $R_{t}$ 13 TeV & 0.91 & -0.07 & 1.01 & 0.01 & 0.93 & -0.05 & 1.04 & 0.03 \\
ATLAS single top $y_t$ (normalised) & 0.94 & -0.07 & 1.07 & 0.09 & 0.93 & -0.09 & 1.04 & 0.04 \\
ATLAS single antitop $y$ (normalised) & 0.92 & -0.10 & 0.91 & -0.11 & 0.97 & -0.04 & 0.98 & -0.03 \\
CMS $W$ asymmetry 840 pb & 0.99 & -0.03 & 0.98 & -0.04 & 0.98 & -0.04 & 1.00 & -0.01 \\
CMS $W$ asymmetry 4.7 fb & 0.97 & -0.07 & 0.97 & -0.06 & 0.97 & -0.08 & 1.00 & 0.00 \\
CMS Drell-Yan 2D 7 TeV 2011 & 1.01 & 0.05 & 1.01 & 0.07 & 1.00 & 0.04 & 1.01 & 0.10 \\
CMS $W$ rapidity 8 TeV & 1.06 & 0.21 & 1.12 & 0.39 & 1.07 & 0.22 & 1.13 & 0.42 \\
CMS $Z$ $p_T$ 8 TeV $(p_T^{ll},y_{ll})$ & 1.03 & 0.12 & 1.03 & 0.11 & 1.03 & 0.12 & 1.04 & 0.14 \\
CMS dijets 7 TeV & 0.97 & -0.15 & 1.05 & 0.24 & 0.97 & -0.14 & 1.05 & 0.25 \\
CMS jets 8 TeV & 0.99 & -0.11 & 1.00 & -0.03 & 0.99 & -0.09 & 1.00 & -0.01 \\
CMS $\sigma_{tt}^{\rm tot}$ 7 TeV & 0.86 & -0.10 & 0.95 & -0.03 & 0.86 & -0.10 & 1.00 & 0.00 \\
CMS $\sigma_{tt}^{\rm tot}$ 8 TeV & 1.18 & 0.13 & 1.09 & 0.06 & 1.21 & 0.15 & 1.07 & 0.05 \\
CMS $\sigma_{tt}^{\rm tot}$ 13 TeV & 0.98 & -0.01 & 1.11 & 0.08 & 0.99 & -0.00 & 1.12 & 0.09 \\
CMS $t\bar{t}$ rapidity $y_{t\bar{t}}$ & 1.06 & 0.12 & 1.04 & 0.08 & 1.04 & 0.09 & 1.01 & 0.02 \\
CMS $\sigma_{tt}^{\rm tot}$ 5 TeV & 0.86 & -0.10 & 0.77 & -0.17 & 0.82 & -0.13 & 0.75 & -0.18 \\
CMS $t\bar{t}$ double differential $(m_{t\bar{t}},y_{t\bar{t}})$ & 0.99 & -0.04 & 1.00 & 0.01 & 1.02 & 0.04 & 1.03 & 0.07 \\
CMS $t\bar{t}$ absolute $y_t$ & 1.01 & 0.03 & 1.02 & 0.04 & 1.02 & 0.05 & 1.03 & 0.06 \\
CMS $t\bar{t}$ absolute $|y_t|$ & 0.98 & -0.05 & 0.99 & -0.03 & 0.97 & -0.06 & 0.96 & -0.09 \\
CMS single top $\sigma_{t}+\sigma_{\bar{t}}$ 7 TeV & 0.93 & -0.05 & 0.91 & -0.06 & 0.89 & -0.08 & 0.86 & -0.10 \\
CMS single top $R_{t}$ 8 TeV & 0.64 & -0.26 & 1.21 & 0.15 & 0.63 & -0.26 & 1.14 & 0.10 \\
CMS single top $R_{t}$ 13 TeV & 1.50 & 0.35 & 1.44 & 0.31 & 1.46 & 0.33 & 1.42 & 0.30 \\
LHCb $Z$ 940 pb & 1.08 & 0.17 & 0.96 & -0.09 & 1.11 & 0.24 & 0.97 & -0.06 \\
LHCb $Z\to ee$ 2 fb & 1.03 & 0.08 & 1.04 & 0.13 & 1.01 & 0.02 & 1.04 & 0.11 \\
LHCb $W,Z \to \mu$ 7 TeV & 0.98 & -0.07 & 0.97 & -0.10 & 1.02 & 0.06 & 1.01 & 0.05 \\
LHCb $W,Z \to \mu$ 8 TeV & 1.08 & 0.32 & 1.13 & 0.51 & 1.09 & 0.35 & 1.18 & 0.68 \\
LHCb $Z\to \mu\mu$ & 1.09 & 0.26 & 1.05 & 0.15 & 1.10 & 0.27 & 1.05 & 0.13 \\
LHCb $Z\to ee$ & 1.07 & 0.19 & 1.03 & 0.08 & 1.07 & 0.19 & 1.04 & 0.10 \\
CMS HM DY 8 TeV & 0.98 & -0.09 & 0.98 & -0.08 & 0.97 & -0.13 & 0.98 & -0.10 \\
CMS HM DY 13 TeV - combined channel & 0.97 & -0.14 & 0.97 & -0.16 & 0.97 & -0.14 & 0.97 & -0.15 \\
HL-LHC HM DY 14 TeV - neutral current - electron channel & 1.01 & 0.03 & 1.15 & 0.36 & 2.08 & 2.64 & 4.22 & 7.88 \\
HL-LHC HM DY 14 TeV - neutral current - muon channel & 1.02 & 0.04 & 1.15 & 0.37 & 2.09 & 2.66 & 4.16 & 7.75 \\
HL-LHC HM DY 14 TeV - charged current - electron channel & 1.01 & 0.02 & 0.98 & -0.07 & 1.03 & 0.08 & 0.99 & -0.03 \\
HL-LHC HM DY 14 TeV - charged current - muon channel & 0.97 & -0.09 & 0.95 & -0.14 & 1.01 & 0.02 & 0.98 & -0.05 \\
\bottomrule
\end{tabular}
\caption{\label{tab:chi2_y} Fit quality in fits contaminated with the $\hat{Y}$ parameter.}
\end{table}


==> Chapters/SIMUnet/sec-data.tex <==
\section{A first global simultaneous fit of SMEFT WCs and PDFs}
\label{sec:data}

In this section we present the first global simultaneous fit of SMEFT WCs and PDFs, including Deep-Inelastic-Scattering, 
Drell-Yan, top, jets, Higgs, diboson and EW precision observables.  This analysis can be now performed thanks to the 
\simunet{} methodology that we have described so far. 
We start in Sect.~\ref{subsec:data} by listing the data that have been included, and giving details of their implementation. 
In Sect.~\ref{subsec:fixedpdf} we 
present the result of the fixed-PDF analysis, 
producing a global SMEFT fit of a large number of datapoints from the Higgs, top, and EW sectors ($n_{\rm data}\,=\,366$)
to a set of $n_{\rm op}\,=\,40$ SMEFT operators.
Finally in Sect.~\ref{subsec:simu} we present the 
simultaneous PDF and SMEFT global fit ($n_{\rm data}\,=\,4985$).
We compare the resulting PDFs and SMEFT bounds to the SM PDFs and to the SMEFT bounds obtained in the fixed-PDF fit respectively, hence 
assessing the effect of the interplay between PDFs and SMEFT effects on both our description of the proton and 
on New Physics bounds. 

\subsection{Experimental data}
\label{subsec:data}
The dataset explored in this study builds on those already implemented in the high-mass Drell-Yan analysis 
presented in Refs.~\cite{Greljo:2021kvv,Iranipour:2022iak} and on the
top quark analysis presented in Ref.~\cite{Kassabov:2023hbm}. 
These studies extended the datasets included in the global \nnpdf{}~\cite{NNPDF:2021njg} analysis, 
by adding observables that enhance the sensitivity to the SMEFT and that constrain PDFs in the Drell-Yan and in the 
top sector respectively. 

The \nnpdf{} NNLO analysis~\cite{NNPDF:2021njg} included $n_{\rm data}\,=\,4618$ data points corresponding to a wide variety of processes in
deep-inelastic lepton-proton scattering (from the HERA $ep$ collider and from fixed-target experiments such as NMC, SLAC, 
BCDMS, CHORUS and NuTeV), fixed-target DY data from the
Fermilab E605 and E866 experiments, hadronic proton-antiproton collisions from the Tevatron, and proton-proton collisions from LHC. 
The LHC data in turn include inclusive gauge boson production data; $Z$- and $W$-boson transverse momentum production data, 
single-inclusive jet and di-jets production data, as well as gauge boson with jets and inclusive isolated photon
production data and top data. 
In Refs.~\cite{Greljo:2021kvv,Iranipour:2022iak} the high-mass Drell-Yan sector of the \nnpdf{} analysis 
was augmented by two extra measurements taken by CMS at $\sqrt{s}=8,13$ TeV, for a total of 65 extra datapoints. 
In Ref.~\cite{Kassabov:2023hbm}, besides inclusive and differential $t\bar{t}$ cross sections and $t$-channel 
single top production already implemented in \nnpdf{}, more observables were included, such as $t\bar{t}$ production asymmetries, 
$W$-helicity fractions, associated top pair production with vector bosons and heavy quarks, including 
$\bar{t}t Z$, $\bar{t}t W$, $\bar{t}t \gamma$, $\bar{t}t\bar{t}t$, $\bar{t}t\bar{b}b$, $s$-channel 
single top production, and associated single top and vector boson production, bringing the total number of datapoints to $n_{\rm data}\,=\,4710$. 

In this present study, we further extend the datasets by probing electroweak precision observables (EWPOs), 
the Higgs sector and the diboson sector. 
The datasets are described below and details such as the centre-of-mass energy, the observable, the integrated luminosity, the number 
of data points, the dataset name as implemented in \simunet \ and the source are given 
in Tables~\ref{tab:dataset_EWPO},~\ref{tab:dataset_Higgs} and~\ref{tab:dataset_diboson} respectively. 

We remind the reader that, thanks to the functionality of \simunet{} that enables users to include PDF-independent observables 
as well as to freeze PDFs for the observables in which the PDF dependence is mild, we can add observables such as the measurement of 
$\alpha_e$ that are completely independent of PDFs (but which are affected by SMEFT corrections) or Higgs signal strengths and Simplified Template Cross Section (STXS) measurements that 
are mildly dependent on PDFs but are strongly dependent on the relevant SMEFT-induced corrections. 

To summarise, in this analysis we include a total of {\bf 4985 datapoints}, of which 366 are affected by SMEFT corrections. 
Among those 366 datapoints, 210 datapoints are PDF independent. 
Hence our pure PDF analysis performed with \simunet{} includes $(4985-210) = 4775$ datapoints and is equivalent to the 
\nnpdf{} global analysis augmented by 78 datapoints from the top sector~\cite{Kassabov:2023hbm} and 
by 65 datapoints measuring the high-mass Drell-Yan tails~\cite{Greljo:2021kvv,Iranipour:2022iak}. Our pure 
SMEFT-only analysis performed with \simunet{} includes 366 datapoints, while our simultaneous PDF-SMEFT fit includes 
4985 datapoints. 

\vspace*{0.4cm}
\noindent {\bf EWPOs:}
In Table~\ref{tab:dataset_EWPO}, we list EWPOs included in this study. 
The dataset includes the pseudo-observables
measured on the $Z$ resonance by LEP~\cite{ALEPH:2005ab}, 
which include cross sections, forward-backward and polarised asymmetries. 
Branching ratios of the decay of the $W$ boson into leptons~\cite{ALEPH:2013dgf} are also included, 
along with the LEP measurement of the Bhabha scattering cross section~\cite{ALEPH:2013dgf}. 
Finally we include the measurement of the effective electromagnetic coupling constant~\cite{Workman:2022ynf}, 
for a total of {\bf 44 datapoints}.  These datasets and their SMEFT predictions
are taken from the public \smefit{} code
\cite{Giani:2023gfq,terHoeve:2023pvs}.
These datapoints are all PDF independent, hence they directly 
affect only the SMEFT part of the fits.
\input{tab-data-LEP.tex}

\vspace*{0.4cm}
\noindent {\bf Higgs sector:}
In Table~\ref{tab:dataset_Higgs}, we list the Higgs sector datasets included in this study. 
The Higgs dataset at the LHC includes the combination of Higgs signal strengths
by ATLAS and CMS for Run 1, and for Run 2 both signal strengths and STXS
measurements are used. ATLAS in particular provides the combination of stage 1.0 STXS bins
for the $4l$, $\gamma\gamma$, $WW$, $\tau\tau$ and $b\bar{b}$ decay channels, while for CMS we use the combination
of signal strengths of the $4l$,
$\gamma\gamma$, $WW$, $\tau^-\tau^+$, $b\bar{b}$ and $\mu^-\mu^+$ decay channels. 
We also include the $H \rightarrow Z\gamma$ 
and $H \rightarrow \mu^-\mu^+$ signal strengths from ATLAS, for a total of {\bf 73 datapoints}. 
The Run I and CMS datasets and their corresponding predictions are
taken from the \smefit{} code~\cite{Giani:2023gfq,terHoeve:2023pvs},
whereas the STXS observables and signal strength measurements of
$H \rightarrow Z\gamma$ and $H \rightarrow \mu^-\mu^+$ are taken from the \fitmaker ~\cite{Ellis:2020unq} code.
The signal strength's dependence on the PDFs is almost completely negligible, given that the 
PDF dependence cancels in the ratio, hence all the datapoints are treated as PDF independent and 
are directly affected only by the SMEFT Wilson coefficients.
\input{tab-data-HIGGS.tex}

\vspace*{0.4cm}
\noindent {\bf Diboson sector:}
In Table~\ref{tab:dataset_diboson}, we list the diboson sector datasets included in this study. 
We have implemented four measurements from LEP at low energy, three from ATLAS and one from CMS both at 13 TeV. 
The LEP measurements are of the differential 
cross-section of $e^+ e^- \rightarrow W^+ W^-$ as a function of the cosine of the $W$-boson polar angle. 
The ATLAS measurements are of 
the differential cross-section of $W^+ W^-$ as a function of the invariant mass of the electron-muon pair 
and of the transverse mass of the $W$-boson. 
The third ATLAS measurement is of the differential cross-section of $Zjj$ as a function of the azimuthal angle 
between the two jets, $\Delta \phi_{jj}$.  Although this is not a diboson 
observable, it is grouped here as this observable constrains operators typically 
constrained by the diboson sector,
such as the triple gauge interaction $O_{WWW}$. The CMS dataset is a measurement of the differential cross-section of $WZ$ as 
a function of the transverse momentum 
of the $Z$-boson, for a total of {\bf 82 datapoints}. 
Almost all datasets and corresponding predictions in this sector are
taken from the \smefit{} code~\cite{Giani:2023gfq, terHoeve:2023pvs},
except for the ATLAS measurement of $Zjj$ production, taken from the \fitmaker ~\cite{Ellis:2020unq} code.
While the LEP measurements are PDF-independent by definition, 
the LHC measurements of diboson cross sections do depend on PDFs. However, their impact on the 
PDFs is extremely mild, due to much more competitive constraints in the same Bjorken-$x$ region given by other measurements
such as single boson production and single boson production in association with jets. 
Therefore we consider all diboson measurements 
to be PDF-independent, i.e. the PDFs are fixed and their parameters are not varied in the computation of these observables. 
\input{tab-data-VV.tex}

\vspace*{0.4cm}
\noindent {\bf SMEFT Wilson coefficients:}
We include a total of 40 operators from the dimension-6 SMEFT in our global analysis 
of the measurements of the
Higgs, top, diboson and electroweak precision observables outlined above.
%
\begin{figure}[thb!]
    \centering
    \includegraphics[width=0.7\textwidth]{venn.eps}
    \caption{Schematic representation of the data categories included in this analysis and of 
    their overlapping dependences on the 40 dim-6 SMEFT operators included in our global analysis, 
    adapted from Ref.~\cite{Ellis:2020unq}.}
\label{fig:operators}
\end{figure}
%
In Fig.~\ref{fig:operators} we display the SMEFT Wilson coefficients included in our analysis, following
the operator conventions of Refs.~\cite{Kassabov:2023hbm,Ethier:2021bye}. 
The schematic diagram, adapted from Ref.~\cite{Ellis:2020unq}, demonstrates the sectors of data affected by each WC and highlights
the interconnected nature of the global SMEFT determination.
The overlaps between the different rectangles show explicitly how a given operator contributes to several data categories.
For example, $O_{WWW}$, contributes to both the diboson sector and the top sector (through its contribution to $tZq$ production),
while the operators $O_{\varphi e}$,$O_{\varphi l}$ contribute to the Higgs, diboson 
and electroweak sectors, but have no effect on the top sector.


==> Chapters/SIMUnet/sec-results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Global SMEFT fit}
\label{subsec:fixedpdf}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We present the results of this new global fit in two parts, beginning with a discussion 
of the result of the fixed PDF fit, that is a global fit purely of the SMEFT Wilson 
coefficients. 
In Sect.~\ref{subsec:simu} we will present the results of the simultaneous global 
fit of SMEFT WCs and will compare the results to those obtained here.

The global analysis is performed at linear order in the SMEFT operator
coefficients, accounting for the interference between the SM and the insertion of a dimension-6 SMEFT operator. 
The linear constraints can be viewed as 
provisional for operators where quadratic contributions are non-negligible. Nevertheless,
keeping those operators in the global fit typically yields conservative marginalised limits
that allows one to assess the impact on other operators and whether this is significant to a first
approximation. An analysis including quadratic constributions requires a new methodology that does not 
rely on the Monte-Carlo sampling method to propagate uncertainties~\cite{progr}, given that the latter fails at
reproducing the Bayesian confidence intervals once quadratic corrections are dominant,  
as described in App.~E of Ref.~\cite{Kassabov:2023hbm}.

Our analysis comprises  $n_{\rm op} = 40$ operators in a simultaneous combination of the constraints 
from $n_{\rm data}\,=\,366$ datapoints 
from the Higgs, EWPO, diboson and top sectors. Note that in the \simunet{} code there 
are more SMEFT operators implemented, in particular the set of four-fermion operators that 
affect Drell-Yan and DIS data. As demonstrated in~\cite{Carrazza:2019sec,Greljo:2021kvv}, 
the effect of the four 
fermion operators in DIS and on the current Drell-Yan data, including the high-mass Drell-Yan 
data included in \nnpdf{} is not significant enough for this data to provide strong constraints 
on the relevant set of four-fermion operators. 
On the contrary, the HL-LHC projections, which include both neutral and charged current 
Drell-Yan data have a strong potential in constraining such operators~\cite{Iranipour:2022iak}. 
As a results, Drell-Yan data are not affected by SMEFT corrections in this current analysis, 
but we leave the user the opportunity to include such effects straightforwardly, 
should the measurements by the LHC increase the constraining potential, or should the user combine 
those with flavour observables, as is done in Ref.~\cite{Bartocci:2023nvp}.

In the following, we also omit from the results the $4$ heavy quark production datasets (four tops and $t\bar{t}b\bar{b}$). 
Their effect is practically negligible on all the operators affecting the other sectors and they would simply constrain $2$ 
directions in the $5$-dimensional space of the four heavy fermion operators. These observables are therefore {\it de facto} decoupled 
from the rest of the dataset.

The input PDF set, which is kept fixed during the pure SMEFT fit, is the {\tt nnpdf40nnlo\_notop} 
baseline, corresponding to the \nnpdf{} fit without the top data, to avoid possible contamination 
between PDF and EFT effects in the top sector~\cite{Kassabov:2023hbm}. 

The sensitivity to the EFT operators of the various processes entering the fit can
be evaluated by means of the Fisher information, which, for $N$ EFT coefficients, is an $N \times N$ matrix given by
\begin{equation}
  \label{eq:fisher}
  F_{ij} = {L_{i}}^T (\text{cov}_{\text{exp}})^{-1} L_{j} .
\end{equation}
Here $L_{i}$ is the vector of the linear contributions to the observables of the $i$-th SMEFT Wilson coefficient, 
entering into the theory prediction $T(c)$ as $T(c)_{\alpha} = T(c)^{\rm SM}_{\alpha} + (L_i)_{\alpha} c_i$, where the index
$\alpha$ runs over the datapoints in the fit, and $\text{cov}_{\text{exp}}$ is the experimental covariance matrix. The covariance matrix in the space of SMEFT coefficients $C_{ij}$, 
by the Cramér-Rao bound, satisfies $C_{ij} \geq (F^{-1})_{ij}$, hence the larger the entries of the Fisher information matrix, 
the smaller the possible uncertainties of the SMEFT coefficients and, therefore, the bigger the constraining power of the relevant dataset. 
%
\begin{figure}[tb!]
  \centering
  \includegraphics[width=0.9\textwidth]{plot_fisher_information_by_sector.eps}
  \caption{
Relative constraining power (in \%) on each of the operators for each of the processes entering the fit, 
as defined in Eq.~\eqref{eq:relativeconstrainingpower_simu}.}
\label{fig:fisher}
\end{figure}
%
In Fig.~\ref{fig:fisher} we use the Fisher information to assess the relative impact of each sector of 
data included in our analysis on the SMEFT parameter space by plotting the relative percentage constraining power of the dataset $D$
via:
\begin{equation}
\label{eq:relativeconstrainingpower_simu}
	\textrm{relative constraining power of }D\textrm{ on operator }c_i = F_{ii}(D) \bigg/ \displaystyle \sum_{\text{sectors }D'} F_{ii}(D'),
\end{equation}
%
which gives a general qualitative picture of some of the expected behaviour in the global fit. 
%
In Fig.~\ref{fig:fisher} we observe that the coefficients $c_{tZ}$, $c_{tW}$ are dominantly constrained by the Higgs sector, while
the coefficient $c_{tG}$ is now constrained both by the $t \bar{t}$ total cross sections and by the 
Higgs measurements, as expected.
Higgs measurements also provide the dominant constraints on the bosonic coefficients
$c_{\varphi G}$, $c_{\varphi W}$, $c_{\varphi B}$, $c_{\varphi \Box}$
and on the Yukawa operators.
Coefficients coupling the Higgs to fermions,
$c_{\varphi Q}^{(3)}$,
$c_{\varphi q}^{(3)}$, $c_{\varphi Q}^{(-)}$, $c_{\varphi q}^{(-)}$, $c_{\varphi u}$, $c_{\varphi d}$,
$c_{\varphi l}^{(3)}$ and $c_{\varphi e}$, receive their dominant constraining power from the electroweak precision observables,
as does the four-fermion coefficient $c_{ll}$.
The coefficient $c_{WWW}$ is constrained by the diboson sector, with measurements of $Zjj$ production
providing the leading constraints at linear order in the SMEFT.
From the top sector of the SMEFT, the four-fermion operators are constrained by measurements of top quark pair
production total cross sections, differential distributions and charge asymmetries.  The exception to this is $c_{Qq}^{(1,3)}$,
which is constrained by both single top production and single top production in association with a $Z$ boson.
Overall we find qualitatively similar results to those shown in Refs.~\cite{Ellis:2020unq,Ethier:2021bye}.

To assess the strength of the bounds on the Wilson coefficients that we find in this work and 
for reference, in Fig.~\ref{fig:simunet_vs_fitmaker} we compare the bounds that we obtain here 
against the fixed-PDF SMEFT analysis presented by the \fitmaker{} 
collaboration~\cite{Ellis:2020unq}, which is the global public SMEFT analysis that currently 
includes all sectors that are considered here.
%
\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.8\textwidth]{fitmaker_vs_simunet_linear.eps}
    \caption{
  Comparison of the bounds for the SMEFT Wilson coefficients determined in the pure  
  SMEFT analysis presented in this work and the \fitmaker{} analysis~\cite{Ellis:2020unq}. 
  The dashed horizontal line is the SM prediction. In each bound, the dot represents 
  the best-fit value and the 95\% CL interval is constructed from the envelope of 
  two standard deviations away from this best-fit value.}
\label{fig:simunet_vs_fitmaker}
\end{figure}
%
We observe that the bounds are comparable, with a few differences. First of all \fitmaker{} 
uses LO QCD predictions for the SMEFT corrections in the top sector, hence most of the singlet four 
fermion operators in the top sector are not included, while \simunet{} uses NLO QCD predictions 
and obtains bounds on those, although weak~\cite{Degrande:2020evl}. Moreover, while the 
other bounds overlap and are of comparable size, the ${\cal O}_{tZ}$ is much more constrained in 
the \simunet{} analysis, as compared to the \fitmaker{} one. 
This is due to the combination of all operators and observables, which collectively improves the constraints 
on this specific operator, thanks to the interplay between $O_{tZ}$ and the other operators that enter the same 
observables. 


In Fig.~\ref{fig:smeft_only_top_vs_global} we show the comparison between the results of this current global SMEFT analysis against 
the SMEFT analysis of the top sector presented in~\cite{Kassabov:2023hbm}.
%
\begin{figure}[b!]
  \centering
  \includegraphics[width=0.8\textwidth]{fixed_pdf_top_vs_global_lin_without_0_dots.eps}
  \caption{Same as Fig.~\ref{fig:simunet_vs_fitmaker}, now comparing the 95\% CL bounds obtained in the SMEFT top analysis 
  of Ref.~\cite{Kassabov:2023hbm} (old dataset) with the 95\% CL bounds obtained in this global SMEFT analysis.}
\label{fig:smeft_only_top_vs_global}
\end{figure}
%
In general, the results are very compatible, with bounds on most Wilson coefficients comparable between the two fits. 
However, the increased dataset size results in a marked improvement on the constraints of several Wilson coefficients, 
in particular $c_{\phi t}$, $c_{tZ}$ and $c_{\phi Q}^{(-)}$; see Table~\ref{tab:global_vs_top} for comparisons. 
%
\begin{table}[ht]
  \begin{center}
{\fontsize{8pt}{8pt}\selectfont
%\begin{table}[t]
  \centering
   \renewcommand{\arraystretch}{2}
   \setlength{\tabcolsep}{5pt}
   \begin{tabular}{lcc}
   \toprule
    \textbf{Operator} & \textbf{Global fit} & \textbf{Top fit} \\% & \textbf{Broadening} \\
  \toprule
  $c_{\phi t}$ & (-13, -0.22)  & (-18, 3.1) \\%& $-39.4$\%  \\
  \midrule
  $c_{tZ}$ & (-0.18, 0.37)  & (-13, 5.5) \\%& $-97.0$\%  \\
  \midrule
  $c_{\phi Q}^{(-)}$ & (-3.6, -0.042)  & (-9.4, 3.4)\\% & $-72.2$\%  \\
   \bottomrule
  \end{tabular}
  }
\end{center}
    \caption{\label{tab:global_vs_top} The 95\% confidence intervals on three key Wilson coefficients included in this analysis.}
  \end{table}
  %
We observe that the bounds on $c_{\phi t}$ become more stringent by nearly a factor of 2, due to the extra constraints that come 
from the Higgs sector. Analogously, the Higgs constrains reduce the size of the bounds on $c_{\phi Q}^{(-)}$ by a factor of 3. 
The most remarkable effect is seen in $c_{tZ}$ which is now strongly constrained by the top loop contribution to the $H\to\gamma\gamma$ 
decay, for which we include experimental information on the signal strength from LHC Run II. 


\begin{figure}[tb!]
  \centering
  \includegraphics[width=0.47\textwidth]{fisher_top.eps}
  \includegraphics[width=0.47\textwidth]{fisher_global.eps}
  \caption{The values of the correlation coefficients evaluated between all pairs of Wilson coefficients entering the
  SMEFT fit of the top-only analysis (left) and the global analysis (right). }
\label{fig:fisher_info}
\end{figure}
It is interesting to compare the correlations between Wilson coefficients evaluated in this analysis
to the top-only SMEFT analysis of Ref.~\cite{Kassabov:2023hbm}. In Fig.~\ref{fig:fisher_info} we 
note that the additional sectors, particularly the Higgs one, 
introduce a degree of anti-correlation between $c_{\phi Q}^{(3)}$ and $c_{\phi t}$ and between $c_{Q q}^{(8,3)}$ and $c_{Q q}^{(1,3)}$, 
while the one between $c_{u t}^{8}$ and $c_{d t}^{8}$ goes away in the global analysis. In the EW sector, we find very strong correlations, 
in agreement with similar studies in the literature. This suggests that there is room for improvement in the sensitivity to the operators 
affecting EW observables once more optimal and targeted measurements are employed in future searches~\cite{GomezAmbrosio:2022mpm,Long:2023mrj}. 

Finally we display the correlations  observed between the PDFs and Wilson coefficients.
The PDF-EFT correlation coefficient for a Wilson coefficient $c$ and a
PDF $f(x, Q)$ at a given $x$ and $Q^2$ is defined as
%
\begin{equation}
\label{eq:correlationL2CT_simu}
\rho\lp c, f(x,Q^2)\rp=\frac{\la c^{(k)}f^{(k)}(x,Q^2)\ra_k - \la c^{(k)}\ra_k \la f^{(k)}(x,Q^2)\ra_k
}{\sqrt{\la (c^{(k)})^2\ra_k - \la c^{(k)}\ra_k^2}\sqrt{\la\left( f^{(k)}(x,Q^2)\right)^2\ra_k - \la f^{(k)}(x,Q^2)\ra_k^2}}  \, ,
\end{equation}
%
where $c^{(k)}$ is the best-fit value of the Wilson coefficient for
the $k$-th replica and $f^{(k)}$ is the $k$-th PDF replica computed at
a given $x$ and $Q$, and $\la \cdot \ra_k$ represents the average
over all replicas. We compute the correlation between a SM PDF and the Wilson coefficients of
this new global analysis. By doing so we have a handle on 
which PDF flavours and kinematical regions are strongly impacted by the presence of
a given SMEFT-induced correction to the SM theoretical predictions, thus exhibiting a potential for interplay
in a simultaneous EFT-PDF determination.
%
\begin{figure}[hbt!]
  \centering
          \includegraphics[width=0.48\textwidth]{correlations_fitpdf_plot_bsm_pdf_corr_Otz.eps}
          %
          \includegraphics[width=0.48\textwidth]{correlations_fitpdf_plot_bsm_pdf_corr_Ophit.eps}
    \caption{The value of the correlation coefficient $\rho$
            between the PDFs and selected EFT coefficients as a function of $x$
            and $Q=172.5$ GeV.
            %
            We show the results for the gluon, the total singlet $\Sigma$, total valence $V$, and non-singlet
            triplet $T_3$ PDFs.
            We provide results for representative EFT coefficients,
            namely $c_{tZ}$ and  $c_{\phi t}$.
          }
  \label{fig:pdfbsmcorr_simu}
  \end{figure}
Fig.~\ref{fig:pdfbsmcorr_simu} displays a selection of the largest correlations.
We observe that the gluon PDF in the medium to large-$x$ region is significantly correlated with the Wilson coefficients 
$c_{tZ}$, as one would expect given that $c_{tZ}$ is strongly constrained by the top loop contribution to the Higgs decay, which
in turn is predominantly correlated to the gluon-gluon parton luminosity. On the other hand $c_{\phi t}$ is anticorrelated
with the gluon and correlated to the singlet and triplet in the large-$x$ region.
This is not surprising, given the impact of top quark pair production total cross sections and differential distributions
in constraining these PDFs and Wilson coefficients.  
Whilst these correlations are computed from a determination of the SMEFT in which the PDFs are fixed to SM PDFs, 
the emergence of non-zero correlations provides an indication of the potential for interplay between the PDFs and the SMEFT
coefficients; this interplay will be investigated in a simultaneous determination
in the following section.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Global simultaneous SMEFT and PDF fit}
\label{subsec:simu} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section we present the results of the simultaneous global fit of SMEFT Wilson coefficients and PDFs. We 
compare the bounds on the coefficients obtained in the two analyses as well as the resulting PDF sets, 
to assess whether the inclusion of more PDF-independent observables modifies the interplay 
observed in the top-focussed analysis of Ref.~\cite{Kassabov:2023hbm}.

The first observation is that, similarly to the top-sector results observed in Ref.~\cite{Kassabov:2023hbm}, 
in the global fit presented here the interplay between PDFs and SMEFT Wilson coefficients is weak. 
Indeed in Fig.~\ref{fig:fixed_vs_simu} we observe that, including all data listed in Sect.~\ref{subsec:data}, 
the bounds on the SMEFT Wilson coefficients are essentially identical in a SMEFT-only fit and  
in a simultaneous fit of SMEFT WCs and PDFs. The only mild sign of interplay is shown by the 
operator $c_{\phi t}$, which undergoes a fair broadening in the simultaneous fit compared to the fixed-PDF 
SMEFT fit.
%
\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.8\textwidth]{95_CL_smeftpdf_vs_fixedpdf_linear_scale.eps}
\caption{
  Comparison of the 95\% CL intervals on the 40 Wilson coefficients considered in this work (in the linear
EFT case) between the outcome of the joint SMEFT-PDF determination and that of the fixed-PDF EFT analysis. The
latter is based on SM and EFT calculations performed with {\tt NNPDF4.0-notop} as input. In both cases,
results are based on the global dataset being considered and SMEFT cross-sections are evaluated up to linear,
corrections. The dashed horizontal line indicates the SM prediction, $c_k = 0$. Note that some coefficients are
multiplied by the indicated prefactor to facilitate the visualisation of the results.}
\label{fig:fixed_vs_simu}
\end{figure}

The PDF fit is more interesting. It was shown in Ref.~\cite{Kassabov:2023hbm} that when comparing: 
(i) a SM PDF fit excluding top data, (ii) a simultaneous PDF-SMEFT using top data, 
(iii) a SM PDF fit including top data, there is a hierarchy of shifts in the gluon-gluon luminosity 
at high invariant masses. In particular, the gluon-gluon luminosity of the simultaneous fit (ii) is reduced at high 
invariant masses compared to fit (i), whilst the gluon-gluon luminosity of the SM fit including all top data 
(iii) is even further reduced at high invariant masses relative to the result of the simultaneous fit (ii). 
This can be explained due to the additional SMEFT degrees of freedom in (ii) allowing for a better description 
of the top data with the PDF remaining compatible with the no-top PDF.

\begin{figure}[tb!]
\centering
\includegraphics[width=0.7\textwidth]{fixed_vs_simu_gglumi.eps}
\caption{ \label{fig:gglumi} The gluon-gluon partonic luminosities at $\sqrt{s} = 13$ TeV
as a function of the final-state invariant mass $m_X$. We compare the {\tt NNPDF4.0-notop} 
baseline fit with its SM-PDF counterpart including all new data presented in Sect.~\ref{subsec:data}, 
as well as with the simultaneous SMEFT-PDF determination. Results are presented as the ratio to the 
central value of the {\tt NNPDF4.0-notop} baseline.}
\end{figure}
As it can be observed in Fig.~\ref{fig:gglumi}, 
in the new global fit presented in this chapter, there is a shift in the gluon-gluon luminosity in the simultaneous 
PDF and SMEFT fit relative to the baseline no-top PDF set, however the shift is much smaller than the shift that one 
has by including all data in the SM, meaning that the effect of the inclusion of the top, Higgs, EWPO and diboson
data has a much smaller effect on the PDFs due to the interplay between the pull of the SMEFT coefficients and the 
pull of the new data on the PDFs.  
The shift is even smaller compared to the shift of the simultaneous top fit relative to the no-top 
PDF presented in Ref.~\cite{Kassabov:2023hbm}. 
This is due to the inclusion of new high-mass Drell-Yan data in the new fit, which were not 
included in \nnpdf{}. These data favour a softer singlet PDF combination in the high-mass region, 
and as a result they enhance the gluon in the same region, due to sum rules. 

Finally, it is also interesting to compare the fit quality of the SMEFT fit keeping PDF fixed and the
simultaneous SMEFT-PDF fit. We display the $\chi^2$ per datapoint in Tables~\ref{tab:chi2-top-pair},~\ref{tab:chi2-single-top-simu} and ~\ref{tab:chi2-other}
for each dataset appearing in both the simultaneous SMEFT-PDF fit and the fixed PDF SMEFT fit.
The fit quality for inclusive and associated top pair production is shown in Table~\ref{tab:chi2-top-pair},
for inclusive and associated single top production in Table~\ref{tab:chi2-single-top-simu} and
for Higgs, diboson and electroweak precision observables in Table~\ref{tab:chi2-other}.
We also display the total fit quality of the 366 SMEFT-affected datapoints in Table~\ref{tab:chi2-other}.

Overall, we observe that the fit quality of the total dataset remains stable between the SMEFT-PDF
fit and the SMEFT fit, with a total $\chi^2$ of 0.91 for both fits, as shown in Table~\ref{tab:chi2-other}.
This is also observed in the Higgs and electroweak precision observables, while in the diboson sector
a small improvement from $\chi^2 = 1.24$ to $\chi^2 = 1.23$
is observed.
A similar improvement in the $\chi^2$ is observed in the inclusive top quark pair production 
datasets in Tables~\ref{tab:chi2-top-pair} from $\chi^2=1.03$ to $\chi^2=1.01$, and in inclusive single top datasets 
in Tables~\ref{tab:chi2-single-top-simu} from $\chi^2=0.34$ to $\chi^2=0.33$, indicating that
in these sectors, the SMEFT-PDF fit provides a better fit to the data.  This improvement in 
the $\chi^2$ in these sectors is not as significant as the improvement observed in Ref.~\cite{Kassabov:2023hbm},
however.  As discussed below Fig.~\ref{fig:gglumi}, this is due to the inclusion of new high-mass Drell-Yan data in the new fit.

\input{tab-chi2.tex}
\input{tab-chi2-split.tex}
\input{tab-chi2-singletop.tex}
\input{tab-chi2-other.tex}




==> Chapters/SIMUnet/sec-usage.tex <==
\section{Usage and applicability of the code}
\label{sec:usage}
In this section we define the realm of applicability of \simunet{} and summarise a series of caveats that users should be
aware of when using our tool for phenomenological applications.

\begin{itemize}
  %
\item {\bf Truncation of the SMEFT expansion:}
In a simultaneous fit of PDF and SMEFT Wilson coefficients, \simunet{}
only includes the linear SMEFT correction terms of ${\cal O}(1/\Lambda^2)$,
{\it i.e.} the interference between the SM and the SMEFT
amplitudes. The reason why a simultaneous fit of PDF and SMEFT Wilson
coefficients based on the Monte Carlo replica sampling method would
not give faithful confidence intervals for the SMEFT coefficients is
explained in details in Ref.~\cite{Costantini:2024wby}. There it is
shown that the uncertainty estimates of the fitted parameters are discrepant between the Monte Carlo
replica method and a numerical Bayesian method (like for example a
nested sampling approach) beyond linear models.
On the other hand, in the context of 'contaminated' fits
there is no restriction to linearity, as pseudodata can be produced with any BSM model correction (EFT or UV complete). In this case only the PDFs are fitted on pseudo-data that are generated according to a given BSM model,
and linearity around the best-fit of PDF parameters is assumed to be a
good approximation independently of the linearity of the underlying
BSM model.
\vspace*{0.3cm}

%
\item{\bf Analysing flat directions: }
Given a selection of data to include in a fit, it is important to
choose the Wilson coefficients to fit 
such that there are no unconstrained parameters or directions in the fit.  
It is possible to do this using the principal component analysis (PCA) function
available in the \texttt{simunet\_analysis.py} set of analysis tools.

The PCA proceeds as follows.
The covariance between Wilson coefficients $c_i$, $c_j$ is described by the covariance matrix $U_{ij} = (F^{-1})_{ij}$,
where $F$ denotes the Fisher information matrix given in Eq.~\eqref{eq:fisher}.
The Fisher information matrix $F_{ij}$
depends only on the theory predictions $T(c)$ and on the experimental covariance matrix
$\Sigma_{\mathrm{exp}}$, and not on the values of the Wilson coefficients, and can therefore be computed pre-fit
assuming a fixed input PDF set.
The PCA consists of computing the eigenvalues of $F_{ij}$ using a singular value decomposition.  If all eigenvalues are
nonzero, we can conclude that $F$ is an invertible matrix and $U_{ij}$ can be computed, 
implying that all coefficients in the fit will be constrained.
On the other hand, if there are eigenvalues equal to zero, the
combination of parameters leading to these unconstrained directions is indicated by the eigenvectors: these parameters can then be
removed from the fit.
\vspace*{0.3cm}

 %
%%%%%%
  \item {\bf Correlation between PDFs and SMEFT corrections in the
     $K$-factors:}
The SMEFT $K$-factors defined in Eq.~\eqref{eq:gradient_approximation}
are determined with a fixed choice of reference
PDF, given that $\pmb{\omega} = \pmb{\omega}^*$, where they do
actually depend on PDFs freely. In practice however, this
approximation is often justified, as the PDF dependence cancels out to
a good approximation. To verify the level of accuracy of such
approximation, that consists in neglecting the correlation at the
pre-fit level between the SMEFT corrections and the PDFs, one can
recalculate the $K$-factors post-fit, by using as input PDF set the
one coming out of the simultaneous fit and verify that the $K$-factors
are stable, otherwise the user should recompute them recursively until
stability is reached, as it is discussed in App.~C of
Ref.~\cite{Greljo:2021kvv}.
\vspace*{0.3cm}

%%%%%%
\item {\bf Number of replicas: }
Throughout this study we use fits of $N_{\text{rep}} = 1000$ replicas, both in fixed-PDF and in simultaneous fits. 
This ensures that central values, covariance and correlations of
experiments are reproduced to a good accuracy at 1\% level for all experiments. Still, it has been
shown that even $N_{\text{rep}} = 100$ replicas is sufficient to obtain a good estimate of the solutions in the case of relatively few
Wilson coefficients, and adding more replicas causes little change~\cite{Iranipour:2022iak}. If possible, in terms of computational resources,
using $N_{\text{rep}} = 1000$ is the standard to ensure that the results are stable and robust. Increasing the number of Wilson
coefficients in the fit amounts to simply having some more trainable weights in the \simunet{} architecture, and does not really
affect the number of replicas required.
\vspace*{0.3cm}


\item {\bf Choice of scale parameter: }
Choosing appropriate {\tt scale} parameters is important for the optimal performance of the \simunet{} framework, in the same way
that choosing correct learning rates is important for any NN
architecture. As described in Sect.~\ref{sec:codedes}, choosing a {\tt scale} parameter $\lambda$ to fit a Wilson coefficient $c$ amounts to multiplying the associated learning rate by $\frac{1}{\lambda}$, or equivalently, fitting $\lambda c$ instead of $c$. In practice, choosing a small scale gives large steps during the gradient descent which can speed up the convergence but at the risk to probe regions of the parameter space where the $\chi ^2$ is gigantic. This can also create oscillatory-like behaviours toward the end of the fit if the minimum is found for a value of $c$ much smaller than the step. On the other hand, choosing a large scale reduces the risk of probing regions of the parameter space very far from the minimum, provided the initialisation conditions are reasonable. It also reduces the risk of oscillation around the minimum. However, it may slow down the convergence if the fit is initialised far away from the minimum and, in the worst case scenario, it may prevent the fit from converging before the maximum number of allowed iterations is reached.

It is important to note that, usually, the optimal {\tt scale} choice for each Wilson coefficient
is found a posteriori. In practice, it is useful to first launch an
exploratory SMEFT-only fit to obtain a preliminary estimate of the size of
the bounds and central values of the Wilson coefficients, and then use
this information to set the {\tt scale} parameters, which are usually
of $\mathcal{O}(10)$ or smaller, so that the Wilson coefficients is of
 $\mathcal{O}(10)$. 
%
Naturally, it is expected that PDFs and SMEFT coefficients will change in the case of fixed-PDF or simultaneous fits. Depending on the
dataset, the overall fit quality may change very little, but the PDFs can accommodate better the inclusion of new data. In this way, the impact of the
new data on the PDFs is diluted, and the constraining power of the global dataset is also absorbed by the Wilson coefficients.
\end{itemize}

==> Chapters/SIMUnet/tab-chi2-other.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
    \begin{center}
    \renewcommand{\arraystretch}{1.60}
  \small
  \begin{tabular}{ l | c| C{1.4cm} |  C{1.4cm} }
   \toprule
   Dataset & $n_{\rm dat}$   &  \multicolumn{2}{c}{$\chi^2/n_{\rm dat}$}  \\[1.5ex]
    &   & SMEFT-PDF fit & SMEFT fit   \\
   \midrule 
	 ATLAS STXS combination, $\mu_{H}$, 13 TeV & 25 & 0.49 & 0.50 \\
	 ATLAS signal strength $H \rightarrow Z \gamma$, 13 TeV & 1 & 4$\cdot 10^{-5}$ & 3$\cdot 10^{-3}$ \\
	 ATLAS signal strength $H \rightarrow \mu^{+} \mu^{-}$, 13 TeV & 1 & 7$\cdot 10^{-3}$ & 2$\cdot 10^{-3}$ \\
	 CMS signal strength combination, $\mu_{H}$, 13 TeV & 24 & 0.66 & 0.67 \\
	 ATLAS \& CMS signal strength combination, $\mu_{H}$,  7 and 8 TeV & 22 & 0.98 & 0.96 \\
	 \midrule
	 {\bf Total Higgs}  & {\bf 73}  &  {\bf 0.68} &  {\bf 0.68}  \\
	 \midrule
	 \midrule
	 ATLAS $d \sigma _{W^+W^-}/d m_{e \mu}$, 13 TeV & 13 & 1.69 & 1.70 \\
	 ATLAS $d \sigma _{WZ} / d m_{T}$, 13 TeV & 6 & 0.77 & 0.77 \\
	 ATLAS $d \sigma(Zjj)/d \Delta \phi_{jj}$, 13 TeV & 12 & 0.79 & 0.79 \\
	 CMS $d \sigma _{WZ} / d p_{T}$, 13 TeV & 11 & 1.42 & 1.43 \\
	 LEP $d \sigma _{WW} / d cos(\theta _W)$, 0.182 TeV & 10 & 1.39 & 1.39 \\
	 LEP $d \sigma _{WW} / d cos(\theta _W)$, 0.189 TeV & 10 & 0.91 & 0.92 \\
	 LEP $d \sigma _{WW} / d cos(\theta _W)$, 0.198 TeV & 10 & 1.58 & 1.57 \\
         LEP $d \sigma _{WW} / d cos(\theta _W)$, 0.206 TeV & 10 & 1.07 & 1.08 \\
	 \midrule
	  {\bf Total Diboson}  & {\bf 82}  &  {\bf 1.23} &  {\bf 1.24 }  \\
	 \midrule 
	 \midrule
	 LEP $Z$ observables, 0.25 TeV & 19 & 0.52  & 0.52 \\
	 LEP $\mathcal{B}(W \rightarrow l^{-} \bar{v}_l)$ 0.196 TeV & 3 & 2.59 & 2.59 \\
	 LEP $\sigma(e^+ e^- \rightarrow e^+ e^-)$ 0.189 TeV & 21 & 1.02 & 1.03 \\
	 LEP $\hat{\alpha}^{(5)}_{\rm}(M_Z)$ 0.209 TeV & 1 & 0.47 & 0.25 \\
	 \midrule
	 {\bf Total EWPO}  & {\bf 44}  &  {\bf 0.90} &  {\bf 0.90 }  \\
	  \midrule
	  \midrule
	 {\bf Total} & {\bf 366} & {\bf 0.91} & {\bf 0.91} \\
	 \bottomrule
  \end{tabular}
  \end{center}
	\caption{\label{tab:chi2-other}
	Same as Tab.~\ref{tab:chi2-top-pair}, now for the Higgs, diboson and electroweak precision observables.}
  \end{table}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  


==> Chapters/SIMUnet/tab-chi2-singletop.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
    \begin{center}
    \renewcommand{\arraystretch}{1.30}
  \small
  \begin{tabular}{ l | c| C{1.4cm} |  C{1.4cm} }
   \toprule
   Dataset & $n_{\rm dat}$   &  \multicolumn{2}{c}{$\chi^2/n_{\rm dat}$}  \\[1.5ex]
    &   & SMEFT-PDF fit & SMEFT fit   \\
   \midrule 
	  ATLAS $t$-channel $\sigma(t)$, 7 TeV & 1 & 0.24 & 0.26 \\
	  ATLAS $t$-channel $\sigma(\bar{t})$, 7 TeV & 1 & 0.01 & 0.02 \\
	  ATLAS $t$-channel $1/\sigma d\sigma(tq)/dy_t$, 7 TeV & 3 & 0.9 & 0.89 \\
	  ATLAS $t$-channel $1/\sigma d\sigma(\bar{t}q)/dy_{\bar{t}}$, 7 TeV & 3 & 0.06 & 0.06 \\
	  ATLAS $t$-channel $\sigma(t)$, 8 TeV & 1 & 0.01 & 0.02 \\
	  ATLAS $t$-channel $\sigma(\bar{t})$, 8 TeV & 1 & 0.30 & 0.24 \\
	  ATLAS $t$-channel $1/\sigma d\sigma(tq)/dy_t$, 8 TeV & 3 & 0.28 & 0.28 \\
	  ATLAS $t$-channel $1/\sigma d\sigma(\bar{t}q)/dy_{\bar{t}}$, 8 TeV & 3 & 0.19 & 0.20 \\
	  ATLAS $s$-channel $\sigma(t + \bar{t})$, 8 TeV & 1 & 0.02 & 0.04 \\
	  ATLAS $t$-channel $\sigma(t)$, 13 TeV & 1 & 0.31 & 0.32 \\
	  ATLAS $t$-channel $\sigma(\bar{t})$, 13 TeV & 1 & 0.05 & 0.03 \\
	  ATLAS $s$-channel $\sigma(t + \bar{t})$, 13 TeV & 1 & 0.05 & 0.03 \\
          \midrule
	  CMS $t$-channel $\sigma(t) + \sigma(\bar{t})$, 7 TeV & 1 & 0.02 & 0.02 \\
	  CMS $t$-channel $\sigma(t)$, 8 TeV & 1 & 0.34 & 0.31 \\
	  CMS $t$-channel $\sigma(\bar{t})$, 8 TeV & 1 & 0.98 & 1.07 \\
	  CMS $s$-channel $\sigma(t + \bar{t})$, 8 TeV & 1 & 1.42 & 1.45 \\
	  CMS $t$-channel $\sigma(t)$, 13 TeV & 1 & 0.34 & 0.35 \\
	  CMS $t$-channel $\sigma(\bar{t})$, 13 TeV & 1 & 0.02 & 0.03 \\
	  CMS $t$-channel $1/\sigma d\sigma/d|y^{(t)}|$, 13 TeV & 4 & 0.40 & 0.40 \\
         \midrule
	  {\bf Total inclusive single top}  & {\bf 30}  & {\bf 0.33} & {\bf 0.34}  \\
         \midrule
         \midrule
	  ATLAS $\sigma(tW)$, dilepton, 8 TeV & 1 & 0.07 & 0.05 \\
	  ATLAS $\sigma(tW)$, single-lepton, 8 TeV & 1 & 0.35 & 0.32 \\
	  ATLAS $\sigma(tW)$, dilepton, 13 TeV & 1 & 0.74 & 0.71 \\
	  ATLAS $\sigma_{\text{fid}}(tZj)$, dilepton, 13 TeV & 1 & 0.30 & 0.24 \\
	 \midrule
	  CMS $\sigma(tW)$, dilepton, 8 TeV & 1 & 0.08 & 0.07 \\
	  CMS $\sigma(tW)$, dilepton, 13 TeV & 1 & 2.21 & 2.41 \\
	  CMS $\sigma_{\text{fid}}(tZj)$, dilepton, 13 TeV & 1 & 0.13 & 0.17 \\
	  CMS $d\sigma_{\text{fid}}(tZj)/dp_T^{t}$, dilepton, 13 TeV & 3 & 0.13 & 0.14 \\
	  CMS $\sigma(tW)$, single-lepton, 13 TeV & 1 & 1.51 & 1.42 \\
	 \midrule
         {\bf Total associated single top}  & {\bf 11}  &  {\bf 0.53} &  {\bf 0.53}  \\
	 \bottomrule
  \end{tabular}
  \end{center}
    \caption{\label{tab:chi2-single-top-simu}
	Same as Tab.~\ref{tab:chi2-top-pair}, now for inclusive and associated single top datasets.}
  \end{table}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  


==> Chapters/SIMUnet/tab-chi2-split.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
    \begin{center}
    \renewcommand{\arraystretch}{1.60}
  \small
  \begin{tabular}{ l | c| C{1.4cm} |  C{1.4cm} }
   \toprule
   Dataset & $n_{\rm dat}$   &  \multicolumn{2}{c}{$\chi^2/n_{\rm dat}$}  \\[1.5ex]
    &   & SMEFT-PDF fit & SMEFT fit   \\
   \midrule
      ATLAS $\sigma(t\bar{t}Z)$, 8 TeV & 1 & 1.40 & 1.33 \\
      ATLAS $\sigma(t\bar{t}W)$, 8 TeV & 1 & 0.62 & 0.71   \\
      ATLAS $\sigma(t\bar{t}Z)$, 13 TeV & 1 & 2$\cdot 10^{-6}$ & 5$\cdot 10^{-3}$  \\
      ATLAS $1/\sigma d\sigma(t\bar{t}Z)/dp_T^Z$, 13 TeV & 5 & 1.85 & 1.84 \\
      ATLAS $\sigma(t\bar{t}W)$, 13 TeV & 1& 2$\cdot 10^{-2}$ & 4$\cdot 10^{-3}$\\
      \midrule
      ATLAS $\sigma(t\bar{t}\gamma)$, 8 TeV & 1 & 0.33 & 0.29  \\
      \midrule
      CMS $\sigma(t\bar{t}Z)$, 8 TeV & 1 & 2$\cdot 10^{-3}$ & 5$\cdot 10^{-3}$\\
      CMS $\sigma(t\bar{t}W)$, 8 TeV & 1 & 0.69 & 0.78  \\
      CMS $\sigma(t\bar{t}Z)$, 13 TeV & 1& 0.10 & 0.15 \\
      CMS $1/\sigma d\sigma(t\bar{t}Z)/dp_T^Z$, 13 TeV & 3 & 0.86 & 0.88 \\
      CMS $\sigma(t\bar{t}W)$, 13 TeV & 1 & 0.48 & 0.35 \\
      \midrule
      CMS $\sigma(t\bar{t}\gamma)$, 8 TeV & 1 & 0.01 & 7$\cdot 10^{-3}$ \\
      \midrule
     {\bf Total associated $t\bar{t}$}  & {\bf 18}  &  {\bf 0.86} &  {\bf 0.86 }  \\
   \bottomrule
  \end{tabular}
  \end{center}
    \caption{ \label{tab:chi2-top-pair-2}
      Same as Table~\ref{tab:chi2-top-pair} for associate $t\bar{t}$ and vector boson production.
  }
  \end{table}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  


==> Chapters/SIMUnet/tab-chi2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{table}[htbp]
    \begin{center}
    \renewcommand{\arraystretch}{1.4}
    \scriptsize
    \begin{tabular}{ l | c| C{1.2cm} |  C{1.2cm} }
   \toprule
   Dataset & $n_{\rm dat}$   &  \multicolumn{2}{c}{$\chi^2/n_{\rm dat}$}  \\[1ex]
    &   & SMEFT-PDF fit & SMEFT fit   \\
   \midrule
      ATLAS $\sigma(t\bar{t})$, dilepton, 7 TeV    & 1    & 1.87 &  1.84 \\
      ATLAS $\sigma(t\bar{t})$, dilepton, 8 TeV & 1 & 0.33 & 0.35 \\
      ATLAS $1/\sigma d\sigma/dm_{t\bar{t}}$, dilepton, 8 TeV & 5 & 0.30 &  0.30 \\
      ATLAS $\sigma(t\bar{t})$, $\ell+$jets, 8 TeV & 1 & 3$\cdot 10^{-5}$ &  3$\cdot 10^{-4}$ \\
      ATLAS $1/\sigma d\sigma/d|y_t|$, $\ell+$jets, 8 TeV & 4&  1.27 & 1.22 \\
      ATLAS $1/\sigma d\sigma/d|y_{t\bar{t}}|$, $\ell+$jets, 8 TeV & 4 & 2.8 & 2.95  \\
      ATLAS $\sigma(t\bar{t})$, dilepton, 13 TeV           & 1   & 2$\cdot 10^{-3}$ & 2$\cdot 10^{-4}$  \\
      ATLAS $\sigma(t\bar{t})$, hadronic, 13 TeV         & 1    & 0.09 &  0.09   \\
      ATLAS $1/\sigma d^2\sigma/d|y_{t\bar{t}}|dm_{t\bar{t}}$, hadronic, 13 TeV & 10 & 1.84 & 1.88 \\
      ATLAS $\sigma(t\bar{t})$, $\ell+$jets, 13 TeV & 1 & 0.01 & 0.01 \\
      ATLAS $1/\sigma d\sigma/dm_{t\bar{t}}$, $\ell+$jets, 13 TeV & 8 & 2.07 & 2.1  \\
      \midrule
      CMS $\sigma(t\bar{t})$, combined, 5 TeV & 1 & 0.23 &  0.22 \\
      CMS $\sigma(t\bar{t})$, combined, 7 TeV & 1 & 0.01 & 0.01  \\
      CMS $\sigma(t\bar{t})$, combined, 8 TeV & 1 & 0.12 & 0.13  \\
      CMS $1/\sigma d^2\sigma/d|y_{t\bar{t}}|dm_{t\bar{t}}$, dilepton, 8 TeV & 16 & 0.51 & 0.53  \\
      CMS $1/\sigma d\sigma/d|y_{t\bar{t}}|$, $\ell+$jets, 8 TeV & 9  & 0.93 & 0.94  \\
      CMS $\sigma(t\bar{t})$, dilepton, 13 TeV & 1 & 0.60 & 0.62 \\
      CMS $1/\sigma d\sigma/dm_{t\bar{t}}$, dilepton, 13 TeV & 5 & 2.26 & 2.24  \\
      CMS $\sigma(t\bar{t})$, $\ell+$jets, 13 TeV & 1 & 1.90 & 1.98 \\
      CMS $1/\sigma d\sigma/dm_{t\bar{t}}$, $\ell+$jets, 13 TeV & 14& 0.93 & 0.94  \\
      \midrule
      ATLAS charge asymmetry, 8 TeV & 1 & 0.63 & 0.63\\
      ATLAS charge asymmetry, 13 TeV & 5& 0.87 & 0.91 \\
      CMS charge asymmetry, 8 TeV & 3 & 0.06 & 0.06\\
      CMS charge asymmetry, 13 TeV & 3 & 0.39 & 0.36  \\
      ATLAS \& CMS combined charge asy., 8 TeV & 6 & 0.60 & 0.61\\
      \midrule
      ATLAS $W$-hel., 13 TeV & 2 & 7$\cdot 10^{-5}$ &  1$\cdot 10^{-3}$ \\
      ATLAS \& CMS combined $W$-hel., 8 TeV & 2&  0.33 & 0.34  \\
         \midrule
	  {\bf Total inclusive $t\bar{t}$}  & {\bf 108}  & {\bf 1.01}
    & {\bf 1.03}\\
       \bottomrule
    \end{tabular}
    \end{center}
    \caption{\label{tab:chi2-top-pair}
    The values of the $\chi^2$ per data point for the $t\bar{t}$
    production datasets that enter both the SMEFT-only fit and the 
    simultaneous SMEFT-PDF fit. For each dataset, we indicate the number of data points $n_{\rm dat}$ and the 
    $\chi^2$ for the SMEFT-only fit with PDF fixed to the input PDF {\tt NNPDF4.0-notop}  and for the 
    simultaneous SMEFT-PDF determination. 
  }
  \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Chapters/SIMUnet/tab-data-HIGGS.tex <==
\begin{table}[htb!]
    \begin{center}
  {\fontsize{8pt}{8pt}\selectfont
  %\begin{table}[t]
    \centering
     \renewcommand{\arraystretch}{2}
     \setlength{\tabcolsep}{5pt}
     \begin{tabular}{lcccccc}
       \toprule \textbf{Exp.}   & $\bf{\sqrt{s}}$ \textbf{(TeV)}
      &  \textbf{Observable} & $\mathcal{L}$ (fb${}^{-1}$) & $\mathbf{n_{\rm dat}}$ & \textbf{Dataset name}
       &\textbf{Ref.}\\
      \toprule
        \bf{ATLAS and CMS}
        & 7 and 8
        & $\mu_{H \rightarrow \mu^+ \mu^-}$
        & 5 and 20
        & 22
        & ATLAS\_CMS\_SSinc\_RunI
        & \cite{ATLAS:2016neq}\\
      \midrule
        \bf{CMS}
        & 13
        & $\mu_{H}$
        & 35.9
        & 24
        & CMS\_SSINC\_RUNII
        & \cite{CMS:2018uag}\\
      \midrule
        \bf{ATLAS}
        & 13
        & $\mu_{H}$
        & 80
        & 25
        & ATLAS\_STXS\_RUNII
        & \cite{ATLAS:2019nkf}\\
      \midrule
        \bf{ATLAS}
        & 13
        & $\mu_{H \rightarrow Z \gamma}$
        & 139
        & 1
        & ATLAS\_SSINC\_RUNII\_ZGAM
        & \cite{ATLAS:2020qcv}\\
      \midrule
        \bf{ATLAS}
        & 13
        & $\mu_{H \rightarrow \mu^+ \mu^-}$
        & 139
        & 1
        & ATLAS\_SSINC\_RUNII\_MUMU
        & \cite{ATLAS:2020fzp}\\
  
  
  
  \bottomrule
     \end{tabular}
     \vspace{0.3cm}
     \caption{Same as~\ref{tab:dataset_EWPO} for the measurements of the Higgs sector.
      \label{tab:dataset_Higgs}  }
  }
  \end{center}
  \end{table}

==> Chapters/SIMUnet/tab-data-LEP.tex <==
\begin{table}[htb!]
    \begin{center}
  {\fontsize{8pt}{8pt}\selectfont
  %\begin{table}[t]
    \centering
     \renewcommand{\arraystretch}{2}
     \setlength{\tabcolsep}{5pt}
     \begin{tabular}{lcccccc}
       \toprule \textbf{Exp.}   & $\bf{\sqrt{s}}$ \textbf{(TeV)}
      &  \textbf{Observable} & $\mathcal{L}$ (fb${}^{-1}$) & $\mathbf{n_{\rm dat}}$ & \textbf{Dataset name}
       &\textbf{Ref.}\\
      \toprule
        \bf{LEP}
        & 0.250
        & Z observables
        & 
        & 19
        & LEP\_ZDATA
        & \cite{ALEPH:2005ab}\\
      \midrule
        \bf{LEP}
        & 0.196
        & $\mathcal{B}(W \rightarrow l^{-} \bar{v}_l)$
        & 3
        & 3
        & LEP\_BRW
        & \cite{ALEPH:2013dgf}\\
      \midrule
        \bf{LEP}
        & 0.189
        & $\sigma(e^+ e^- \rightarrow e^+ e^-)$
        & 3
        & 21
        & LEP\_BHABHA
        & \cite{ALEPH:2013dgf}\\
      \midrule
        \bf{LEP}
        & 0.209
        & $\hat{\alpha}^{(5)}_{\rm}(M_Z)$
        & 3
        & 1
        & LEP\_ALPHAEW
        & \cite{Workman:2022ynf}\\
  
  \bottomrule
     \end{tabular}
     \vspace{0.3cm}
     \caption{Measurements of electroweak precision observables included in \simunet{}. The columns contain information on the 
     centre-of-mass energy, the observable, the integrated luminosity, the number 
     of data points, the dataset name as implemented in \simunet \ and the source.
      \label{tab:dataset_EWPO}
  }
  }
  \end{center}
  \end{table}
  


==> Chapters/SIMUnet/tab-data-VV.tex <==
\begin{table}[htb!]
    \begin{center}
  {\fontsize{8pt}{8pt}\selectfont
  %\begin{table}[t]
    \centering
     \renewcommand{\arraystretch}{2}
     \setlength{\tabcolsep}{5pt}
     \begin{tabular}{lcccccc}
       \toprule \textbf{Exp.}   & $\bf{\sqrt{s}}$ \textbf{(TeV)}
      &  \textbf{Observable} & $\mathcal{L}$ (fb${}^{-1}$) & $\mathbf{n_{\rm dat}}$ & \textbf{Dataset name}
       &\textbf{Ref.}\\
      \toprule
        \bf{LEP}
        & 0.182
        & $d \sigma _{WW} / d cos(\theta _W)$
        & 0.164
        & 10
        & LEP\_EEWW\_182GEV
        & \cite{ALEPH:2013dgf}\\
      \midrule
        \bf{LEP}
        & 0.189
        & $d \sigma _{WW} / d cos(\theta _W)$
        & 0.588
        & 10
        & LEP\_EEWW\_189GEV
        & \cite{ALEPH:2013dgf}\\
      \midrule
        \bf{LEP}
        & 0.198
        & $d \sigma _{WW} / d cos(\theta _W)$
        & 0.605
        & 10
        & LEP\_EEWW\_198GEV
        & \cite{ALEPH:2013dgf}\\
      \midrule
        \bf{LEP}
        & 0.206
        & $d \sigma _{WW} / d cos(\theta _W)$
        & 0.631
        & 10
        & LEP\_EEWW\_206GEV
        & \cite{ALEPH:2013dgf}\\
      \midrule
        \bf{ATLAS}
        & 13
        & $d \sigma _{W^+W^-}/d m_{e \mu}$
        & 36.1
        & 13
        & ATLAS\_WW\_13TeV\_2016\_MEMU
        & \cite{ATLAS:2019rob}\\
      \midrule
        \bf{ATLAS}
        & 13
        & $d \sigma _{WZ} / d m_{T}$
        & 36.1
        & 6
        & ATLAS\_WZ\_13TeV\_2016\_MTWZ
        & \cite{ATLAS:2019bsc}\\
      \midrule
        \bf{ATLAS}
        & 13
        & $d \sigma(Zjj)/d \Delta \phi_{jj}$
        & 139
        & 12
        & ATLAS\_Zjj\_13TeV\_2016
        & \cite{ATLAS:2020nzk}\\
      \midrule
        \bf{CMS}
        & 13
        & $d \sigma _{WZ} / d p_{T}$
        & 35.9
        & 11
        & CMS\_WZ\_13TeV\_2016\_PTZ
        & \cite{ATLAS:2020nzk}\\
  
  
  
  
  \bottomrule
     \end{tabular}
     \vspace{0.3cm}
     \caption{Same as~\ref{tab:dataset_EWPO} for the measurements of the diboson sector.
      \label{tab:dataset_diboson}
  }
  }
  \end{center}
  \end{table}
  


==> Chapters/Top/tables/chi2_pdfs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
  \begin{center}
  \renewcommand{\arraystretch}{1.20}
%\scriptsize
\tiny
\begin{tabular}{ l | c| C{1.2cm} | C{1.2cm} | C{1.0cm} | C{1.2cm} | C{1.2cm} | C{1.2cm} }
 \toprule
 \multirow{3}{*}{Dataset}    & \multirow{3}{*}{$n_{\rm dat}$}   &  \multicolumn{6}{c}{$\chi^2/n_{\rm dat}$}  \\[1.5ex]
 &   & \multicolumn{3}{c|}{\bf SM-PDF fits} & \multicolumn{2}{c|}{\bf Fixed-PDF EFT fits}   & {\bf SMEFT-PDFs}    \\
  &   & NNPDF4.0 (no top)  & NNPDF4.0 & Fit H & NNPDF4.0 (no top) & Fit H & Joint fit   \\
 \midrule
 \midrule
 SLAC      & 67   & 0.768   & 0.758 & 0.753 & 0.768 & 0.753  & 0.761  \\
 BCDMS   & 581 &  	1.265  & 1.247 & 1.251 & 1.265  & 1.251  & 1.245   \\
 NMC       & 325 & 1.298   & 1.306 & 1.304  & 1.298  & 1.304  & 1.292    \\
 CHORUS  & 832 & 0.899    & 0.900 & 0.901  & 0.899  & 0.901  & 0.898     \\
  NuTeV     & 76  & 0.398 & 0.425  & 0.423 & 0.398  & 0.423  & 0.393    \\
 HERA  & 1208 & 1.204  & 1.203 & 1.204  & 1.204  & 1.204  & 1.200    \\
 \midrule
     {\bf Total DIS}  & {\bf 3089} &  {\bf 1.122 }  & {\bf 1.119 } & {\bf 1.119 } & {\bf 1.122 } & {\bf 1.119 } & {\bf 1.114 } \\
     \midrule
     \midrule
 E886    $\sigma^d_{\rm DY}/\sigma^p_{\rm DY}$ & 15  & 0.527    & 0.524  & 0.536  & 0.527 & 0.536   & 0.544   \\
 E886    $\sigma^p_{\rm DY}$                               & 89  & 1.566  & 1.559  & 1.615  & 1.566 & 1.615  & 1.602   \\
 E605   $\sigma^p_{\rm DY}$                                & 85  & 0.456   & 0.456  & 0.460 & 0.456  & 0.460  & 0.464    \\
 E906   $\sigma^d_{\rm DY}/\sigma^p_{\rm DY}$ &  6  &  0.827   &    0.885  & 0.886   & 0.827 & 0.886  &  0.955    \\
\midrule
{\bf Total fixed-target DY} & {\bf 195} & {\bf 0.981 } & {\bf 0.979 }   & {\bf 1.008 } & {\bf 0.981} & {\bf 1.008 } & {\bf 1.006 }  \\
 \midrule
 \midrule
 CDF    $d\sigma_Z/dy_Z$                                    & 28 &  1.234  & 1.280  &  1.275 & 1.234  & 1.275  & 1.188    \\
 D0     $d\sigma_Z/dy_Z$                                     & 28 &   0.637  & 0.644 &  0.640 & 0.637  & 0.640 & 0.632   \\
 D0    	$W\to \mu \nu$ asy.                       & 9  &   1.958 & 1.929 & 1.905  & 1.958  & 1.905 & 1.641     \\
 \midrule
 ATLAS low-mass DY 7 TeV               & 6 &  0.875  & 0.879 & 0.883  & 0.875  & 0.883 & 0.888    \\
 ATLAS high-mass DY 7 TeV               & 5 & 1.694 & 1.691 & 1.661 & 1.694  & 1.661 & 1.629  \\
 ATLAS $W, Z$ 7 TeV ($\mathcal{L} = 35$ pb${}^{-1}$) & 30   &  1.000 & 0.988 & 1.000 & 1.000 & 1.000  & 0.991    \\
 ATLAS  $W,Z$ 7 TeV ($\mathcal{L} = 4.6$ fb${}^{-1}$) & 61  & 1.689 & 1.686  & 1.685 & 1.685  & 1.685 & 1.599    \\
ATLAS low-mass DY 2D 8 TeV            & 60 & 1.203 &1.216 & 1.225 & 1.203  & 1.225 & 1.207   \\
ATLAS high-mass DY 2D 8 TeV           & 48 & 1.123  & 1.110 & 1.118 & 1.123  & 1.118 & 1.147   \\
ATLAS $\sigma_{W,Z}^{\rm tot}$ 13 TeV    & 3 & 0.727 & 0.778  & 0.706 & 0.727 & 0.706 & 0.471 \\
 \midrule
 CMS $W$ electron asymmetry 7 TeV             & 11 & 0.836 & 0.833 & 0.836 & 0.836 & 0.836 & 0.892   \\
CMS $W$ muon asymmetry 7 TeV              & 11 & 1.728 & 1.714 & 1.733 & 1.728  & 1.733 &  1.699  \\
CMS DY 2D 7 TeV                                        & 110 & 1.367 & 1.361 & 1.353 & 1.367 & 1.353 &  1.339 \\
CMS $W$ rapidity 8 TeV                              & 22 & 1.375 & 1.361 & 1.365 & 1.375  & 1.365 & 1.162  \\
 \midrule
 LHCb $Z \rightarrow ee$ 7 TeV                       & 9  &  1.630  & 1.648 & 1.636 & 1.630 & 1.636 & 1.669 \\
 LHCb $Z \rightarrow ee$ 8 TeV                        & 17  & 1.272   & 1.325 & 1.334 & 1.272 &  1.334 & 1.266 \\
 LHCb  $W,Z \rightarrow \mu$  7 TeV                 & 29  &   2.032 &  1.948 & 1.902 & 2.032 & 1.902 & 1.896   \\
 LHCb  $W,Z \rightarrow \mu$   8 TeV                & 30  & 1.494   & 1.426 & 1.417 & 1.494  & 1.417 & 1.386  \\
  LHCb  $Z \rightarrow ee$   13 TeV                & 15  & 1.701 & 1.726  & 1.717  & 1.701  & 1.717 & 1.640   \\
  LHCb  $Z \rightarrow \mu\mu$   13 TeV                & 16  & 0.970 & 0.993 & 0.978  & 0.970  & 0.978 & 0.928   \\
\midrule
{\bf Total inclusive gauge boson production} & {\bf 548} &  {\bf 1.344}  & {\bf 1.339}  & {\bf 1.335}  & {\bf 1.344}  & {\bf 1.335} & {\bf 1.297}    \\
 \midrule
 \midrule
ATLAS $W^{\pm}+$jet 8 TeV                      & 30 & 0.954 & 0.959 & 0.957  & 0.954  & 0.957 & 0.973 \\
ATLAS $Z$ $p_T$ 8 TeV ($p_T, m_{\ell\ell}$)      & 44 & 0.911 & 0.905 & 0.904 & 0.911 & 0.904 & 0.910 \\
ATLAS $Z$ $p_T$ 8 TeV ($p_T, y_Z$)                 & 48 & 0.909 & 0.898 & 0.896 & 0.909 & 0.896 & 0.924\\
ATLAS incl. jets 8 TeV, $R=0.6$                           & 171 & 0.682 & 0.687 & 0.687 & 0.682  & 0.687 & 0.667  \\
ATLAS dijets 7 TeV, $R=0.6$                               & 90 & 2.184  & 2.149  & 2.125  & 2.184 & 2.125 &. 2.177  \\
ATLAS isolated $\gamma$ prod. 13 TeV             & 53 & 0.811  & 0.763 & 0.753 & 0.811  & 0.753 & 0.813  \\
 \midrule
CMS $Z$ $p_T$ 8 TeV                                 & 28 & 1.447 & 1.401 & 1.407  & 1.447 & 1.407 & 1.473  \\
CMS incl. jets 8 TeV                                     & 185 & 1.140 & 1.183 & 1.200 & 1.140  & 1.200 & 1.118   \\
CMS dijets 7 TeV                                          & 54 & 1.788 & 1.810  & 1.809 & 1.788 & 1.809  & 1.800  \\
 \midrule
     {\bf Total jets, $Z$ $p_T$ and isolated photon}                      & {\bf 703} &  {\bf 1.154}  & {\bf 1.157} & {\bf 1.158}  & {\bf 1.154}  & {\bf 1.158}  & {\bf 1.148}  \\
      \midrule
 \midrule
     {\bf Total non-top data}                      & {\bf 4535} & {\bf 1.148}  &  {\bf 1.145} & {\bf 1.146} & {\bf 1.148} & {\bf 1.146} & {\bf 1.137} \\
 \bottomrule
\end{tabular}
\end{center}
  \caption{\small \label{tab:chi2-baseline} The values of the $\chi^2$ per data point (using the experimental
    definition of Eq.~\eqref{eq:chi2exp}) for key PDF and EFT analyses presented in this work.
    %
    For each dataset, we indicate the number of data points $n_{\rm dat}$
    and the the $\chi^2$ values for {\it i)} three SM-PDF fits:
    \nnpdfnotop, \nnpdf,
    and Fit H in Table~\ref{tab:fit_list} (full top quark dataset);
    {\it ii)} two fixed-PDF EFT fits: one based on \nnpdfnotop as input,
    and the other using Fit H as input; and finally  {\it iii)} the outcome
    of the simultaneous SMEFT-PDF determination.
    %
    Here we restrict ourselves to the non-top datasets considered in this
    analysis, the corresponding results for the top quark observables
    are provided in Tables~\ref{tab:chi2-top} and~\ref{tab:chi2-single-top}.
    %
    We also provide the total $\chi^2$ for separate groups of processes as well
    as for the full non-top dataset.
    %
    The $\chi^2$ values for the \nnpdfnotop fit
    and for the fixed-PDF EFT fit based on \nnpdfnotop are identical,
    since the latter uses only top data as input.
    %
    For the same reason, the entries in the columns for the SM-PDF Fit H
    and the fixed-PDF EFT fits based on Fit H are the same.
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Chapters/Top/tables/chi2_pdfs_single_top.tex <==
\begin{table}[htbp]
  \begin{center}
  \renewcommand{\arraystretch}{1.50}
%\scriptsize
    \tiny
\begin{tabular}{ l | c| C{1.2cm} | C{1.2cm} | C{1.0cm} | C{1.2cm} | C{1.2cm} | C{1.5cm} }
 \toprule
 \multirow{3}{*}{Dataset}    & \multirow{3}{*}{$n_{\rm dat}$}   &  \multicolumn{6}{c}{$\chi^2/n_{\rm dat}$}  \\[1.5ex]
 &   & \multicolumn{3}{c|}{\bf SM-PDF fits} & \multicolumn{2}{c|}{\bf Fixed-PDF EFT fits}   & {\bf SMEFT-PDFs}    \\
  &   & NNPDF4.0 (no top)  & NNPDF4.0 & Fit H & NNPDF4.0 (no top) & Fit H & Joint fit   \\
 \midrule
 \midrule
     ATLAS $t$-channel $\sigma(t)$, 7 TeV & 1 & \textit{0.785} & \textit{0.756} & 0.757 & 0.179 & 0.135 & 0.155  \\
    ATLAS $t$-channel $\sigma(\bar{t})$, 7 TeV & 1 & \textit{0.304}  & \textit{0.296} & 0.282 & 0.003 & 0.005 & 0.004  \\
    ATLAS $t$-channel $1/\sigma d\sigma(tq)/dy_t$, 7 TeV & 3 & \textit{0.909} & 0.959 & 0.971 & 0.885 & 0.946 & 0.900  \\
     ATLAS $t$-channel $1/\sigma d\sigma(\bar{t}q)/dy_{\bar{t}}$, 7 TeV & 3 & \textit{0.061}  & 0.062 & 0.062 & 0.061 & 0.063 & 0.062  \\
     ATLAS $t$-channel $\sigma(t)$, 8 TeV & 1 & \textit{0.795}  & \textit{0.739} & 0.739 & 0.000 & 0.017 & 0.007 \\
     ATLAS $t$-channel $\sigma(\bar{t})$, 8 TeV & 1 & \textit{2.314} & \textit{2.277}  & 2.221 & 0.379 & 0.337 & 0.356  \\
    ATLAS $t$-channel $1/\sigma d\sigma(tq)/dy_t$, 8 TeV & 3 & \textit{0.288} & 0.246 & 0.241 & 0.290 & 0.245 & 0.283  \\
     ATLAS $t$-channel $1/\sigma d\sigma(\bar{t}q)/dy_{\bar{t}}$, 8 TeV & 3 & \textit{0.196} & 0.190 & 0.187 & 0.198 & 0.189 & 0.192  \\
     ATLAS $s$-channel $\sigma(t + \bar{t})$, 8 TeV & 1 & \textit{0.211} & \textit{0.203} & 0.216 & 0.000 & 0.000 & 0.000  \\
    ATLAS $t$-channel $\sigma(t)$, 13 TeV & 1 & \textit{0.738} & \textit{0.722} & 0.720 & 0.261 & 0.224 & 0.235  \\
    ATLAS $t$-channel $\sigma(\bar{t})$, 13 TeV & 1 & \textit{0.400} & \textit{0.393} & 0.384 & 0.057 & 0.050 & 0.051  \\
     ATLAS $s$-channel $\sigma(t + \bar{t})$, 13 TeV & 1 & \textit{0.700} & \textit{0.688} & 0.703 & 0.127 & 0.138 & 0.118  \\
    \midrule
    CMS $t$-channel $\sigma(t) + \sigma(\bar{t})$, 7 TeV & 1 & \textit{0.765}  & 0.729  & 0.719 & 0.010 & 0.001 & 0.004  \\
    CMS $t$-channel $\sigma(t)$, 8 TeV & 1 & \textit{0.010} & \textit{0.006} & 0.005 & 0.487 & 0.628 & 0.566  \\
    CMS $t$-channel $\sigma(\bar{t})$, 8 TeV & 1 & \textit{0.079} & \textit{0.084} & 0.092 & 0.886 & 0.934  & 0.911 \\
    CMS $s$-channel $\sigma(t + \bar{t})$, 8 TeV & 1 & \textit{1.108}  & \textit{1.112} & 1.105 & 1.348 & 1.338 & 1.350 \\
    CMS $t$-channel $\sigma(t)$, 13 TeV & 1 & \textit{0.904} & \textit{0.883} & 0.880 & 0.281 & 0.235 & 0.248  \\
    CMS $t$-channel $\sigma(\bar{t})$, 13 TeV & 1 & \textit{0.136} & \textit{0.132} & 0.125 & 0.010 & 0.014 & 0.013 \\
   CMS $t$-channel $1/\sigma d\sigma/d|y^{(t)}|$, 13 TeV & 4 & \textit{0.412} & \textit{0.387} & 0.383 & 0.405 & 0.378 & 0.396  \\
       \midrule
   {\bf Total single top}  & {\bf 30}  & {\bf 0.509 }  &  {\bf 0.498 } & {\bf 0.495 } & {\bf 0.332 } & {\bf 0.330 } & {\bf 0.331 }  \\
     \midrule
     \midrule
    ATLAS $\sigma(tW)$, dilepton, 8 TeV & 1 & \textit{0.510} & \textit{0.529} & 0.538 & 0.144  & 0.168 & 0.167 \\
    ATLAS $\sigma(tW)$, single-lepton, 8 TeV & 1 & \textit{0.695} & \textit{0.708} & 0.713 & 0.428 & 0.449 & 0.448  \\
    ATLAS $\sigma(tW)$, dilepton, 13 TeV & 1 & \textit{1.150} & \textit{1.149} & 1.148 & 0.840 & 0.847 & 0.849  \\
    ATLAS $\sigma_{\text{fid}}(tZj)$, dilepton, 13 TeV & 1 & \textit{0.115} & \textit{0.115} & \textit{0.115} & 0.871 & 0.611 & 0.795  \\
    \midrule
    CMS $\sigma(tW)$, dilepton, 8 TeV & 1 & \textit{0.359} & \textit{0.371} & 0.376 & 0.134 & 0.150 & 0.149 \\
    CMS $\sigma(tW)$, dilepton, 13 TeV & 1 & \textit{0.434} & \textit{0.437} & 0.438 & 1.612 & 1.573 & 1.563 \\
    CMS $\sigma_{\text{fid}}(tZj)$, dilepton, 13 TeV & 1 & \textit{1.041} & \textit{1.041} & \textit{1.041} & 0.279 & 0.427 & 0.316  \\
    CMS $d\sigma_{\text{fid}}(tZj)/dp_T^{t}$, dilepton, 13 TeV & 3 & \textit{0.362} & \textit{0.362} & \textit{0.362} & 0.130 & 0.156 & 0.134  \\
   CMS $\sigma(tW)$, single-lepton, 13 TeV & 1 & \textit{2.837} & \textit{2.833} & 2.832 & 1.817 & 1.839 & 1.846  \\
    \midrule
   {\bf Total associated single top}  & {\bf 11}  & {\bf 0.748 }  & {\bf 0.752 } &  {\bf 0.753 }  & {\bf 0.592 } & {\bf 0.594 } & {\bf 0.594 } \\
     \midrule
     \midrule
   {\bf Total top}  & {\bf 175}  & {\bf 1.370}   & {\bf 1.139} & {\bf 1.102} & {\bf 0.868} & {\bf 0.839} & {\bf 0.848}    \\
     \midrule
     \midrule
     {\bf Total dataset}   &  {\bf 4710} & {\bf 1.156}  & {\bf 1.145} & {\bf 1.144} & {\bf 1.138} & {\bf 1.135} & {\bf 1.126}  \\
 \bottomrule
\end{tabular}
\end{center}
  \caption{\small \label{tab:chi2-single-top}
     Same as Table~\ref{tab:chi2-top} now
    for the  inclusive and associated single-top production datasets.
    %
    Values in italics indicate datasets 
    that do not enter the corresponding fits: for those processes,
    we evaluate a posteriori the physical observables and the associated
    $\chi^2$ values using the resulting PDFs from the fit.
    %
    The last row indicates the total values adding together the non-top
    and top data contributions to the $\chi^2$,
    and the next-to-last row the total top quark contribution.
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Chapters/Top/tables/chi2_pdfs_top.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
  \begin{center}
  \renewcommand{\arraystretch}{1.30}
%\scriptsize
  \tiny
\begin{tabular}{ l | c| C{1.2cm} | C{1.2cm} | C{0.8cm} | C{1.2cm} | C{1.0cm} | C{1.2cm} }
 \toprule
 \multirow{3}{*}{Dataset}    & \multirow{3}{*}{$n_{\rm dat}$}   &  \multicolumn{6}{c}{$\chi^2/n_{\rm dat}$}  \\[1.5ex]
 &   & \multicolumn{3}{c|}{\bf SM-PDF fits} & \multicolumn{2}{c|}{\bf Fixed-PDF EFT fits}   & {\bf SMEFT-PDFs}    \\
  &   & NNPDF4.0 (no top)  & NNPDF4.0 & Fit H & NNPDF4.0 (no top) & Fit H & Joint fit   \\
 \midrule
 \midrule
    ATLAS $\sigma(t\bar{t})$, dilepton, 7 TeV    & 1    &   \textit{4.100}  & 4.540 & 4.599 & 1.733 & 1.824 & 1.974     \\
    ATLAS $\sigma(t\bar{t})$, dilepton, 8 TeV & 1 & \textit{0.005} & 0.021 & 0.023 & 0.405 & 0.382 & 0.307 \\
    ATLAS $1/\sigma d\sigma/dm_{t\bar{t}}$, dilepton, 8 TeV & 5 & \textit{0.262} & \textit{0.284} & 0.291 & 0.305 & 0.309 & 0.310  \\
    ATLAS $\sigma(t\bar{t})$, $\ell+$jets, 8 TeV & 1 & \textit{0.218} & \textit{0.270} & 0.277 & 0.002 & 0.001  & 0.000  \\
    ATLAS $1/\sigma d\sigma/d|y_t|$, $\ell+$jets, 8 TeV & 4 & \textit{6.266} & 3.219 & 2.827 & 1.178 & 1.021 & 1.144 \\
    ATLAS $1/\sigma d\sigma/d|y_{t\bar{t}}|$, $\ell+$jets, 8 TeV & 4 & \textit{7.978} & 3.725 & 3.332 & 2.883 & 2.105 & 2.646  \\
    ATLAS $\sigma(t\bar{t})$, dilepton, 13 TeV           & 1    &  \textit{1.388}  & \textit{1.397}  & 1.374 & 0.004 & 0.004 & 0.002    \\
    ATLAS $\sigma(t\bar{t})$, hadronic, 13 TeV         & 1    & \textit{0.231}   &  \textit{0.231} & 0.230 & 0.082 & 0.082  & 0.092    \\
    ATLAS $1/\sigma d^2\sigma/d|y_{t\bar{t}}|dm_{t\bar{t}}$, hadronic, 13 TeV & 10 & \textit{2.276}  & \textit{2.007}  & 1.928 & 1.915 & 1.824 & 1.857  \\
    ATLAS $\sigma(t\bar{t})$, $\ell+$jets, 13 TeV & 1 & \textit{0.489} & 0.492 & 0.485 & 0.004 & 0.004 & 0.013 \\
    ATLAS $1/\sigma d\sigma/dm_{t\bar{t}}$, $\ell+$jets, 13 TeV & 8 & \textit{1.607} & \textit{1.788}  & 1.835 & 2.087 & 2.072 & 2.090  \\
    \midrule
    CMS $\sigma(t\bar{t})$, combined, 5 TeV & 1 & \textit{0.442}  & 0.542 & 0.555 & 0.211 & 0.236 & 0.239  \\
    CMS $\sigma(t\bar{t})$, combined, 7 TeV & 1 & \textit{0.795} & 1.032 & 1.065 & 0.004 & 0.010 & 0.027  \\
    CMS $\sigma(t\bar{t})$, combined, 8 TeV & 1 & \textit{0.170} & 0.247 & 0.258 & 0.174 & 0.156 & 0.103  \\
    CMS $1/\sigma d^2\sigma/d|y_{t\bar{t}}|dm_{t\bar{t}}$, dilepton, 8 TeV & 16 & \textit{1.094}  & \textit{0.994} & 0.963  & 0.519 & 0.580 & 0.514  \\
    CMS $1/\sigma d\sigma/d|y_{t\bar{t}}|$, $\ell+$jets, 8 TeV & 9 & \textit{2.127} &1.245 & 1.131 & 0.928 & 0.995 & 0.935  \\
    CMS $\sigma(t\bar{t})$, dilepton, 13 TeV & 1 & \textit{0.064}  & 0.063 & 0.066 & 0.680 & 0.680 & 0.600  \\
    CMS $1/\sigma d\sigma/dm_{t\bar{t}}$, dilepton, 13 TeV & 5 & \textit{2.760}  & 2.550 & 2.485 & 2.246 & 2.232 & 2.194  \\
    CMS $\sigma(t\bar{t})$, $\ell+$jets, 13 TeV & 1 & \textit{0.230} & \textit{0.227} & 0.234 & 2.153 & 2.155  & 1.907  \\
    CMS $1/\sigma d\sigma/dm_{t\bar{t}}$, $\ell+$jets, 13 TeV & 14 & \textit{1.829}  & \textit{1.481} & 1.393 & 0.962 & 0.911 & 0.912  \\
    \midrule
    ATLAS charge asymmetry, 8 TeV & 1 & \textit{0.679}  & \textit{0.678} & 0.675 & 0.567 & 0.587 & 0.571 \\
    ATLAS charge asymmetry, 13 TeV & 5 & \textit{1.012} & \textit{0.997} & 0.989 & 0.872 & 0.786 & 0.836 \\
    CMS charge asymmetry, 8 TeV & 3 & \textit{0.052} & \textit{0.052} & 0.053 & 0.072 & 0.069  & 0.071\\
    CMS charge asymmetry, 13 TeV & 3 & \textit{0.277} & \textit{0.283} & 0.286 & 0.443 & 0.510 & 0.451  \\
    ATLAS \& CMS combined charge asy., 8 TeV & 6 & \textit{0.603}  &\textit{0.602} & 0.602 & 0.646 & 0.659 & 0.651  \\
    \midrule
    ATLAS $W$-hel., 13 TeV & 2 & \textit{0.370} & \textit{0.370} & \textit{0.370} & 0.037 & 0.037 & 0.038   \\
    ATLAS \& CMS combined $W$-hel., 8 TeV & 2 & \textit{1.046} & \textit{1.046} & \textit{1.046} & 0.853 & 0.853 & 0.854  \\
       \midrule
   {\bf Total inclusive $t\bar{t}$}  & {\bf 108}  &  {\bf 1.700 } &  {\bf 1.328 } & {\bf 1.271 } & {\bf 1.032 } & {\bf 0.994} & {\bf 1.002 }  \\
     \midrule
     \midrule
    ATLAS $\sigma(t\bar{t}Z)$, 8 TeV & 1 & \textit{0.264}  &   \textit{0.232}  & 0.235 & 1.331 & 1.161 & 1.258 \\
    ATLAS $\sigma(t\bar{t}W)$, 8 TeV & 1 &  \textit{2.461} &  \textit{2.482} & 2.430 & 0.751 & 0.708 & 0.722   \\
    ATLAS $\sigma(t\bar{t}Z)$, 13 TeV & 1 &  \textit{0.702} &  \textit{0.747} & 0.742 & 0.001 & 0.000 & 0.000  \\
    ATLAS $1/\sigma d\sigma(t\bar{t}Z)/dp_T^Z$, 13 TeV & 5 &  \textit{1.961}  &  \textit{1.940} & 1.933 & 1.870 & 1.840 & 1.860  \\
    ATLAS $\sigma(t\bar{t}W)$, 13 TeV & 1 &  \textit{1.436} &  \textit{1.456} & 1.417 & 0.000 & 0.002 & 0.000 \\
    \midrule
    ATLAS $\sigma(t\bar{t}\gamma)$, 8 TeV & 1 & \textit{0.426} & \textit{0.426} & \textit{0.426} & 0.037 & 0.009 & 0.034  \\
    \midrule
    ATLAS $\sigma(t\bar{t}t\bar{t})$, multi-lepton, 13 TeV & 1 & \textit{3.655} & \textit{3.655} & \textit{3.655} & 4.289 & 3.784 & 4.145  \\
    ATLAS $\sigma(t\bar{t}t\bar{t})$, single lepton, 13 TeV & 1 & \textit{0.872} & \textit{0.872} & \textit{0.872} & 0.997 & 0.898 & 0.969  \\
    ATLAS $\sigma(t\bar{t}b\bar{b})$, $\ell+$jets, 13 TeV & 1 & \textit{2.062} & \textit{2.062} & \textit{2.062} & 1.093 & 1.316 & 1.152  \\
       \midrule
    CMS $\sigma(t\bar{t}Z)$, 8 TeV & 1 &  \textit{0.432}  &  \textit{0.470} & 0.466 & 0.005 & 0.020 & 0.010 \\
    CMS $\sigma(t\bar{t}W)$, 8 TeV & 1 &  \textit{2.281}  &  \textit{2.298} & 2.255 & 0.808 & 0.770 & 0.783  \\
    CMS $\sigma(t\bar{t}Z)$, 13 TeV & 1 &  \textit{1.185}  &  \textit{1.238} & 1.233 & 0.085 & 0.113 & 0.110 \\
    CMS $1/\sigma d\sigma(t\bar{t}Z)/dp_T^Z$, 13 TeV & 3 &  \textit{0.628}  &  \textit{0.598} & 0.590 & 0.936 & 0.756 & 0.898 \\
    CMS $\sigma(t\bar{t}W)$, 13 TeV & 1 &  \textit{0.667} &  \textit{0.682} & 0.652 & 0.297 & 0.329 & 0.307  \\
    \midrule
    CMS $\sigma(t\bar{t}\gamma)$, 8 TeV & 1 & \textit{0.508} & \textit{0.508} & \textit{0.508} & 0.022 & 0.045 & 0.024 \\
    \midrule
    CMS $\sigma(t\bar{t}t\bar{t})$, multi-lepton, 13 TeV & 1 & \textit{0.027} & \textit{0.027} & \textit{0.027} & 0.124 & 0.041 & 0.096  \\
    CMS $\sigma(t\bar{t}t\bar{t})$, single lepton, 13 TeV & 1 & \textit{0.231} & \textit{0.231} & \textit{0.231} & 0.262 & 0.238 & 0.255 \\
    CMS $\sigma(t\bar{t}b\bar{b})$, all-jet, 13 TeV & 1 & \textit{1.878} & \textit{1.878} & \textit{1.878} & 1.334 & 1.466 & 1.369  \\
    CMS $\sigma(t\bar{t}b\bar{b})$, dilepton, 13 TeV & 1 & \textit{0.962} & \textit{0.962} & \textit{0.962} & 0.312 & 0.447 & 0.347  \\
    CMS $\sigma(t\bar{t}b\bar{b})$, $\ell+$jets, 13 TeV & 1 & \textit{0.900} & \textit{0.900} & \textit{0.900} & 0.135 & 0.269 & 0.167  \\
    \midrule
   {\bf Total associated $t\bar{t}$}  & {\bf 26}  &  {\bf 1.255 } &  {\bf 1.255 } & {\bf 1.246 } & {\bf 0.925 } & {\bf 0.888 } & {\bf 0.913 } \\
%     \midrule
%     \midrule
%   {\bf Total top}  & {\bf 260}  &   &    \\
%     \midrule
%     \midrule
%     {\bf Grand total across all non-top \& top data}   &  {\bf 4022} & 1.1623  & 1.1627  \\
 \bottomrule
\end{tabular}
\end{center}
  \caption{\small \label{tab:chi2-top}
    Same as Table~\ref{tab:chi2-baseline} now
    for the  inclusive and associated $t\bar{t}$ production datasets.
    %
     Values in italics indicate datasets 
    that do not enter the corresponding SM-PDF fit: for those processes,
    we evaluate a posteriori the physical observables and the associated
    $\chi^2$ values using the resulting PDFs from the fit.
    %
    For instance, top data is removed from the \nnpdfnotop,
    and for some top quark observables like $t\bar{t}t\bar{t}$ their
    PDF dependence is neglected.
    %
      The last row indicates the total values adding together the non-top
    and top data contributions to the $\chi^2$.
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Chapters/Top/tables/table-input-dataset-top4b.tex <==
\begin{table}[h!]
{\fontsize{7pt}{7pt}\selectfont
%\begin{table}[t]
  \centering
   \renewcommand{\arraystretch}{2}
   \setlength{\tabcolsep}{5pt}
   \begin{tabular}{lcccc|c}
     \toprule \textbf{Experiment}     & $\bf{\sqrt{s}}$\textbf{(TeV)}
     &  \textbf{Observable} & $\mathbf{n_{\rm dat}}$ & \textbf{Ref.}   
    &  \textbf{New (SMEFT fits)} \\
    \toprule
      ATLAS
      & 13
      & $\sigma_{\text{fid}}(tl^+l^-q)$
      & 1
      & \cite{Aad:2020wog}
      & \\
%-------------------------------------------------------------------------------
     \midrule
      CMS
      & 13
      & $\sigma_{\text{fid}}(tl^+l^-q)$
      & 1
      & \cite{Sirunyan:2018zgs}
      & \\
%-------------------------------------------------------------------------------
      & 
      & $d\sigma_{\text{fid}}(tZq)/dp_T(Z)$ or $d\sigma_{\text{fid}}(tZq)/dp_T(t)$
      & 4 or 3
      & \cite{CMS:2021rvz}
      & $\checkmark$\\
\bottomrule
  \end{tabular}
  \caption{\small Same as Table~\ref{tab:input_datasets_toppair} for all the single-top production in association with a $Z$-boson included in this analysis.
     \label{tab:input_datasets_4b}
}
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Chapters/appendices/contamination/tables/tab_chi2_w8.tex <==
\begin{table}[t]
        \tiny
        \centering
        \begin{tabular}{lc|c|c|c|c|c|}
                \toprule
       & & \multicolumn{2}{c}{SM} & \multicolumn{2}{c}{$W=8\cdot 10^{-5}$}\\
          \midrule
       Dataset  & $n_{\rm dat}$ & $\chi^2$ &  $n_\sigma$ & $\chi^2$ & $n_\sigma$ \\
          \midrule
 NMC $F^d_2/F^p_2$         & 121 & 0.90 & -0.78 & 0.94 &-0.47 \\
 NMC $\sigma^{\rm NC,p}$ & 204 & 0.93 & -0.71 & 0.93 &-0.71 \\
 SLAC $F^p_2$                   & 33 & 0.52 & -1.95 & 0.55 & -1.83 \\
SLAC $F^d_2$                   & 34 & 1.12 & +0.49 &  1.12 & +0.49 \\
BCDMS $F^p_2$                & 333 & 1.04 & +0.51 &1.03 &+0.39 \\
BCDMS $F^d_2$                & 248 & 0.93 & -0.78 & 0.93 &-0.78 \\
CHORUS $\sigma^\nu_{\rm CC}$ & 416 & 0.98 &-0.28&0.98 &-0.28 \\
CHORUS $\sigma^{\bar\nu}_{\rm CC}$& 416 & 0.95 &-0.72&0.95 &-0.72 \\
NuTeV $\sigma^\nu_{\rm CC}$ (dimuon) & 39 & 0.85 &-0.66& 0.87 &-0.57 \\
NuTeV $\sigma^{\bar\nu}_{\rm CC}$ (dimuon) & 37 & 0.48&-2.23& 0.59&-1.76 \\
                    \midrule
HERA I+II $\sigma^p_{\rm NC} e^-$ & 159 & 1.01&+0.09& 1.02&+0.18 \\
HERA I+II $\sigma^p_{\rm NC} e^+$ (460 GeV) & 204 &0.95&-0.51& 0.95&-0.51 \\
HERA I+II $\sigma^p_{\rm NC} e^+$ (575 GeV) & 254 &1.12 &+1.35&1.12 &+1.35 \\
HERA I+II $\sigma^p_{\rm NC} e^+$ (820 GeV) & 70 &0.89 &-0.65&0.90 &-0.59 \\
HERA I+II $\sigma^p_{\rm NC} e^+$ (920 GeV) & 377 & 0.94&-0.82&0.95 &-0.69 \\
          HERA I+II $\sigma^p_{\rm CC} e^+$ & 42 & 1.22&+1.01&1.22 &+1.01 \\
          HERA I+II $\sigma^p_{\rm CC} e^+$ & 39 & 1.06 &+0.26&1.03 &+0.13\\
          HERA I+II $\sigma^c_{\rm NC}$    & 37 & 0.83 &-0.73&0.84 &-0.69 \\
         HERA I+II $\sigma^b_{\rm NC}$     & 26 & 1.15 &+0.54&1.15&+0.54 \\
                \midrule
                \textbf{Total DIS} & \textbf{3089} & \textbf{0.98} &-0.79&\textbf{0.98} & -0.79 \\
                \midrule
           E886 \(\sigma^p\) (NuSea) & 89 & 1.02&+0.13&0.97 &-0.20 \\
           E886 \(\sigma^{d}/2\sigma^p\) (NuSea) & 15 & 1.17 &+0.46& 1.42&+1.15 \\
           E605 \(\sigma^p\) & 85 & 0.38&-4.04 &0.37 & -4.11\\
           E906 \(\sigma^{d}/2\sigma^p\) (SeaQuest) & 6 & 0.59&-0.71&0.67 &-0.57 \\
          \midrule
           CDF $Z$ differential & 28 & 1.02 &+0.07&1.00 &+0.00\\
           D0  $Z$ differential & 28 & 0.98 &-0.07& 1.00&+0.00\\
           D0  $W$ muon asymmetry & 9 &1.23 &+0.48&1.48 &+1.02\\
                \midrule
         ATLAS low-mass DY 7\,TeV & 6 &1.21 &+0.36&1.21 &+0.36 \\
         ATLAS \(W, Z\) 7 TeV (${\cal L}=35\,{\rm pb}^{-1}$) & 30 & 0.78&-0.85& 0.78&-0.85 \\
         ATLAS \(W, Z\) 7 TeV (${\cal L}=4.6\,{\rm fb}^{-1}$) central& 46 & 1.39&+1.87& 1.44&+2.11\\
         ATLAS \(W, Z\) 7 TeV (${\cal L}=4.6\,{\rm fb}^{-1}$) forward&15 & 0.91&-0.25& 0.92&-0.22 \\
         ATLAS low-mass DY 2D 8 TeV&60 & 0.87&-0.71& 0.86&-0.77 \\
        ATLAS $\sigma^{\rm tot}_{W,Z}$13 TeV & 3 &0.38 &-0.76&0.40&-0.73 \\
        ATLAS $W^+$+jet 8 TeV   &15&1.26&+0.71 &1.24 &+0.66 \\       
        ATLAS $W^-$ +jet 8 TeV   &15&1.02&+0.05 &0.98 &-0.05 \\       

          ATLAS $Z$ $p_T$ 8 TeV $(p_T , m_{ll})$& 44 &0.91 &-0.42&0.91 &-0.42 \\
          ATLAS $Z$ $p_T$ 8 TeV $(p_T , y_Z)$ & 48 &0.70 &-1.47&0.68 &-1.57 \\
                \midrule
CMS $W$ electron asymmetry 7 TeV & 11 &1.48&+1.13&1.50 &+1.17 \\
CMS $W$ muon asymmetry 7 TeV & 11 &1.22 &+0.52&1.28 &+0.66 \\
CMS $W$ rapidity 8 TeV& 22 &1.36 &+1.19& 1.37&+1.23 \\
 CMS  \(Z_{p_T}\) 8 TeV  & 28 &0.83&-0.64&0.82&-0.67\\
                \midrule
LHCb \(Z\rightarrow ee\)  7\,TeV & 9 &0.69&-0.66&0.69&-0.66 \\
LHCb \(W,Z\rightarrow\mu\) 7\,TeV & 29 &0.99&-0.04&0.94&-0.23 \\
LHCb \(Z\rightarrow ee\)  8\,TeV &17  &1.24&+0.70&1.24&+0.70 \\
LHCb \(W,Z\rightarrow\mu\) 8\,TeV &30&0.85&-0.58&0.74&-1.0\\
LHCb \(Z\rightarrow ee\)  13\,TeV & 15 &1.58&+1.59&1.60&+1.64 \\
LHCb \(Z\rightarrow\mu\) 13\,TeV & 16 &1.36&+1.02&1.37&+1.05 \\
                \midrule
                \textbf{Total DY (excl. HM)} & \textbf{670} & \textbf{xx} & \textbf{xx}& & \\
                \midrule
                ATLAS high-mass DY 7 TeV (${\cal L}=49\,{\rm fb}^{-1}$)& 13 &0.40 &-1.53& 0.40&-1.53 \\
                ATLAS high-mass DY 2D 8 TeV & 46 & 0.94&-0.29&0.94&-0.29 \\
                CMS high-mass DY 2D 7 TeV & 117 &0.92&-0.61&0.92&-0.61 \\
                CMS high-mass DY 8 TeV & 41 &1.30 &+1.36&1.29 &+1.31 \\
                CMS high-mass DY 13 TeV & 43 &1.06 &+0.28&1.07 &+0.32 \\
                \midrule
                \textbf{Total DY (HM only)} & \textbf{260} & \textbf{xx} & \textbf{xx}& & \\
                \midrule
%                \textbf{Total (excl. HL-LHC)} & \textbf{4715} & \textbf{xx} & \textbf{xx}& & \\
%                \midrule
                HL-LHC CC \(e\)& 16 & 0.79 &-0.60 & 1.00 & +0.0 \\ %% SM vs  Wcont   | Wcont vs SM
                HL-LHC CC \(\mu\)& 16 & 0.55 & -1.27 & 0.74 & -0.74\\
                HL-LHC NC \(e\)& 12 & 1.63 & +1.54 & 1.61 &+1.49 \\
                HL-LHC NC \(\mu\)& 12 & 0.81 &-0.46 & 0.79 &-0.51  \\
                \midrule
                \textbf{Total HL-LHC only} & \textbf{56} &\textbf{0.92} &-0.42 & \textbf{1.03} &+0.16 \\
                \midrule
                \textbf{Total} & \textbf{4771} & \textbf{0.97} & -1.41 & \textbf{0.96} &-1.89 \\
                \bottomrule
        \end{tabular}
        \caption{Values of the \(\chi^2\) per data point across all datasets
        used in this study. We tabulate values for the baseline PDF set as well
        as those obtained in the contaminated PDF fit. \label{tab:chi2w000008}}
\end{table}


==> Chapters/appendices/contamination/tables/tab_chi2_weighted.tex <==
\begin{table}[t]
        \tiny
        \centering
        \begin{tabular}{lc|c|c|c|c|c|}
                \toprule
       & & \multicolumn{2}{c}{SM} & \multicolumn{2}{c}{$W=8\cdot 10^{-5}$}\\
          \midrule
       Dataset  & $n_{\rm dat}$ & $\chi^2$  & $\chi^2$ (weighted) & $\chi^2$ & $\chi^2$ (weighted) \\
          \midrule
           E866 (NuSea) & 89 & 0.80 & 0.81 & 0.98 & 1.14 \\
           D0  $W$ muon asymmetry & 9 & 2.38 & 2.76 & 3.05  & 3.82\\
         ATLAS \(W, Z\) 7 TeV (${\cal L}=4.6\,{\rm fb}^{-1}$) central & 46 & 0.81 & 0.82 & 0.82 & 0.82\\
         ATLAS \(W, Z\) 7 TeV (${\cal L}=4.6\,{\rm fb}^{-1}$) forward & 15 & 1.82 & 1.80 & 1.81 & 1.80 \\
%                \midrule
%                ATLAS high-mass DY 7 TeV (${\cal L}=49\,{\rm fb}^{-1}$)& 13 & 0.85  & 0.85 & 0.87 & 0.84 \\
%                ATLAS high-mass DY 2D 8 TeV & 46 & 0.86 & 0.85 & 0.88 & 0.86 \\
%                CMS high-mass DY 2D 7 TeV & 117 & 0.90 & 0.90 & 0.91 & 0.90 \\
%                CMS high-mass DY 8 TeV & 41 & 0.84 & 0.84 & 0.85 & 0.84 \\
%                CMS high-mass DY 13 TeV & 43 & 1.12 & 1.12 &1.13 & 1.13 \\
                \midrule
                HL-LHC NC \(e\)& 16 & 1.98 & 1.79 & 2.21 & 1.83 \\
                HL-LHC NC \(\mu\)& 16 & 1.10 & 1.04 & 1.17 & 1.05\\
                HL-LHC CC \(e\)& 12 & 0.75 & 0.74 & 1.14 & 0.77\\
                HL-LHC CC \(\mu\)& 12 & 0.65 & 0.64 & 1.16 & 0.63  \\
                \midrule
                \textbf{Total} & \textbf{4771} & \textbf{0.97} & -1.41 & \textbf{0.96} &-1.89 \\
                \bottomrule
        \end{tabular}
        \caption{\label{tab:chi2weighted} Values of the \(\chi^2\) per data point  in the baseline and in the $\hat{W}=8\cdot 10^{-5}$ contaminated fit 
        in the regular fit and in a weighted fit in which high-mass Drell-Yan data are given a larger weight according to Eq.~\eqref{eq:wgts}.}
\end{table}

==> Chapters/appendices/smeft_dglap/app-notation.tex <==
\section{Notation}
\label{app-notation}

In QCD the $\beta$ function is given by
\begin{equation}
\label{eq:beta}
\beta(\alpha_S) = -b \alpha_S^2 (1 + b^{\prime}\alpha_S + b^{\prime \prime} \alpha_S^2 + \mathcal{O}(\alpha_S^3)), 
\end{equation}
where the coefficients are given by 
\begin{align}
    b &= \frac{33-2 n_f}{12 \pi}, \\
    b^{\prime} &= \frac{153 - 19 n_f}{2 \pi (33 -2 n_f)}, \\
    b^{\prime\prime} &= \frac{77139 - 15099 n_f + 325 n_f^2}{288 \pi^2 (33 - 2 n_f)},   
\end{align}
where $n_f$ is the number of active flavours at the energy scale $\mu$, and the first, second, and third terms on the right-hand side of Eq. (\ref{eq:beta}) represent respectively the $1$-loop, $2$-loop, and $3$-loop corrections.

The leading-order QCD splitting functions are given by
%
\begin{equation}
\label{eq:sm_P}
\begin{aligned}
    P_{qq}(z) &= C_F \left(\frac{1+z^2}{(1-z)_+} + \frac{3}{2}\delta(1-z) \right), \\
    P_{gq}(z) &= C_F \left(\frac{1+(1-z)^2}{z} \right), \\
    P_{qg}(z) &= T_F (z^2 + (1-z)^2),\\
    P_{gg}(z) &= 2 C_A \left( \frac{z}{(1-z)_+} + \frac{1-z}{z} + z(1-z)\right) + \left( \frac{11 C_A}{6} - \frac{2}{3}T_F n_f  \right) \delta(1-z), 
\end{aligned}
\end{equation}
%
where $C_F = 4/3$, $T_F=1/2$, $C_A = 3$, and the plus distribution for any smooth function $f(x)$ satisfies 
%
\begin{equation*}
    \int_{0}^{1} \frac{f(x)}{(1-x)_{+}} dx = \int_{0}^{1} \frac{f(x) - f(1)}{1-x} dx. 
\end{equation*}

==> Chapters/appendices/sr/app_denoising.tex <==
\section{Selection criteria and denoising}
\label{app:denoising}

PySR has three selection criteria options:
%
\begin{itemize}
    \item \texttt{accuracy}: selects the candidate model with the lowest loss.
    \item \texttt{best}: selects the candidate model with the highest score among expressions with a loss better than at least $1.5x$ the most accurate model. This is the default criterion.
    \item \texttt{score}: selects the candidate model with the highest score, defined as the negated derivative of the log-loss with respect to complexity.
\end{itemize}
%

Additionally, PySR has a denoising feature which can perform an optional preprocessing step that refines the input data using a Gaussian process with an adaptable kernel. This kernel is a composite of a Gaussian function for smoothing, a white noise component to address inherent noise, and a constant kernel to adjust the mean of the Gaussian process. The Gaussian process then provides denoised target values for each data point, which PySR then fits.

We can use the events of subsection \ref{subsec:l1} to evaluate the results that we obtain with the denoising feature. We show the equations that we obtain with PySR, according to the denoising options and the three  selection criteria, in tables \ref{tab:10bins}, \ref{tab:30bins}, and \ref{tab:100bins}, for 10, 30, and 100 bins, respectively. We see that, in general, the denoising Gaussian process leads to more convolved equations that miss the real distribution. Not using the denoising tends to lead to better performance. It is worth noting, however, that PySR can deal with noisy data in different ways. One alternative is to use a weighted loss that accounts for the uncertainty in each target value. 

\begin{table}[h]
\begin{center}
\begin{tabular}{@{}cl|l|l@{}}
\toprule
Denoise & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Best} & \multicolumn{1}{c}{Score} \\
\midrule
True & 
\begin{minipage}[t]{0.25\columnwidth}$0.0007090032 \cdot x_{0} + 9090.917$\end{minipage} & 
\begin{minipage}[t]{0.25\columnwidth}$9090.844 \cdot x_{0} \cdot (9.63109 \cdot 10^{-5} - 7.7957055 \cdot 10^{-5} \cdot x_{0}) \cdot (x_{0} - 0.22291435) + 9090.844$\end{minipage} & 
\begin{minipage}[t]{0.25\columnwidth}$0.20396256 \cdot x_{0} + 9090.812$\end{minipage} \\
\noalign{\smallskip} \hline \noalign{\smallskip}
False & 
\begin{minipage}[t]{0.25\columnwidth}$x_{0}^{2} \cdot (296.52358194355 \cdot x_{0}^{4} + 7046.0674) + 7613.42$\end{minipage} & 
\begin{minipage}[t]{0.25\columnwidth}$7250.1396 \cdot x_{0}^{2} + 7589.319$\end{minipage} & 
\begin{minipage}[t]{0.25\columnwidth}$7250.1396 \cdot x_{0}^{2} + 7589.319$\end{minipage} \\
\bottomrule
\end{tabular}
\caption{SR results for 10 bins.}
\label{tab:10bins}
\end{center}
\end{table}

\begin{table}[h]
\begin{center}
\begin{tabular}{@{}cc|c|c@{}}
\toprule
Denoise & Accuracy & Best & Score \\
\midrule
True & 
\begin{minipage}[t]{0.25\columnwidth}$-0.21235736(x_{0}-1.1249065)(2x_{0}-1.1303912)(2x_{0}+0.2443421) + 3225.8237$\end{minipage} & 
\begin{minipage}[t]{0.25\columnwidth}$0.024268737x_{0}^{2} + 3225.7983$\end{minipage} & 
\begin{minipage}[t]{0.25\columnwidth}$x_{0}^{2}(-0.86325264x_{0}^{2} + x_{0}) + 3225.7295$\end{minipage} \\
\noalign{\smallskip} \hline \noalign{\smallskip}
False & 
\begin{minipage}[t]{0.25\columnwidth}$x_{0}^{2}(123.43398x_{0}^{4}+2326.98053420264)+2538.3494$\end{minipage} & 
\begin{minipage}[t]{0.25\columnwidth}$2417.7627x_{0}^{2} + 2527.635$\end{minipage} & 
\begin{minipage}[t]{0.25\columnwidth}$2415.3643x_{0} + 2125.6453$\end{minipage} \\
\bottomrule
\end{tabular}
\caption{SR results for 30 bins.}
\label{tab:30bins}
\end{center}
\end{table}

\begin{table}[h]
\begin{center}
\begin{tabular}{@{}cc|c|c@{}}
\toprule
Denoise & Accuracy & Best & Score \\
\midrule
True & 
\begin{minipage}[t]{0.25\columnwidth}$x_{0}^{2}(-1.615747x_{0}^{2}+2x_{0}-0.081652954)+995.048$\end{minipage} & 
\begin{minipage}[t]{0.25\columnwidth}$x_{0}(-0.46552044x_{0}^{4}+x_{0}-0.24463812)+995.06415$\end{minipage} & 
\begin{minipage}[t]{0.25\columnwidth}$995.1925$\end{minipage} \\
\noalign{\smallskip} \hline \noalign{\smallskip}
False & 
\begin{minipage}[t]{0.25\columnwidth}$x_{0}(207.340216x_{0}+428.81232)+109.830989048+750.30175$\end{minipage} & 
\begin{minipage}[t]{0.25\columnwidth}$726.08685x_{0}^{2}+757.9762$\end{minipage} & 
\begin{minipage}[t]{0.25\columnwidth}$725.2477x_{0}+637.3749$\end{minipage} \\
\bottomrule
\end{tabular}
\caption{SR results for 100 bins.}
\label{tab:100bins}
\end{center}
\end{table}

The denoising option proved to be effective just to fit the level 1 distribution with a $(1 + \cos^2 \theta)^{-1}$ reweighting to find the overall constant, as shown in Tab. \ref{tab:const}. With denoising, any selection criterion gives the correct constant answer. On the other hand, if the denoising is not applied PySR finds equations that are more expressive than the real law of Nature.

\begin{table}[h]
\begin{center}
\begin{tabular}{@{}l|c|c|c@{}}
\toprule
Denoise & Accuracy & Best & Score \\
\midrule
True & 
$6833.678$ & 
$6833.678$ & 
$6833.678$ \\
\noalign{\smallskip} \hline \noalign{\smallskip}
False & 
\begin{minipage}[t]{0.25\columnwidth}
$x_{0}^{2}(661.2393x_{0} - 706.5968)(x_{0}^{2} + x_{0}) + 7593.010$
\end{minipage} & 
\begin{minipage}[t]{0.25\columnwidth}
$7614.049 - 194.01741x_{0}$
\end{minipage} & 
\begin{minipage}[t]{0.25\columnwidth}
$7614.0547 - 194.02724x_{0}$
\end{minipage} \\
\bottomrule
\end{tabular}
\caption{SR equations with denoising for the reweighted distribution.}
\label{tab:const}
\end{center}
\end{table}

The SR results are consistent even if we change the number of events of the dataset ($10^4$ or $10^5$, for example) and obtain different levels of statistical uncertainty.

It is reassuring that, even if we do not input our knowledge of the Natural law by reweighting the level 1 distribution, PySR is still clever enough to find the correct functional form in spite of the noise in the data.

==> Chapters/appendices/sr/app_kinematics.tex <==
\section{Kinematics}

In this appendix we want to settle in the \textit{clearest} way the kinematics and the structure of the equations that we want to regress. For kinematic variables $x$, $y$, $z$, we want to write \textit{precisely} equations like

\begin{equation}
    F(x, y, z) = f_1 (x, y) \left(f_2 (z) \cdot x - 2 y^2 \cdot f_3(x, z) + f_4 (y) \right),
\end{equation}

where we understand clearly the 'structure' of the equation (what is or isn't factorised, the algebraic operations involved, etc) and the variables upon which every function $F$, $\{f_i \}_{i=1}^{4}$ depend on (what enters and does not enter in the functions, and the kinematics of \textit{which} particle in the process is the relevant one: is the lepton, the lepton pair, the intermediate boson?)

\subsection{The centre-of-mass hadronic frame}

Let us compute the Born process (leading-order)
\begin{equation}
    q_i(p_1) + \bar{q}_i(p_2) \, \to \, \gamma^* \to  l^-(p_3) + l^+(p_4),
\end{equation}
where $i$ is the flavour index. \\
Let us write explicitly the momenta in the partonic centre-of-mass energy, then we will move into the hadronic centre-of-mass energy
\begin{align*}
p_1 &= \frac{\sqrt{\hat{s}}}{2}(+1,0,0,+1)\\
p_2 &= \frac{\sqrt{\hat{s}}}{2}(+1,0,0,-1)\\
p_3 &= \frac{\sqrt{\hat{s}}}{2}(+1,+\sin\theta,0,+\cos\theta)\\
p_4 &= \frac{\sqrt{\hat{s}}}{2}(+1,-\sin\theta,0,-\cos\theta),
\end{align*}
where $\hat{s}$ is the partonic centre-of-mass energy squared and $\theta$ is the angle between the outgoing leptons and the incoming beams. Let us define the Mandelstam variables as
\begin{align*}
    \hat{s} & = (p_1+p_2)^2=(p_3+p_4)^2\\
    \hat{t} & = (p_1-p_3)^2 = (p_4 - p_2)^2 = -\frac{\hat{s}}{2}(1-\cos\theta)\\
    \hat{u} & = (p_1-p_4)^2 = (p_3 - p_2)^2 = -\frac{\hat{s}}{2}(1+\cos\theta)
\end{align*}
%
Computing the squared of the matrix element averaging/summing over the polarisation and colors, we get
\begin{equation}
    \overline{{\cal M}^2} = Q_i^2\alpha^2
    \frac{2^5\pi^2}{3}\frac{\hat{t}^2+\hat{u}^2}{\hat{s}^2} = Q_i^2\alpha^2
    \frac{2^4\pi^2}{3}(1+\cos^2\theta),
\end{equation}
where in the last passage we wrote $\hat{t}$ and $\hat{u}$ in terms of $\hat{s}$ and $\cos\theta$. The differential partonic cross section is given by
\begin{equation}
    d\hat{\sigma}^{(0)} = \frac{1}{2\hat{s}}\overline{{\cal M}^2} d\Pi_2,
\end{equation}
where $d\Pi_2$ is the two body massless phase space given by
\begin{equation}
 d\Pi_2=\frac{d^3p_3}{(2\pi)^32E_3}   \frac{d^3p_4}{(2\pi)^32E_4}(2\pi)^4\delta^{(4)}(p_1+p_2-p_3-p_4) = \frac{d\cos\theta}{16\pi}. 
\end{equation}
Putting everything together we get
\begin{equation}
\label{eq:pcs}
    \frac{d\hat{\sigma}^{(0)}}{d\cos\theta} = Q_i^2\alpha^2
    \frac{\pi}{6}\frac{1}{\hat{s}}(1+\cos^2\theta)
\end{equation}
and 
\begin{equation}
\label{eq:pcs_tot}
    \hat{\sigma}^{(0)} = Q_i^2\alpha^2
    \frac{4\pi}{9}\frac{1}{\hat{s}}
\end{equation}

Let us now go the the hadronic centre-of-mass frame (or laboratory frame as T. Han calls it in Ref.~\cite{Han:2005mu})
\begin{align*}
P_1 &= \frac{\sqrt{S}}{2}(+1,0,0,+1)\\
P_2 &= \frac{\sqrt{S}}{2}(+1,0,0,-1),
\end{align*}
where $p_1 = x_1P_1$ and $p_2 = x_2P_2$, so that
\begin{equation*}
    S = (P_1+P_2)^2 = \frac{\hat{s}}{x_1x_2} 
\end{equation*}
The factorisation theorem tells us that
\begin{align}
    \sigma(pp\to l^+l^-) &= \sum_{i}\int_{\tau^0}^1 dx_1\int_{\tau^0/x_1}^1 dx_2\, \left[q_i(x_1)\bar{q}(x_2)+q_i(x_2)\bar{q}_i(x_1)\right] \notag \\
    &\qquad\qquad \hat{\sigma}^{(0)}(q_i\bar{q}_i\to l^+l^-)
    \,\delta(x_1x_2-\tau^0),
\end{align}
where the $\delta$ functions comes because of the leading-order kinematics that constrains the product of $x_1$ and $x_2$ to be equal to $\tau^0=m_{ll}^2/S$, where $m_{ll}^2$ is the invariant mass of the outgoing lepton pair, which at the Born level is equal to the partonic centre-of-mass energy. 
Let us now define the rapidity in the hadronic centre-of-mass frame as
\begin{equation}
\label{eq:rap_def}
y = \frac{1}{2}\log\left(\frac{E_1+E_2+p^z_1+p^z_2}{E_1+E_2-(p^z_1+p^z_2)}\right)=\frac{1}{2}\log\left(\frac{x_1+x_2+x_1-x_2}{x_1+x_2-x_1+x_2}\right)=\frac{1}{2}\log(x_1/x_2).
\end{equation}
%%%%%%%%%%%%%%%%%%%%%
%Note that we can also express the rapidity of Eq. (\ref{eq:rap_def}) in terms of the kinematics of the final state and, in particular, in terms of the angle between the outgoing lepton and the incoming hadrons. To do this, we use conservation of momentum and write the rapidity as before

%\begin{equation*}
%y = \frac{1}{2}\log\left(\frac{E_3+E_4+p^z_3+p^z_4}{E_3+E_4-(p^z_3+p^z_4)}\right).
%\end{equation*}

%Since we are neglecting the masses of the particles, for each one we have $E_i^2 - |\vec{p}_i|^2 = m_i^2 = 0$, and therefore $E_i = |\vec{p}_i|$. We can write the $z$ component of each momentum of the leptons by projecting on the $Z$ axis (defined by the incoming hadrons) as ${p_z}_3 = |\vec{p}_3| \cos \theta = E_3 \cos \theta$. In this way, we have
%\begin{equation*}
%y = \frac{1}{2}\log\left(\frac{1 + \cos \theta}{1 - \cos \theta}\right).
%\end{equation*}

%However, for now, we come back to the rapidity in terms of the initial state kinematics.

%%%%%%%%%%%%%%%%%%%%% 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MMA: completing this
Rapidity of the outgoing lepton-antilepton pair

\begin{equation}
    y = \frac{1}{2} \log(\frac{(E_3 + E_4) + (p_3^z + p_4^z)}{(E_3 + E_4) - (p_3^z + p_4^z)})
\end{equation}
In the parton c.o.m frame

\begin{equation}
    \begin{cases}
        E_3 = \gamma E (1 - \beta \cos \theta*) \\
        E_4 = \gamma E (1 + \beta \cos \theta*) \\
        p_3^z = \gamma E (\cos \theta* - \beta) \\
        p_4^z = \gamma E (\cos \theta* + \beta) \\
    \end{cases}
\end{equation}
We notice that

\begin{equation}
    \begin{cases}
        E_3 + E_4 = 2 \gamma E \\
        p_3^z + p_4^z = 2 \gamma E \cos \theta* \\
    \end{cases}
\end{equation}
We sustitute these results in the first Eq. and collect and simplify the common factor $2 \gamma E$ between the numerator and the denominator

\begin{equation}
    y = \frac{1}{2} \log(\frac{1 + \cos \theta*}{1 - \cos \theta*})
\end{equation}
Hence

\begin{equation}
    \frac{1 + \cos \theta*}{1 - \cos \theta*} = e^{2y}
\end{equation}
We want to express $\cos \theta*$ in terms of $y$

\begin{equation}
    \cos \theta* = \tanh(y)
\end{equation}
% completing this now
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Using Eq. (\ref{eq:rap_def}) we can now make a change of variables $(x_1,x_2)\to(\tau,y)$,
\begin{equation}
   \tau = x_1x_2, y=\frac{1}{2}\log(x_1/x_2) \Longleftrightarrow x_1=\sqrt{\tau}e^{+y}, x_2=\sqrt{\tau}e^{-y},
\end{equation}
which gives $dx_1dx_2=d\tau d y$. The hadronic cross section becomes
\begin{align}
    \sigma(pp\to l^+l^-) &= \sum_{i}\int_{\tau^0}^1 d\tau \int_{1/2\log\tau}^{-1/2\log\tau} dy\, \left[q_i(\tau e^{+y})\bar{q}(\tau e^{-y})+q_i(\tau e^{-y})\bar{q}_i(\tau e^{+y})\right]\notag\\ 
    & \qquad\qquad \hat{\sigma}^{(0)}(q_i\bar{q}_i\to l^+l^-)
    \,\delta(\tau-\tau^0).
\end{align}
Using the $\delta$ function to set the leading-order constraint $\tau=\tau^0$ we have
\begin{equation}
  \sigma(pp\to l^+l^-) = \sum_{i} \int_{1/2\log\tau^0}^{-1/2\log\tau^0} dy\, \left[q_i(\tau^0 e^{+y})\bar{q}(\tau^0 e^{-y})+q_i(\tau^0 e^{-y})\bar{q}_i(\tau^0 e^{+y})\right] \hat{\sigma}^{(0)}(q_i\bar{q}_i\to l^+l^-)
\end{equation}
Substituting the expression we obtained in Eq.~\eqref{eq:pcs_tot} for the partonic cross section we obtain
\begin{align}
    \sigma(pp\to l^+l^-) &=  \frac{4\pi\alpha^2}{9} \frac{1}{m_{ll}^2}\notag\\
    &\sum_{i}Q_i^2 \int_{1/2\log\tau^0}^{-1/2\log\tau^0} dy\, \left[q_i(\tau^0 e^{+y})\bar{q}(\tau^0 e^{-y})+q_i(\tau^0 e^{-y})\bar{q}_i(\tau^0 e^{+y})\right],
\end{align}
where we substitute the $1/\hat{s}$ factor in the partonic cross section by $1/(\tau^0S) = 1/m_{ll}^2$. 

What happens if we want to be differential in the rapidity $y$ or in the angle $\theta$? First of all note that, given that $E_1+E_2=E_3+E_4=m_{ll}$ and 




\subsection{The Collins-Soper frame}

The purpose of the Collins-Soper frame is to retain the factorised angular dependence on $(1+\cos^2\theta)$ even when one goes beyond the Born (leading-order) calculation. 

\subsection{Complete decomposition}

Below you find the complete differential distribution of lepton pair production via Z boson DY.

\begin{align}
\frac{d\sigma}{dp_T dy dm d\cos\theta d\phi} = \frac{3}{16\pi} \frac{d\sigma^{U+L}}{dp_T dy dm} \Bigg\{ & (1 + \cos^2\theta) + \frac{1}{2} A_0(1 - 3\cos^2\theta) + A_1 \sin 2\theta \cos \phi \nonumber \\
& + \frac{1}{2} A_2 \sin^2\theta \cos 2\phi + A_3 \sin\theta \cos\phi + A_4 \cos\theta \nonumber \\
& + A_5 \sin^2\theta \sin 2\phi + A_6 \sin 2\theta \sin \phi + A_7 \sin\theta \sin \phi \Bigg\}
\label{eq:full}
\end{align}

where, as explained above Eq. (\ref{eq:full}) in Ref.~\cite{ATLAS:2016rnf} we have

\begin{enumerate}
    \item $p_T$: transverse momentum of the Z boson,
    \item $y$: rapidity of the Z boson,
    \item $m$: invariant mass of the Z, boson\footnote{When working with MG events, the invariant mass distribution of the Z boson has to be found in terms of the invariant mass of the final state, with the lepton pair. This gives the distribution centered around $m_Z \approx 90$ GeV.},
    \item $\cos \theta$: cosine of the polar angle of the lepton,
    \item $\phi$: azimuthal angle of the lepton.
\end{enumerate}

Explicitly, the functional dependence is 

\begin{equation}
    \frac{d\sigma}{dp_T dy dm d\cos\theta d\phi} = \frac{d\sigma}{dp_T dy dm d\cos\theta d\phi}(p_T, y, m, \cos\theta, \phi),
\end{equation}

\begin{equation}
    \frac{d\sigma^{U+L}}{dp_T dy dm} = \frac{d\sigma^{U+L}}{dp_T dy dm} (p_T, y, m),
\end{equation}

\begin{equation}
    A_i = A_i (p_T, y, m),
\end{equation}

for $i = 0, \dots, 7$. Some considerations for Eq. (\ref{eq:full}):

\begin{enumerate}
    \item At LO, only $A_4$ is non zero.
    \item At NLO QCD ($\mathcal{O}(\alpha_s)$) $A_{0 - 3}$ become non-zero.
    \item The coefficients $A_{5, 6, 7}$ become non-zero, while remaining small, only at NNLO QCD ($\alpha_s^2$)
\end{enumerate}

Before we tackle the fully differential distribution in Eq. (\ref{eq:full}), we move through different levels of increasing complexity.

\subsection{Level 1: $e^+ \ e^- \to \gamma \to  \mu^+ \ \mu^-$}

In this case, the distribution (very well known, see for example Eq. (1.8) in P. and S.) is
%
\begin{equation}
    \frac{d\sigma}{d\Omega} = \frac{ \alpha^2}{4s}\left(1 + \cos^2\theta\right),
\end{equation}
%

where $d \Omega$ is a differential solid angle. The distribution has azimuthal symmetry (independent of $\phi$), so the only dependence is on $\cos \theta$. Explicitly, 

\begin{equation}
    \frac{d\sigma}{d\Omega} = \frac{d\sigma}{d\Omega} (\cos \theta),
\end{equation}

\begin{equation}
    \frac{ \alpha^2}{4s} = \text{constant},
\end{equation}

and the angular dependence is known. This concludes L1.

\subsection{Level 2: $p\ p \to \gamma \to \mu^+\mu^-$}

\begin{equation}
\frac{d\sigma}{dy dm d\cos\theta d\phi} = \frac{3}{16\pi} \frac{d\sigma^{U+L}}{dy dm} \left(1 + \cos^2\theta \right),
\label{eq:l2}
\end{equation}

where

\begin{enumerate}
    \item $y$: rapidity of the intermediate boson ($\gamma$), expressed as the average of the rapidities of the muon and antimuon.
    \item $m$: invariant mass of the intermediate boson ($\gamma$)\footnote{In terms of the lepton pair, as before.},
    \item $\cos \theta$: cosine of the polar angle of the lepton,
    \item $\phi$: azimuthal angle of the lepton.
\end{enumerate}

Explicitly, the functional dependence is 

\begin{equation}
    \frac{d\sigma}{dy dm d\cos\theta d\phi} = \frac{d\sigma}{dy dm d\cos\theta d\phi}(y, m, \cos\theta, \phi),
\label{eq:l2_angs}
\end{equation}

\begin{equation}
    \frac{d\sigma^{U+L}}{dy dm} = \frac{d\sigma^{U+L}}{dy dm} (y, m),
\end{equation}

Do you agree with this?

To compare the SR closed formula with the PDFs we have

%
\begin{equation}
    \frac{d^2\sigma}{dy_{ll}dm_{ll}} = \frac{8 \pi \alpha}{3 m_{ll}} \frac{1}{3 s} \left( 
\sum_{q} Q^2 (f_{q}(x_1) f_{\overline{q}} (x_2) + f_{\overline{q}}(x_1) f_{q}(x_2 ) \right),
\label{eq:l2_pdf}
\end{equation}
%

where $y_{ll}$ and $m_{ll}$ are, respectively, the rapidity and the invariant mass of the muon pair, $\alpha = e^2 /(4 \pi)$, $x_1 = \sqrt{\tau} e^y$, $x_2 = \sqrt{\tau} e^{-y}$, $\tau = m_{ll}^2 / s$.

\textbf{Question: how do we relate Eqs. (\ref{eq:l2_angs})  and (\ref{eq:l2_pdf})?}

\subsection{Level 3: $p \ p \to Z \to \mu^+ \mu^-$}

This case is a simplification of Eq. (\ref{eq:full}). It happens at LO, where only the annihilation diagram $q \overline{q} \to \ Z$ is present. In this case, only $A_4$ is non-zero and we have

\begin{equation}
\frac{d\sigma}{dy dm d\cos\theta d\phi} = \frac{3}{16\pi} \frac{d\sigma^{U+L}}{dy dm} \left\{  (1 + \cos^2\theta) + A_4 \cos\theta 
 \right\},
\label{eq:l3}
\end{equation}

where

\begin{enumerate}
    \item $y$: rapidity of the Z boson,
    \item $m$: invariant mass of the Z, boson\footnote{In terms of the lepton pair, as before.},
    \item $\cos \theta$: cosine of the polar angle of the lepton,
    \item $\phi$: azimuthal angle of the lepton.
\end{enumerate}

In this case, there is no $p_T$ of the Z boson. \manuel{let us discuss what happens with $m$ and $y$. We have a (peaked) invariant mass distribution but the rapidity of the $Z$ boson is infinite in this case...}

Explicitly, the functional dependence is 

\begin{equation}
    \frac{d\sigma}{dy dm d\cos\theta d\phi} = \frac{d\sigma}{dy dm d\cos\theta d\phi}(y, m, \cos\theta, \phi),
\end{equation}

\begin{equation}
    \frac{d\sigma^{U+L}}{dy dm} = \frac{d\sigma^{U+L}}{dy dm} (y, m),
\end{equation}

\begin{equation}
    A_4 = A_4 (y, m).
\end{equation}

Do you agree with this?



==> Chapters/appendices/top/app-bench.tex <==
\section{Benchmarking with  SMEFiT}
\label{app:benchmark}

Here we  benchmark the performance of \simunet{} when operating
as a fixed-PDF EFT fitter, by means of a tuned comparison with
the {\sc\small SMEFiT} framework when identical theory and experimental inputs
are used in both cases.
%
\smefit currently provides two strategies to determine posterior
distributions in the EFT parameter space. The first, known as MCfit, is based on the Monte Carlo
replica method followed by parameter optimisation (as similarly used in \simunet{}).
The second is based on Nested Sampling (NS), a purely Bayesian approach for parameter inference.
%
At the linear EFT level, \smefit results based on MCfit and NS are identical~\cite{Ethier:2021bye}.
%
At the quadratic level~\cite{Giani:2023gfq},
however, the MCfit approach is affected by the potential pitfalls described in App.~\ref{app:quad},
which also prevent the use of \simunet{} for joint SMEFT-PDF fits in the presence
of quadratic EFT corrections.
%
We demonstrate now that, for a  linear EFT determination and a common choice of inputs, 
the results obtained using the two frameworks display excellent agreement.

Fig.~\ref{fig:simunet-vs-smefit-linear} displays this comparison between the
marginalised 95\% CL intervals of \simunet{}
and {\sc\small SMEFiT} (operating in the Nested Sampling mode) for a linear EFT fit that takes as input
in both cases the full dataset discussed in this work as well as the same SM and EFT
theory calculations (and hence also the same operator basis).
%
To ensure identical inputs, a parser has been written that automatically converts data and theory files
from the \simunet{} to the  {\sc\small SMEFiT} standard formats.
%
 The \simunet{} results displayed here coincide with those
 displayed in Fig.~\ref{fig:smeft_simu_bounds} in the fixed-PDF EFT analysis.
 %
 Satisfactory agreement between the two fitting frameworks is obtained,
 and similar benchmarks have been successfully performed for other variants
 of the fixed-PDF EFT fits presented in this work.

%-----------------------------------------
\begin{figure}[t]
        \centering
        \includegraphics[width=\linewidth]{smeft_plots/comparison_alltop_nlo_lin_95.png}
	\caption{Comparison between the 95\% CL intervals
          obtained with \simunet{} in the fixed-PDF linear EFT case (full top quark dataset)
          with the corresponding results based on the {\sc\small SMEFiT}
          framework (with the Nested Sampling option).
          %
          In both cases 
          the same experimental and theoretical inputs are adopted, see text for more details.
          %
          These \simunet{} results coincide with those
          displayed in Fig.~\ref{fig:smeft_simu_bounds} in the fixed-PDF EFT analysis.
        }
	\label{fig:simunet-vs-smefit-linear}
\end{figure}
%-----------------------------------------

 This benchmark study ensures that the optimisation
 algorithm adopted by \simunet{} is suitable both for PDF determinations (since it is based
 on the NNPDF4.0 settings) as well as for the determination of the EFT coefficients.
 %
 The optimisation settings that provide the best performance
 of the SM-PDF and fixed-PDF EFT analyses are then combined
 for the  simultaneous SMEFT-PDF extraction, where all weights of the \simunet{} network
 are allowed to be constrained by the data.

%\FloatBarrier


==> Chapters/appendices/top/app-chi2sm.tex <==
\section{Fit quality}
\label{app:fit_quality}

Here we summarise the $\chi^2$ (computed using the experimental
definition, Eq.~\ref{eq:chi2exp}) for the key PDF and EFT analyses presented in this work.
%
Tables~\ref{tab:chi2-baseline},~\ref{tab:chi2-top} and~\ref{tab:chi2-single-top} display
the values of the $\chi^2$ per data point for  representative PDF and EFT fits,
where for each dataset we also indicate the number of data points $n_{\rm dat}$.
%
Specifically, we consider: (i) three SM-PDF fits: \nnpdfnotop, \nnpdf, 
and Fit H in Table~\ref{tab:fit_list} (using our full top quark dataset);
(ii) two fixed-PDF EFT fits, one based on \nnpdfnotop as input,
and the other using Fit H as input; (iii) the outcome
of the simultaneous SMEFT-PDF determination.
%
We show sequentially the non-top datasets,
the $t\bar{t}$ inclusive and associated production datasets,
and the single-top inclusive and associated production datasets.
%
We also provide the total $\chi^2$ for separate groups of processes,
including the  full non-top and top datasets, and well as for their total sum.
    
In Tables~\ref{tab:chi2-top} and~\ref{tab:chi2-single-top},
entries in italics indicate datasets 
that do not enter the corresponding SM-PDF fit; for these datasets,
we evaluate the associated
$\chi^2$ values \textit{a posteriori} using the resulting PDFs.
%
For instance, all top data is removed from the \nnpdfnotop fit,
and for some top quark observables such as four-heavy-quark production,
PDF dependence is neglected.
%
Furthermore, we note that the $\chi^2$ values for the \nnpdfnotop fit
and for the fixed-PDF EFT fit based on \nnpdfnotop are identical
in Table~\ref{tab:chi2-baseline},
since the latter uses only top data as input.
%
For the same reason, the entries in the columns for the SM-PDF Fit H
and the fixed-PDF EFT fits based on Fit H are the same.
   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{tables/chi2_pdfs.tex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{tables/chi2_pdfs_top.tex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{tables/chi2_pdfs_single_top.tex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Several observations can be drawn
from the results presented in Tables~\ref{tab:chi2-baseline},~\ref{tab:chi2-top} and~\ref{tab:chi2-single-top}.
%
First of all, we note that the description of the non-top data is improved in the simultaneous
SMEFT-PDF analysis, with $\chi^2=1.137$ to be compared with the analogous SM-PDF analysis (Fit H)
which leads to $\chi^2=1.146$.
%
Given that we have $n_{\rm dat}=4535$ no-top data points, this
improvement corresponds to 40 units in the absolute $\chi^2$.
%
This improvement cannot be traced back to a specific measurements or group
of processes.
%
In turn, this improvement is also reflected for the full dataset,
whose $\chi^2$ is the lowest (1.126 for $n_{\rm dat}=4710$ points) in the SMEFT-PDF analysis.
%
This lower $\chi^2$ as compared to the SM-PDF baseline fits is not surprising,
taking into account the fact that (as discussed in Sect.~\ref{sec:res_smeft}) we now have more degrees
of freedom in the fit, and in particular the inclusion of linear EFT corrections
is instrumental in improving the $\chi^2$ to the top quark data as compared
to the SM-PDF fits.
%
We also find that the fit quality to the top datasets is similar in the joint SMEFT-PDF analysis
and in the fixed-PDF EFT fits with either \nnpdfnotop or Fit H as input
PDFs, with $\chi^2 = 0.848, 0.868, 0.839$ respectively in each case for
$n_{\rm dat}=175$.
%
The small differences between the three cases (less than five units
in absolute $\chi^2$) are consistent with the reported independence of the EFT interpretation
of top quark data with respect to the choice of input PDF in the calculation.

Finally, we note the only class of top quark production process for which the $\chi^2$ values
are markedly different in the SM-PDF fits is inclusive top quark pair production.
%
Indeed, the $\chi^2$ values for the complete top quark dataset are $1.370, 1.139$, and $1.102$ in the
SM-PDF fits without top data, with \nnpdf, and with the full top quark
dataset (Fit H) respectively; this improvement arises mostly from the $t\bar{t}$ group, whose $\chi^2$
values are $1.700, 1.328$, and $1.271$ for the same three fits respectively.
%
This observation is consistent with the findings of Sect.~\ref{sec:baseline_sm_fits}, that
the dominant PDF sensitivity in Fit H arises from inclusive $t\bar{t}$ production.
%
We also note that the $\chi^2$ for top quark data is similar between \nnpdf and Fit H, again
in agreement with the fact that the additional top quark measurements considered
here as compared to those in \nnpdf have a consistent pull on the PDFs, in particular
on the large-$x$ gluon.


%\subsection{Data-theory comparisons}
%\label{app-datatheory}

%In this section we display two data-theory comparisons which highlight the improvement in the agreement for various theory settings.

%
%%
%\begin{figure}[t]
%\centering
%\includegraphics[width=0.49\textwidth]{data_theory_plots/atlas_ttbar_ttmnorm_absolute.pdf}
%\includegraphics[width=0.49\textwidth]{data_theory_plots/atlas_ttbar_ttmnorm.pdf}
%\caption{A data-theory comparison for the ATLAS $13$ TeV differential measurement in the $\ell+$jets channel~\cite{Aad:2019ntk}, binned with respect to invariant top pair mass; predictions are evaluated with the {\tt NNPDF40\_nnlo\_as\_01180} input PDFs set, and yield a $\chi^2$ per datapoint of $2.15$. Left panel: Absolute comparison of data and theory predictions. Right panel: The ratio of the data and theory predictions to the central data values.}
%\label{fig:atlas_ttbar_ttmnorm}
%\end{figure}
%
%
%\begin{figure}
%\centering
%	\begin{subfigure}[b]{0.3\textwidth}
%	\includegraphics[scale=0.3]{data_theory_plots/atlas2D_absolute_a.pdf}
%	\includegraphics[scale=0.3]{data_theory_plots/atlas2D_norm_a.pdf}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.3\textwidth}
%	\includegraphics[scale=0.3]{data_theory_plots/atlas2D_absolute_b.pdf}
%	\includegraphics[scale=0.3]{data_theory_plots/atlas2D_norm_b.pdf}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.3\textwidth}
%	\includegraphics[scale=0.3]{data_theory_plots/atlas2D_absolute_c.pdf}
%	\includegraphics[scale=0.3]{data_theory_plots/atlas2D_norm_c.pdf}
%	\end{subfigure}
%\caption{Same as Fig.~\ref{fig:atlas_ttbar_ttmnorm} for the ATLAS $13$ TeV double-differential measurement in the hadronic channel~\cite{ATLAS:2020ccu}, binned with respect to invariant top pair mass and top pair rapidity; predictions are evaluated with the {\tt NNPDF40\_nnlo\_as\_01180} input PDF set, and yield a normalised $\chi^2$ value of $2.02$.}
%\label{fig:atlas2D}
%\end{figure}
%
%\begin{figure}
%\centering
%	\begin{subfigure}[b]{0.3\textwidth}
%	\includegraphics[scale=0.3]{data_theory_plots/cms2D_absolute_a.pdf}
%	\includegraphics[scale=0.3]{data_theory_plots/cms2D_norm_a.pdf}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.3\textwidth}
%	\includegraphics[scale=0.3]{data_theory_plots/cms2D_absolute_b.pdf}
%	\includegraphics[scale=0.3]{data_theory_plots/cms2D_norm_b.pdf}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.3\textwidth}
%	\includegraphics[scale=0.3]{data_theory_plots/cms2D_absolute_c.pdf}
%	\includegraphics[scale=0.3]{data_theory_plots/cms2D_norm_c.pdf}
%	\end{subfigure}
%         %
%	\begin{subfigure}[b]{0.3\textwidth}
%	\includegraphics[scale=0.3]{data_theory_plots/cms2D_absolute_d.pdf}
%	\includegraphics[scale=0.3]{data_theory_plots/cms2D_norm_d.pdf}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.3\textwidth}
%	\includegraphics[scale=0.3]{data_theory_plots/cms2D_absolute_e.pdf}
%	\includegraphics[scale=0.3]{data_theory_plots/cms2D_norm_e.pdf}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.3\textwidth}
%	\includegraphics[scale=0.3]{data_theory_plots/cms2D_absolute_f.pdf}
%	\includegraphics[scale=0.3]{data_theory_plots/cms2D_norm_f.pdf}
%	\end{subfigure}
%\caption{Same as Fig.~\ref{fig:atlas_ttbar_ttmnorm} for the CMS $13$ TeV differential measurement in the $\ell+$jets channel~\cite{CMS:2021vhb}, binned with respect to invariant top pair mass and top pair rapidity; predictions are evaluated with  the {\tt NNPDF40\_nnlo\_as\_01180} input PDF set and yield a normalised $\chi^2$ value of 7.14.}
%\label{fig:cms2D}
%\end{figure}
%
%\begin{figure}
%\centering
%\includegraphics[scale=0.35]{data_theory_plots/atlas_ttbarz_8tev_abs.pdf}
%\includegraphics[scale=0.35]{data_theory_plots/atlas_ttbarz_8tev_norm.pdf}
%\caption{A data-theory comparison for the ATLAS $8$ TeV total $t\bar{t}Z$ cross section~\cite{Aad:2015eua}; predictions are evaluated on the NNPDF4.0 set, and yield a normalised $\chi^2$ value of $0.23$. \textbf{Left.} Absolute comparison of data and theory predictions. \textbf{Right.} The ratio of the data and theory predictions to the central data values.}
%\label{fig:atlas_ttbarz_8tev}
%\end{figure}
%%
%\begin{figure}
%\centering
%\includegraphics[scale=0.35]{data_theory_plots/atlas_ttbarw_8tev_abs.pdf}
%\includegraphics[scale=0.35]{data_theory_plots/atlas_ttbarw_8tev_norm.pdf}
%\caption{A data-theory comparison for the ATLAS $8$ TeV total $t\bar{t}W$ cross section~\cite{Aad:2015eua}; predictions are evaluated on the NNPDF4.0 set, and yield a normalised $\chi^2$ value of $2.49$. \textbf{Left.} Absolute comparison of data and theory predictions. \textbf{Right.} The ratio of the data and theory predictions to the central data values.}
%\label{fig:atlas_ttbarw_8tev}
%\end{figure}
%%
%\begin{figure}
%\centering
%\includegraphics[scale=0.35]{data_theory_plots/atlas_ttbarz_13tev_abs.pdf}
%\includegraphics[scale=0.35]{data_theory_plots/atlas_ttbarz_13tev_norm.pdf}
%\caption{A data-theory comparison for the ATLAS $13$ TeV total $t\bar{t}Z$ cross section~\cite{Aaboud:2019njj}; predictions are evaluated on the NNPDF4.0 set, and yield a normalised $\chi^2$ value of $0.74$. \textbf{Left.} Absolute comparison of data and theory predictions. \textbf{Right.} The ratio of the data and theory predictions to the central data values.}
%\label{fig:atlas_ttbarz_13tev}
%\end{figure}
%%
%\begin{figure}
%\centering
%\includegraphics[scale=0.35]{data_theory_plots/atlas_ttbarw_13tev_abs.pdf}
%\includegraphics[scale=0.35]{data_theory_plots/atlas_ttbarw_13tev_norm.pdf}
%\caption{A data-theory comparison for the ATLAS $13$ TeV total $t\bar{t}W$ cross section~\cite{Aaboud:2019njj}; predictions are evaluated on the NNPDF4.0 set, and yield a normalised $\chi^2$ value of $1.46$. \textbf{Left.} Absolute comparison of data and theory predictions. \textbf{Right.} The ratio of the data and theory predictions to the central data values.}
%\label{fig:atlas_ttbarw_13tev}
%\end{figure}
%%
%\begin{figure}
%\centering
%\includegraphics[scale=0.7]{data_theory_plots/atlas_ttbarz_13tev_distribution_abs.pdf}
%\includegraphics[scale=0.7]{data_theory_plots/atlas_ttbarz_13tev_distribution_norm.pdf}
%\caption{A data-theory comparison for the ATLAS $13$ TeV $t\bar{t}Z$ normalised distribution, binned with respect to transverse momentum of the associated $Z$-boson~\cite{ATLAS:2021fzm}; predictions are evaluated on the NNPDF4.0 set, and yield a normalised $\chi^2$ value of $1.72$. \textbf{Top.} Absolute comparison of data and theory predictions. \textbf{Bottom.} The ratio of the data and theory predictions to the central data values.}
%\label{fig:atlas_ttbarz_distribution}
%\end{figure}
%%
%\begin{figure}
%\centering
%\includegraphics[scale=0.35]{data_theory_plots/cms_ttbarz_8tev_abs.pdf}
%\includegraphics[scale=0.35]{data_theory_plots/cms_ttbarz_8tev_norm.pdf}
%\caption{A data-theory comparison for the CMS $8$ TeV total $t\bar{t}Z$ cross section~\cite{Khachatryan:2015sha}; predictions are evaluated on the NNPDF4.0 set, and yield a normalised $\chi^2$ value of $0.47$. \textbf{Left.} Absolute comparison of data and theory predictions. \textbf{Right.} The ratio of the data and theory predictions to the central data values.}
%\label{fig:cms_ttbarz_8tev}
%\end{figure}
%%
%\begin{figure}
%\centering
%\includegraphics[scale=0.35]{data_theory_plots/cms_ttbarw_8tev_abs.pdf}
%\includegraphics[scale=0.35]{data_theory_plots/cms_ttbarw_8tev_norm.pdf}
%\caption{A data-theory comparison for the CMS $8$ TeV total $t\bar{t}W$ cross section~\cite{Khachatryan:2015sha}; predictions are evaluated on the NNPDF4.0 set, and yield a normalised $\chi^2$ value of $2.30$. \textbf{Left.} Absolute comparison of data and theory predictions. \textbf{Right.} The ratio of the data and theory predictions to the central data values.}
%\label{fig:cms_ttbarw_8tev}
%\end{figure}
%%
%\begin{figure}
%\centering
%\includegraphics[scale=0.35]{data_theory_plots/cms_ttbarz_13tev_abs.pdf}
%\includegraphics[scale=0.35]{data_theory_plots/cms_ttbarz_13tev_norm.pdf}
%\caption{A data-theory comparison for the CMS $13$ TeV total $t\bar{t}Z$ cross section~\cite{Sirunyan:2017uzs}; predictions are evaluated on the NNPDF4.0 set, and yield a normalised $\chi^2$ value of $1.23$. \textbf{Left.} Absolute comparison of data and theory predictions. \textbf{Right.} The ratio of the data and theory predictions to the central data values.}
%\label{fig:cms_ttbarz_13tev}
%\end{figure}
%%
%\begin{figure}
%\centering
%\includegraphics[scale=0.35]{data_theory_plots/cms_ttbarw_13tev_abs.pdf}
%\includegraphics[scale=0.35]{data_theory_plots/cms_ttbarw_13tev_norm.pdf}
%\caption{A data-theory comparison for the CMS $13$ TeV total $t\bar{t}W$ cross section~\cite{Sirunyan:2017uzs}; predictions are evaluated on the NNPDF4.0 set, and yield a normalised $\chi^2$ value of $0.68$. \textbf{Left.} Absolute comparison of data and theory predictions. \textbf{Right.} The ratio of the data and theory predictions to the central data values.}
%\label{fig:cms_ttbarw_13tev}
%\end{figure}
%%
%\begin{figure}
%\centering
%\includegraphics[scale=0.7]{data_theory_plots/cms_ttbarz_13tev_distribution_abs.pdf}
%\includegraphics[scale=0.7]{data_theory_plots/cms_ttbarz_13tev_distribution_norm.pdf}
%\caption{A data-theory comparison for the CMS $13$ TeV $t\bar{t}Z$ normalised distribution, binned with respect to transverse momentum of the associated $Z$-boson~\cite{CMS:2019too}; predictions are evaluated on the NNPDF4.0 set, and yield a normalised $\chi^2$ value of $1.27$. \textbf{Top.} Absolute comparison of data and theory predictions. \textbf{Bottom.} The ratio of the data and theory predictions to the central data values.}
%\label{fig:cms_ttbarz_distribution}
%\end{figure}



==> Chapters/appendices/top/app-quad.tex <==
\section{Pitfalls of the Monte-Carlo replica method for quadratic EFT fits}
\label{app:quad}

This analysis was originally prepared with the intention of performing a fully simultaneous SMEFT-PDF
fit using NLO QCD theory, including \textit{quadratic}, $\mathcal{O}\lp \Lambda^{-4}\rp$, contributions from the SMEFT.
To this end, the capabilities of the \simunet{} framework were extended, as discussed in Sect.~\ref{sec:new_simunet}, and
all necessary SMEFT $K$-factors needed for the quadratic predictions were produced.
%
However, whilst benchmarking our code, we noticed significant disagreement between quadratic SMEFT-only fits
produced using the \simunet{} methodology and the \smefit Nested Sampling option;\footnote{This disagreement is not present at the linear level; in this case, \simunet{} using the fixed-PDF option and \smefit using either the Nested Sampling or MCfit options perfectly coincide. See App.~\ref{app:benchmark} for more details.} on the other hand, we note perfect agreement
between our \simunet{} quadratic SMEFT-only fits and the \smefit MCfit option.

This disagreement can be traced back to 
a deficiency in the Monte-Carlo sampling method used to propagate experimental error to the SMEFT coefficients, which
currently prevents us from applying the
the \simunet{} framework to joint SMEFT-PDF
fits with quadratic EFT calculations. 
%
In this Appendix, we describe our current understanding of these limitations within the context of a toy model, 
and give a more realistic example from this work; further work on the topic is deferred to a future publication..

\subsection{A toy model for quadratic EFT fits}
In the following subsection, we consider a toy scenario involving a single data point $d$ and only one
Wilson coefficient $c$ (we ignore all PDF-dependence).
%
We suppose that our observed experimental data point $d$ is a random variable drawn from a normal distribution
centred on the underlying quadratic theory prediction, and with experimental variance $\sigma^2$:
\begin{equation}
\label{eq:data_gaussian}
d \sim N(t(c), \sigma^2).
\end{equation}
We assume that the theory prediction is quadratic in the SMEFT Wilson coefficient $c$, taking the form:
\begin{equation}
t(c) = t^{\text{SM}} + c t^{\text{lin}} + c^2 t^{\text{quad}} \, ,
\end{equation}
where we set $\Lambda=1$ TeV for convenience. Recall that $t^{\text{quad}} > 0$, since it corresponds
to a squared amplitude.
%
Given the observed data $d$, we would like to construct interval estimates for the parameter
$c$ (usually \textit{confidence intervals} in a frequentist setting or \textit{credible intervals} in a Bayesian setting).
%
Here, we shall describe the analytical construction of two interval estimates: first, using the Bayesian method, and second, using the
Monte-Carlo replica method.

\paragraph{Bayesian method.}
In the Bayesian approach, $c$ is treated as a random variable with its own distribution. By Bayes'
theorem, we can write the probability distribution of $c$, given the observed data $d$, up to a proportionality constant (given by $1/\mathbb{P}(d)$, where $\mathbb{P}(d)$ is called the \textit{Bayes' evidence}) as:
\begin{equation}
\mathbb{P}(c | d) \propto \mathbb{P}(d | c) \mathbb{P}(c),
\end{equation}
\noindent
where $\mathbb{P}(c|d)$ is called the \textit{posterior distribution} of $c$, given the observed data $d$,
and  $\mathbb{P}(c)$ is called the \textit{prior distribution} of $c$ - this is our initial `best guess' of the distribution of $c$ before the observation
of the data takes place.
%
This distribution 
is often taken to be uniform in SMEFT fits; we shall assume this here.

Given a value of $c$, the distribution $\mathbb{P}(d|c)$ of the data $d$ is assumed to be Gaussian, as specified in Eq.~(\ref{eq:data_gaussian}). In particular, we can deduce that the posterior distribution of $c$ obeys the following proportionality relation:\footnote{Technically, truncated according to the end-points of the uniform prior.}
\begin{equation}
\label{eq:bayesian_posterior}
\mathbb{P}(c|d) \propto \exp\left( -\frac{1}{2\sigma^2} \left( d - t(c) \right)^2 \right).
\end{equation}
\noindent This posterior distribution can be used to place interval estimates on the parameter $c$. One way of doing this is to construct \textit{highest density intervals}. These are computed as follows.
%
For a $100\alpha$\% credible interval, we determine the constant $p(\alpha)$ satisfying:
\begin{equation}
\int\limits_{\{c : ~\mathbb{P}(c|d) > p(\alpha)\}} \mathbb{P}(c|d)\ dc = \alpha.
\end{equation}
\noindent An interval estimate for $c$ is then given by $\{c : \mathbb{P}(c|d) > p(\alpha)\}$. In order to obtain such intervals then, we must construct the posterior $\mathbb{P}(c|d)$; efficient sampling from the posterior
is guaranteed by methods such as Nested Sampling~\cite{Feroz:2013hea,Feroz:2007kg}.

\paragraph{The Monte-Carlo replica method.}
%
This method takes a different approach in order to produce a posterior distribution for the parameter $c$.
%
Given the observed central data value $d$, one samples repeatedly from the normal distribution $N(d, \sigma^2)$ to generate a collection of \textit{pseudodata replicas}, which we shall denote as $d^{(1)}, ..., d^{(N_{\text{rep}})}$, where $N_{\text{rep}}$ is the total number of replicas.
%
Given a pseudodata replica $d^{(i)}$, one obtains a corresponding best-fit value of the Wilson coefficient parameter $c^{(i)}$ by minimising the $\chi^2$ of the theory to the pseudodata:
\begin{equation}
c^{(i)} = \argmin_{c} \chi^2(c,d^{(i)}) = \argmin_{c} \left( \frac{(d^{(i)} - t(c))^2}{\sigma^2} \right).
\end{equation}
In this toy scenario, we can determine an analytical formula for $c^{(i)}$:
\begin{equation}
  c^{(i)} = \begin{cases} \displaystyle -\frac{t^{\text{lin}}}{2t^{\text{quad}}}, & \text{if $d^{(i)} \leq \lp t^{\text{SM}} - (t^{\text{lin}})^2/4t^{\text{quad}}\rp $ ;} \label{eq:app1} \\[2ex]
    \displaystyle \frac{-t^{\text{lin}} \pm \sqrt{(t^{\text{lin}})^2 - 4t^{\text{quad}}(t^{\text{SM}} - d^{(i)})}}{2t^{\text{quad}}}, & \text{if $d^{(i)} \geq \lp t^{\text{SM}} - (t^{\text{lin}})^2/4t^{\text{quad}}\rp $  \, .} \end{cases}
\end{equation}
The first case arises when the $\chi^2$ to the pseudodata $d^{(i)}$ has a single minimum, whilst the second case arises when the $\chi^2$  has two minima.
%
The two cases are split based on the value of
\be
\label{eq:crosssec_minimum}
t_{\text{min}} = t^{\text{SM}} - (t^{\text{lin}})^2/4t^{\text{quad}} \, ,
\ee
which is the minimum value of the quadratic theory prediction $t(c) = t^{\text{SM}} + c t^{\text{lin}} + c^2 t^{\text{quad}}$. Note that for data replicas such that $d^{(i)}\le t_{\text{min}}$, the best-fit value $c^{(i)}$
becomes independent of $d^{(i)}$ and depends only on the ratio between linear and quadratic
EFT cross-sections.

Now, given that $d^{(i)}$ is a random variable drawn from the normal distribution $N(d,\sigma^2)$, one can infer the corresponding distribution of the random variable $c^{(i)}$, which is a function of the pseudodata $d^{(i)}$.
%
For a real random variable $X$ with associated probability density $P_X(x)$, a function $f : \mathbb{R} \rightarrow \mathbb{R}$ of the random variable has the distribution:
\begin{equation}
P_{f(X)}(y) = \int\limits_{-\infty}^{\infty} dx\ P_X(x) \delta(y - f(x)).
\end{equation}
In our case, $c^{(i)}$ is a multi-valued function of $d^{(i)}$ given the two square roots, but the formula is easily generalised to this case.
%
Recalling that the pseudodata replicas are generated according
to a Gaussian distribution around the central measurement $d$ with variance $\sigma^2$,
we find that the probability density function for the Wilson coefficient replica
$c^{(i)}$ is given (up to a proportionality constant) by:
\begin{align}
P_{c^{(i)}}(c) &\propto \int\limits_{-\infty}^{t_{\text{min}}} dx\ \delta\left( c + \frac{t^{\text{lin}}}{2t^{\text{quad}}} \right) \exp\left( -\frac{1}{2\sigma^2} (x - d)^2 \right) \notag \\[1.5ex]
&\qquad + \int\limits_{t_{\text{min}}}^{\infty} dx\  \delta\left( c - \left(\frac{-t^{\text{lin}} + \sqrt{(t^{\text{lin}})^2 - 4t^{\text{quad}}(t^{\text{SM}} - x)}}{2t^{\text{quad}}}\right)\right)\exp\left( -\frac{1}{2\sigma^2} (x - d)^2 \right) \notag\\[1.5ex]
& \qquad + \int\limits_{t_{\text{min}}}^{\infty} dx\ \delta\left( c - \left(\frac{-t^{\text{lin}} - \sqrt{(t^{\text{lin}})^2 - 4t^{\text{quad}}(t^{\text{SM}} - x)}}{2t^{\text{quad}}}\right)\right) \exp\left( -\frac{1}{2\sigma^2} (x - d)^2 \right).
\end{align}
Simplifying the delta functions in the second and third integrals, we find:
\begin{equation}
\label{eq:mc_posterior}
P_{c^{(i)}}(c) \propto \delta\left( c + \frac{t^{\text{lin}}}{2t^{\text{quad}}} \right) \int\limits_{-\infty}^{t_{\text{min}}} dx\ \exp\left( -\frac{1}{2\sigma^2} (x - d)^2 \right) + \frac{2}{|2ct^{\text{quad}}  + t^{\text{lin}}|} \exp\left( -\frac{1}{2\sigma^2} (d - t(c))^2 \right) \, .
\end{equation}
This result is different from the posterior distribution obtained by the Bayesian method in Eq.~(\ref{eq:bayesian_posterior}). Notable features of the posterior distribution $P_{c^{(i)}}(c)$ are: (i) the distribution has a Dirac-delta peak at $c = -t^{\text{lin}}/2t^{\text{quad}}$; (ii) elsewhere, the distribution is given by the Bayesian posterior distribution rescaled by a prefactor dependent on $c$.
%
Therefore, the Monte Carlo
replica optimisation method will not in general reproduce the Bayesian posterior.

However, one can note that in an appropriate limit, the Bayesian posterior \textit{is} indeed recovered.
In particular, suppose that the quadratic EFT cross-section is subdominant
compared to the linear term, $t^{\text{lin}} \gg t^{\text{quad}}$; in this case, we have that
$t_{\text{min}} \rightarrow -\infty$ so that the first term in Eq.~\eqref{eq:mc_posterior} vanishes
and the prefactor of the second term can be approximated with $2ct^{\text{quad}} + t^{\text{lin}} \approx t^{\text{lin}}$. 
Thus, the Bayesian posterior from Eq.~(\ref{eq:bayesian_posterior}) is indeed recovered, and we 
see that the two methods are formally identical for a linear EFT analysis.
%
Further, it is possible to show analytically that for multiple SMEFT parameters and multiple correlated data points, 
if only linear theory is used the two distributions agree exactly.

%However, one can note that in appropriate limits, the Bayesian posterior \textit{is} indeed recovered. For example, in the case that  i.e. the case in which the quadratic terms are weaker compared to the linear terms, we find that Hence the first term in Eq.~(\ref{eq:mc_posterior}) vanishes, whilst the denominator of the prefactor in the second term approaches $2ct^{\text{quad}} + t^{\text{lin}} \approx t^{\text{lin}}$. Indeed, more generally, one can show that for multiple SMEFT parameters and multiple correlated data points, if only linear theory is used the two distributions agree exactly.\\
%\noindent Using the identity:
%\begin{equation}
%\int\limits_{t_{\text{\min}}}^{\infty} dx\ \exp\left( -\frac{1}{2\sigma^2} (x - d)^2 \right) = \sqrt{2\pi \sigma^2} - \int\limits_{-\infty}^{t_{\text{min}}} dx\ \exp\left( -\frac{1}{2\sigma^2} (x - d)^2 \right),
%\end{equation}
%\noindent we have:
%\begin{equation}
%P_{c^{(i)}}(c) \propto \left(\delta\left( c + \frac{t^{\text{lin}}}{2t^{\text{quad}}} \right) -\frac{2 }{2ct^{\text{quad}}  + t^{\text{lin}}} \right) \int\limits_{-\infty}^{t_{\text{min}}} dx\ \exp\left( -\frac{1}{2\sigma^2} (x - d)^2 \right) + \frac{2\sqrt{2\pi \sigma^2}}{2ct^{\text{quad}}  + t^{\text{lin}}}.
%\end{equation}

This calculation demonstrates that, for quadratic EFT fits, the Monte-Carlo replica method
will not in general reproduce the Bayesian posteriors that one would obtain from, say, a 
nested sampling approach; agreement will only occur provided quadratic EFT corrections 
are sufficiently subdominant in comparison with the linear ones.
%
For this reason, in this work we restrict the SMEFT-PDF fits based on \simunet{} (which rely
on the use of the Monte-Carlo replica method) to linear EFT calculations;
we defer the further investigation of the use of the Monte-Carlo replica method, and how
it might be modified for use in \simunet{}, to future works. 

%n the case where quadratic theory is used, the  cannot be expected to reliably reproduce the  distributions that one would obtain, say, from a nested sampling approach. It is for this reason that we choose to neglect quadratic contributions in our \simunet{} fits in this work; like \nnpdf and \smefit, \simunet{} assumes that the use of the Monte-Carlo method will produce a reliable posterior, but this is in fact not the case, and - as far as we are aware - has never been justified rigorously in the literature. In Section~\ref{subsec:mc_examples}, we give explicit examples of the failure of the Monte-Carlo method relative to the Bayesian method.

\subsection{Application to one-parameter fits}
\label{subsec:mc_examples}

As demonstrated above, the Monte-Carlo replica method will lead to
posterior distributions differing from their Bayesian counterparts whenever quadratic
EFT corrections dominate over linear ones.
%
Here, we show the numerical impact of these differences in a model case, namely
the one-parameter fit of the coefficient $c_{dt}^8$ to
the CMS 13 TeV $t\bar{t}$ invariant mass distribution measurement
based on the $\ell+$jets final-state~\cite{CMS:2021vhb}.
%
Fig.~\ref{fig:data-theory-CMS} compares the experimental data
from this measurement with the corresponding
SM theory calculations at NNLO using the NNPDF4.0 (no top) PDF
set as input.
%
We observe that the SM theory predictions overshoot the data, especially in the high $m_{t\bar{t}}$
regions, where energy-growing effects enhance the EFT corrections.
%
Given that the pseudodata replicas $d^{(i)}$ are fluctuated around the central value $d$,
the configuration where the SM overshoots the data
potentially enhances the contribution of the upper solution in Eq.~(\ref{eq:app1})
leading to the Dirac delta peak in the posterior Eq.~(\ref{eq:mc_posterior}).     

%-----------------------------------------
\begin{figure}[t]
        \centering
        \includegraphics[width=0.82\linewidth]{data_theory_plots/CMS_TTBAR_13TEV_TTMNORM_NNPDF40-notop.pdf}
        \caption{Comparison between the experimental data
          for the top-quark pair invariant mass $m_{t\bar{t}}$ distribution
          from the $\ell+$jets CMS measurement at 13 TeV~\cite{CMS:2021vhb}, with the corresponding
          SM theory calculations at NNLO using the NNPDF4.0 (no top) PDF
          set as input.
          %
          For the latter, the error band indicates the PDF uncertainties, and
          for the former the diagonal entries of the experimental covariance matrix.
          %
          Results are shown as ratios to the central value of the data.
          %
          The SM theory predictions overshoot the data, especially in the high $m_{t\bar{t}}$
          regions, where energy-growing effects enhance the EFT corrections.
        }
    \label{fig:data-theory-CMS}
\end{figure}
%-----------------------------------------

For the case of the $c_{dt}^8$ coefficient, the quadratic EFT corrections dominate over the linear ones
and hence the net effect of a non-zero coefficient is typically an upwards shift
of the theory prediction.
%
Indeed, we have verified that for this coefficient
the biggest negative correction one can obtain is of order $\sim 2\%$.
%
For the last $m_{t\bar{t}}$ bin, the minimum of the  theory cross
section $t_{\rm min}$ in Eq.~(\ref{eq:crosssec_minimum}) is obtained for a value
$c_{dt}^8 \approx -0.2$, while for the second to last bin instead $t_{\rm min}$
is minimised by $c_{dt}^8 \approx -0.3$.
%
The combination of these two features (a dominant quadratic EFT term, and a SM prediction overshooting
the data) suggests that the Monte-Carlo replica method's
posterior will be enhanced for $c_{dt}^8 \in (-0.3,-0.2)$ as compared
to the Bayesian posterior.

%-----------------------------------------
\begin{figure}[h]
        \centering
        \includegraphics[width=0.49\linewidth]{smeft_plots/linear_O8dt.png}
        \includegraphics[width=0.49\linewidth]{smeft_plots/quadratic_O8dt.png}
        \caption{Posterior distributions for a one-parameter fit
          of the four-fermion coefficient $c_{dt}^8$ with the sole experimental
          input being the CMS $m_{t\bar{t}}$ distribution
          displayed in Fig.~\ref{fig:data-theory-CMS}.
          %
          Results are obtained with \smefit and we compare the outcome of Nested Sampling (in blue) with
          that of MCfit (in red)
          for linear (left panel) and quadratic (right panel) EFT fits.
        }
    \label{fig:O8dt-fit}
\end{figure}
%-----------------------------------------

In Fig.~\ref{fig:O8dt-fit} we
compare the posterior distributions for a one-parameter fit
of the four-fermion coefficient $c_{dt}^8$ with the sole experimental
input being the CMS $m_{t\bar{t}}$ distribution
displayed in Fig.~\ref{fig:data-theory-CMS}.
%
Results are obtained with \smefit and we compare the outcome of Nested Sampling (in blue) with
that of MCfit (in red)
for linear and quadratic  EFT fits.
%
The agreement in the linear fit is lost for its quadratic counterpart,
with the main difference being a sharp peak in the region
$c_{dt}^8 \in (-0.3,-0.2)$ in which the contribution
from the delta function in Eq.~\ref{eq:mc_posterior} is most
marked.

The scenario displayed in Fig.~\ref{fig:O8dt-fit} is chosen to display the maximum effect,
based on a single coefficient with large quadratic EFT corrections, and a dataset
where the SM overshoots the data in the $m_{t\bar{t}}$ region where EFT effects
are the largest.
%
Within a global fit, these differences are \textit{partially} washed out
(indeed the Bayesian and MCfit posterior distributions mostly agree well for
the quadratic \smefit analysis, as shown in~\cite{Giani:2023gfq}, for the majority
of fitted coefficients).
%
Nevertheless, at least in its current implementation, Fig.~\ref{fig:O8dt-fit} highlights
that the Monte-Carlo replica method is affected by pitfalls that
prevent its straightforward application to global EFT interpretations of experimental
data which include quadratic corrections.



==> Chapters/appendices/top/app-recommendations.tex <==
\section{Recommendations to quantify SMEFT-PDF interplay}
\label{app:recommendations}

The strategy presented here, based on 
carrying out a simultaneous determination of the SMEFT-PDFs and the Wilson coefficients, makes possible a
quantitative assessment of the interplay between the PDF and SMEFT
sensitivity when interpreting a given set of LHC measurements. 
%
As discussed in Sect.~\ref{sec:summary}, the \simunet{} framework
will be made public only at a later stage.
%
In the meantime, researchers interested in quantifying this interplay in their
own analysis can use available open-source platforms like {\sc\small xFitter},
as done by the CMS collaboration
in their QCD and EFT analyses of double-differential inclusive jet cross sections
at 13 TeV~\cite{CMS:2021yzl}.
%
In several cases, however, a joint  analysis may not be necessary,
and one can estimate the possible role of the SMEFT-PDF interplay by means
of a simplified approach.
%
The discussion is presented here for the case of top quark measurements,
but it can be straightforwardly extended to any other class of measurements.


\begin{itemize}
\item The most conservative strategy is to introduce a hard boundary between those processes
  used for PDF fits and those entering SMEFT interpretations.
  %
  For instance, for a SMEFT analysis of LHC top quark measurements one can use
  PDF fits without top data, such as the \nnpdfnotop variant.
  %
  We recall that with the NNPDF open-source code~\cite{NNPDF:2021uiq} one can produce fit variants
  with arbitrary input datasets.

\item A somewhat less  conservative assumption would be to introduce a hard boundary,
  not at the process level, but rather at the kinematic level.
  %
  In the case of inclusive top quark pair production data, one can introduce a threshold on the
  top quark pair invariant mass $m_{t\bar{t}}$ such that data points below the threshold
  are used for the PDF fit and above it for the EFT interpretation, thus
  benefiting from the increased sensitivity to BSM effects in the high-energy tails
  of the LHC distributions.
  %
  Again, using public PDF fitting codes one can produce fit variants
  with tailored kinematical cuts to separate the ``PDF'' region from the ``EFT'' region.
  %
  One drawback of this approach is that there is never a clear-cut separation
  between these regions; depending on the EFT operators considered,
  the high-energy region may not be the dominant one.

\item As demonstrated in this work, many measurements of relevance for EFT
  interpretations have limited sensitivity to PDFs and vice-versa.
  %
  In such cases, the SMEFT-PDF interplay can be safely neglected.
  %
  One can determine under which settings this condition is satisfied by
  adding the dataset under consideration either to a global PDF fit
  (using for example the NNPDF fitting code~\cite{NNPDF:2021uiq}) or to a global SMEFT
  fit (using the \smefit or \fitm frameworks).
  %
  If the results of either the PDF or EFT fits are unchanged, one can safely neglect
  the SMEFT-PDF interplay in this case.


\item If instead the above analysis shows that a given dataset provides non-trivial information 
  on both the PDFs and on the EFT Wilson coefficients, the only options for a consistent
  theoretical interpretation are either introducing a hard boundary in the analysis (either
  at the process level or at the kinematic level) or to carry out
  the joint SMEFT-PDF interpretation of the full dataset using 
  \simunet{} or other available tools.

  
\end{itemize}

Furthermore, it should be emphasised that, as opposed to the PDF case,
the sensitivity to EFT coefficients of
a given measurement depends in general on the choice of EFT operator considered.
%
Hence, the above considerations assume a specific choice of operators and could be
different if this choice is varied.


==> Chapters/appendices/top/app-theory.tex <==
\section{EFT operator basis}
\label{sec:operators}

Table~\ref{tab:ops} lists the dimension-six
SMEFT operators relevant for this analysis, together with the corresponding
degrees of freedom (DoF) entering the fit.
%
In terms of the flavour assumptions, we follow the LHC top quark working group
recommendations~\cite{Aguilar-Saavedra:2018ksv},
which were also adopted in~\cite{Ethier:2021bye,Ellis:2020unq}.
%
The flavour symmetry group is
given by U(3)$_l \times$ U(3)$_e \times$ U(3)$_d \times$ U(2)$_u \times$ U(2)$_q$, i.e. one singles out operators that contain
top quarks (right-handed $t$ and SU(2) doublet $Q$).
%
This means that we work in a 5-flavour scheme, where the only massive fermion in the theory is the top quark.
%
The upper part in Table~\ref{tab:ops} defines the relevant two-fermion 
operators modifying the interactions of the third-generation
quarks.
%
We also indicate the notation used for the associated Wilson coefficients; those
in brackets are not degrees of freedom entering the fit,
and instead the two additional DoF defined in the middle table are used.
%
The bottom table defines the four-fermion DoF entering the fit,
expressed in terms of the corresponding four-fermion Wilson coefficients
associated to dimension-six SMEFT operators in the Warsaw basis.

EFT cross-sections at the linear and quadratic order in the EFT expansion
are computed for the datasets considered in this analysis
and for the DoF defined in Table~\ref{tab:ops}, both
at LO and NLO in perturbative QCD.
%
Furthermore we use the $m_W$-scheme,  meaning that the four EW inputs are
$\{m_W, G_F, m_h, m_Z\}$.
%
In particular, the electric charge $e$ becomes a dependent parameter and is shifted by 
the effects of higher-dimensional operators.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
  \begin{center}
    \renewcommand{\arraystretch}{1.25}
    {\small
    \begin{tabular}{lll}
      \toprule
      Operator $\qquad$ & Coefficient & Definition \\
                \midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    $\Op{\varphi Q}^{(1)}$ & --~~($c_{\varphi Q}^{(1)}$) & $i\big(\varphi^\dagger\lra{D}_\mu\,\varphi\big)
 \big(\bar{Q}\,\gamma^\mu\,Q\big)$ \\\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    $\Op{\varphi Q}^{(3)}$ & $c_{\varphi Q}^{(3)}$  & $i\big(\varphi^\dagger\lra{D}_\mu\,\tau_{\sss I}\varphi\big)
 \big(\bar{Q}\,\gamma^\mu\,\tau^{\sss I}Q\big)$ \\ \hline
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    $\Op{\varphi t}$ & $c_{\varphi t}$& $i\big(\varphi^\dagger\,\lra{D}_\mu\,\,\varphi\big)
 \big(\bar{t}\,\gamma^\mu\,t\big)$ \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      $\Op{tW}$ & $c_{tW}$ & $i\big(\bar{Q}\tau^{\mu\nu}\,\tau_{\sss I}\,t\big)\,
 \tilde{\varphi}\,W^I_{\mu\nu}
 + \text{h.c.}$ \\  \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 $\Op{tB}$ & --~~($c_{tB}$) &
 $i\big(\bar{Q}\tau^{\mu\nu}\,t\big)
 \,\tilde{\varphi}\,B_{\mu\nu}
 + \text{h.c.}$ \\\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    $\Op{t G}$ & $c_{tG}$ & $i\,\big(\bar{Q}\tau^{\mu\nu}\,T_{\sss A}\,t\big)\,
 \tilde{\varphi}\,G^A_{\mu\nu}
 + \text{h.c.}$ \\
 \bottomrule\\
 \toprule
      DoF $\qquad$  & Definition \\
                \midrule
$c_{\varphi Q}^{(-)}$ &  $c_{\varphi Q}^{(1)} - c_{\varphi Q}^{(3)}$ \\
\midrule
$c_{tZ}$ &   $-\sin\theta_W c_{tB} + \cos\theta_W c_{tW} $\\
  \bottomrule\\
 \toprule
          DoF $\qquad$ &  Definition (Warsaw basis) \\
          \midrule
      $c_{QQ}^1$    &   $2\ccc{1}{qq}{3333}-\frac{2}{3}\ccc{3}{qq}{3333}$ \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    $c_{QQ}^8$       &         $8\ccc{3}{qq}{3333}$\\  \hline
          %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 $c_{Qt}^1$         &         $\ccc{1}{qu}{3333}$\\   \hline
          %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 $c_{Qt}^8$         &         $\ccc{8}{qu}{3333}$\\   \hline
          %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  $c_{tt}^1$         &     $\ccc{}{uu}{3333}$  \\    \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 $c_{Qq}^{1,8}$       &      $\ccc{1}{qq}{i33i}+3\ccc{3}{qq}{i33i}$     \\   \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  $c_{Qq}^{1,1}$         &   $\ccc{1}{qq}{ii33}+\frac{1}{6}\ccc{1}{qq}{i33i}+\frac{1}{2}\ccc{3}{qq}{i33i} $   \\    \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   $c_{Qq}^{3,8}$         &   $\ccc{1}{qq}{i33i}-\ccc{3}{qq}{i33i} $   \\   \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  $c_{Qq}^{3,1}$          &     $\ccc{3}{qq}{ii33}+\frac{1}{6}(\ccc{1}{qq}{i33i}-\ccc{3}{qq}{i33i}) $   \\     \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   $c_{tq}^{8}$         &  $ \ccc{8}{qu}{ii33}   $ \\    \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   $c_{tq}^{1}$       &   $  \ccc{1}{qu}{ii33} $\\    \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   $c_{tu}^{8}$      &   $2\ccc{}{uu}{i33i}$  \\     \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    $c_{tu}^{1}$        &   $ \ccc{}{uu}{ii33} +\frac{1}{3} \ccc{}{uu}{i33i} $ \\   \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    $c_{Qu}^{8}$         &  $  \ccc{8}{qu}{33ii}$\\     \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    $c_{Qu}^{1}$     &  $  \ccc{1}{qu}{33ii}$  \\     \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    $c_{td}^{8}$        &   $\ccc{8}{ud}{33jj}$ \\    \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    $c_{td}^{1}$          &  $ \ccc{1}{ud}{33jj}$ \\     \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    $c_{Qd}^{8}$        &   $ \ccc{8}{qd}{33jj}$ \\     \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    $c_{Qd}^{1}$         &   $ \ccc{1}{qd}{33jj}$\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
         \bottomrule
\end{tabular}
}
\end{center}
  \caption{Upper table:  definition of the two-fermion dimension-six
    SMEFT operators relevant for this analysis.
    %
    These operators modify the interactions of the third-generation
    quarks.
    %
    We also indicate the notation for the associated Wilson coefficients; those
    in brackets are not degrees of freedom entering the fit.
      %
    Middle table: the two additional degrees of freedom
    used in the fit involving two-fermion operators, defined in terms
    of the coefficients of the upper table.
    %
    Bottom table:
    the four-fermion degrees of freedom considered here,
    expressed in terms of the corresponding four-fermion Wilson coefficients
    of dimension-six SMEFT operators in the Warsaw basis.
    \label{tab:ops}}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%


% \subsection{Notation and definitions}

% We parametrise an observable $\sigma$ with EFT corrections as 

% \begin{equation} \label{eq:1}
%     \sigma = \sigma^{SM} + \sum_{i=1}^{N} c_i \sigma_{i}^{EFT} + \sum_{i=1}^{N} \sum_{j=1}^{i} c_i  c_j \sigma_{ij}^{EFT} + \mathcal{O}(c_i^3) ,
% \end{equation}

% where $N$ is the number of operators in the EFT that affect the observable and 

% \begin{equation}
%     \sigma^{SM} \sim |A^{SM}|^2
% \end{equation}

% \begin{equation}
%     \sigma_{i}^{EFT} \sim 2 Re \left( A^{SM} A^{* EFT}_{i} \right),
% \end{equation}

% \begin{equation}
%     \sigma_{ii}^{EFT} \sim |A_{i}^{EFT}|^2, 
% \end{equation}

% \begin{equation}
%     \sigma_{ij}^{EFT} \sim 2 Re \left( A^{EFT}_{i} A^{* EFT}_{j} \right). 
% \end{equation}

% Notice that we have absorbed the powers of $\Lambda$ in the definition of the Wilson coefficients $\{ c_i \}$. 

% A differential observable in the $k$-th bin of some kinematic variable can then be parametrised as 

% \begin{equation} \label{eq:4}
%     d \sigma^{k} = d {\sigma^{SM}}^{k} + \sum_{i=1}^{N} c_i d {\sigma^{EFT}_{i}}^{k} + \sum_{i=1}^{N} \sum_{j=1}^{i} c_i c_j d {\sigma_{ij}^{EFT}}^{k}
% \end{equation}

% We want to parametrise the linear and quadratic corrections of the EFT operators in an observable. Schematically, we will use Eqs. (\ref{eq:1}) and (\ref{eq:4}) to expand  

% \begin{align}
%     \frac{1}{\sigma} d \sigma^{k} = &\frac{1}{\sigma^{SM} + \cdots} \big( d {\sigma^{SM}}^{k} + \cdots \big) \\
%     = &\frac{1}{\sigma^{SM}} \big( 1 - \cdots \big) \big( d {\sigma^{SM}}^{k}  + \cdots \big). 
% \end{align}

% We will take the ratio of the above expression with respect to the SM observable and obtain 

% \begin{equation} \label{eq:ratio}
% \boxed{
% \Big( \frac{1}{\sigma} d \sigma^{k} \Big) \Big/ \Big(\frac{1}{\sigma^{SM}} d {\sigma^{SM}}^{k} \Big) = 1 +  \sum_{i=1}^{N} c_{i} K^{k}_{i} +  \sum_{i=1}^{N} \sum_{j=1}^{i} c_i  c_j K_{i,j}^{k},
% }
% \end{equation}

% and find $K_i$ and $K_{i,j}$, the so-called linear and quadratic k-factors. 

% \subsection{N = 1 case}

% With 1 EFT operator we have 

% \begin{align}
%     \frac{1}{\sigma} d {\sigma}^{k} &= \frac{1}{\sigma^{SM} + c_1 \sigma_{1}^{EFT} + c_1^2 \sigma_{11}^{EFT} } \Big( d {\sigma^{SM}}^{k} + c_1  d {\sigma_{1}^{EFT}}^{k} + c_{1}^{2}  d {\sigma_{11}^{EFT}}^{k} \Big) \\
%     &= \frac{1}{\sigma^{SM}} \Big( 1 - c_1 \frac{\sigma_{1}^{EFT}}{\sigma^{SM}} - c_1^2  \frac{\sigma_{11}^{EFT}}{\sigma^{SM}} + c_1^2  \Big( \frac{\sigma_{1}^{EFT}}{\sigma^{SM}} \Big)^2 \Big) \\
%     &\ \cdot \Big( d {\sigma^{SM}}^{k} + c_1 d {\sigma_{1}^{EFT}}^{k} + c_{1}^{2} d {\sigma_{11}^{EFT}}^{k} \Big),
% \end{align}

% where we have expanded 

% \begin{equation}
%     \frac{1}{1+x} = 1 - x + x^2 + \mathcal{O}(x^3)
% \end{equation}

% We retain part of the quadratic term in the expansion, as a term $\mathcal{O}(c_i^2)$ appears. We then perform the multiplications and arrange the terms according to power counting 

% \begin{align}
%     \frac{1}{\sigma} {d {\sigma}^{k}} = \frac{1}{\sigma_{SM}} \bigg( &d {\sigma^{SM}}^{k} \\
%     &+ c_1  \Big( d {\sigma^{EFT}_{1}}^{k} - \frac{\sigma_{1}^{EFT}}{\sigma^{SM}} d {\sigma^{SM}}^{k}  \Big) \\
%     &+ c_1^2  \Big( d {\sigma^{EFT}_{11}}^{k} - \frac{\sigma_{1}^{EFT}}{\sigma^{SM}} d {\sigma_{1}^{EFT}}^{k} - \frac{\sigma_{11}^{EFT}}{\sigma^{SM}} d {\sigma^{SM}}^{k} \Big( \frac{\sigma_{1}^{EFT}}{\sigma^{SM}} \Big)^2 d {\sigma^{SM}}^{k} \Big)
% \end{align}

% The linear k-factor seems to be only a difference between differential cross sections, but the quadratic one is a bit more intricate. Let us bring one more operator to the game to see if we can find a pattern, and address the cross terms.

% \subsection{N=2 case}

% Now we have

% \begin{align}
%     &\frac{1}{\sigma} d {\sigma}^{k} = \frac{1}{\sigma^{SM} + c_1  \sigma^{EFT}_{1} + c_2 \sigma^{EFT}_{2} + c_1^2 \sigma^{EFT}_{11} + c_2^2 \sigma^{EFT}_{22} +  c_1 c_2 \sigma_{12}^{EFT} } \\
%     &\cdot \Big( d {\sigma^{SM}}^{k} + c_1 d {\sigma^{EFT}_{1}}^{k} + c_2 d {\sigma^{EFT}_{2}}^{k} + c_1^2 d {\sigma^{EFT}_{11}}^{k} + c_2^2 d {\sigma^{EFT}_{22}}^{k} +  c_1 c_2 d {\sigma_{12}^{EFT}}^{k} \Big),
% \end{align}

% where we have used the fact that $\sigma_{ij} = \sigma_{ji}$ for any $i, j = 1, \dots, N$. Expanding the denominator as we did before, we get 

% \begin{align} \label{eq:useful}
%     \frac{1}{\sigma} d {\sigma}^{k} = &\frac{1}{\sigma^{SM}} \bigg( 1 - c_1 \bigg( \frac{\sigma^{EFT}_{1}}{\sigma^{SM}} \bigg) - c_2 \bigg( \frac{\sigma^{EFT}_{2}}{\sigma^{SM}} \bigg) - c_1^2 \bigg( \frac{\sigma^{EFT}_{11}}{\sigma^{SM}} \bigg) - c_2^2 \bigg( \frac{\sigma^{EFT}_{22}}{\sigma^{SM}} \bigg) -  c_1 c_2 \bigg( \frac{\sigma^{EFT}_{12}}{\sigma^{SM}} \bigg) \\
%     &+  c_1^2\Big( \frac{\sigma_{1}^{EFT}}{\sigma^{SM}} \Big)^{2} + c_2^{2} \Big( \frac{\sigma_{2}^{EFT}}{\sigma^{SM}} \Big)^{2}
%     + 2 c_1 c_2 \frac{\sigma_{1}^{EFT}}{\sigma^{SM}} \frac{\sigma_{2}^{EFT}}{\sigma^{SM}} \bigg)\\
%     &\cdot \bigg( d {\sigma^{SM}}^{k} + c_1 d {\sigma^{EFT}_{1}}^{k} + c_2 d {\sigma^{EFT}_{2}}^{k} + c_1^2 d {\sigma^{EFT}_{11}}^{k} + c_2^2 d {\sigma^{EFT}_{22}}^{k} +  c_1 c_2 d {\sigma_{12}^{EFT}}^{k} \bigg).
% \end{align}

% Rearranging the terms we get 

% \begin{align}
%  \frac{1}{\sigma} d {\sigma}^{k} = &\frac{1}{\sigma_{SM}} \Bigg(  d {\sigma^{SM}}^{k} \\
%  &+  c_1 \Big( d {\sigma_1^{EFT}}^{k} -  \frac{\sigma_1^{EFT}}{\sigma^{SM}} d {\sigma^{SM}}^{k} \Big) + c_2 \Big( d {\sigma_2^{EFT}}^{k} - c_2 \frac{\sigma_2^{EFT}}{\sigma^{SM}} d {\sigma^{SM}}^{k} \Big) \\
%  &+ c_1^2 \bigg( d {\sigma^{EFT}_{11}}^{k} -  \frac{\sigma_{11}^{EFT}}{\sigma^{SM}} d {\sigma^{SM}}^{k} + \Big(\frac{\sigma_1^{EFT}}{\sigma^{SM}} \Big)^2  d {\sigma^{SM}}^{k} - \Big(\frac{\sigma_1^{EFT}}{\sigma^{SM}} \Big) d {\sigma_{1}^{EFT}}^{k} \bigg) \\
%   &+ c_2^2 \bigg( d {\sigma^{EFT}_{22}}^{k} -  \frac{\sigma_{22}^{EFT}}{\sigma^{SM}} d {\sigma^{SM}}^{k} + \Big(\frac{\sigma_2^{EFT}}{\sigma^{SM}} \Big)^2  d {\sigma^{SM}}^{k} - \Big(\frac{\sigma_2^{EFT}}{\sigma^{SM}} \Big) d {\sigma_{2}^{EFT}}^{k} \bigg) \\
%  &+ c_1 c_2 \bigg( d {\sigma^{EFT}_{12}}^{k} - \frac{\sigma_{12}^{EFT}}{\sigma^{SM}} d {\sigma^{SM}}^{k}  + 2 \Big( \frac{\sigma_1^{EFT}}{\sigma^{SM}} \Big) \Big(  \frac{\sigma_2^{EFT}}{\sigma^{SM}} \Big) d {\sigma^{SM}}^{k} \\
%  &- \frac{\sigma_{1}^{EFT}}{\sigma^{SM}} d {\sigma^{EFT}_{2}}^{k} - \frac{\sigma_{2}^{EFT}}{\sigma^{SM}} d {\sigma^{EFT}_{1}}^{k}
%  \bigg)
%  \Bigg)
% \end{align}

% Let us study the equation above, order by order:

% \begin{itemize}
%     \item The first line is simply the $\mathcal{O}(c_i^0)$ term. 
%     \item The second line contains the linear corrections, $\mathcal{O}(c_i)$. It is easy to see the pattern and to generalise to $N$ operators
%     \item Lines $3$ to $6$ contain the quadratic corrections $\mathcal{O}(c_i^2)$. Lines $3$ and $4$ have the diagonal coefficients, and we can see the pattern to generalise to $N$ operators. Lines $5$ and $6$ is the interference between the two EFT operators. In fact, from Eq. (\ref{eq:useful}) it is not hard to see that the coefficient must have the same structure for any mixing of operators with $i \neq j$ (this is has also been checked with Mathematica for arbitrary $N$).  
% \end{itemize}

% \subsection{Result for N operators}


% We can write the above expression for $N$ operators as 

% \begin{align}
%     \frac{1}{\sigma} d {\sigma}^{k} = &\frac{d {\sigma^{SM}}^{k}}{\sigma^{SM}} \\
%     &+   \sum_{i=1}^{N} c_i \Tilde{K}_{i}^{k} \\
%     &+   \sum_{i=1}^{N} \sum_{j=1}^{i} c_i c_j \Tilde{K}_{i,j}^{k} + \mathcal{O} (\Lambda^{-5}),
% \end{align}

% with

% \begin{equation}
%     \Tilde{K}_{i}^{k} \equiv \frac{1}{\sigma^{SM}} \Big( d {\sigma^{EFT}_{i}}^{k}  - \frac{\sigma_{i}^{EFT}}{\sigma^{SM}} d {\sigma^{SM}}^{k} \Big),
% \end{equation}

% for the linear corrections,

% \begin{equation}
%     \tilde{K}_{i,i}^{k} \equiv \frac{1}{\sigma^{SM}} \Big( d {\sigma^{EFT}_{ii}}^{k} - \frac{\sigma^{EFT}_{i}}{\sigma^{SM}} d {\sigma^{EFT}_{i}}^{k} + \Big(  \frac{\sigma^{EFT}_{i}}{\sigma^{SM}} \Big)^2 d {\sigma^{SM}}^{k} - \Big( \frac{\sigma^{EFT}_{ii}}{\sigma^{SM}}  \Big) d {\sigma^{SM}}^{k} \Big),
% \end{equation}

% for the diagonal quadratic corrections, and

% \begin{equation}
%     \Tilde{K}_{i,j}^{k} \equiv \frac{1}{\sigma^{SM}} \Big( d {\sigma^{EFT}_{ij}}^{k} - \frac{\sigma^{EFT}_{i}}{\sigma^{SM}} d {\sigma^{EFT}_{j}}^{k} - \frac{\sigma^{EFT}_{j}}{\sigma^{SM}} d {\sigma^{EFT}_{i}}^{k} + 2 \Big(  \frac{\sigma^{EFT}_{i}}{\sigma^{SM}} \Big) \Big(  \frac{\sigma^{EFT}_{j}}{\sigma^{SM}} \Big) d {\sigma^{SM}}^{k} - \frac{\sigma^{EFT}_{ij}}{\sigma^{SM}} d {\sigma^{SM}}^{k} \Big),
% \end{equation}

% for the off-diagonal quadratic corrections, $i \neq j$. To find the final k-factors, we take the ratio with the SM observable as in Eq. (\ref{eq:ratio}) and obtain 

% \begin{equation}
% \boxed{
%     K_{i}^{k} \equiv  \frac{ d {\sigma^{EFT}_{i}}^{k} }{d {\sigma^{SM}}^{k}  } - \frac{\sigma_{i}^{EFT}}{\sigma^{SM}},
% }
% \end{equation}

% \begin{equation}
% \boxed{
%     K_{i,i}^{k} \equiv \frac{ d {\sigma^{EFT}_{ii}}^{k}}{ d {\sigma^{SM}}^{k} } - \frac{\sigma^{EFT}_{i}}{\sigma^{SM}} \frac{ d {\sigma^{EFT}_{i}}^{k}}{d {\sigma^{SM}}^{k}} + \Big(  \frac{\sigma^{EFT}_{i}}{\sigma^{SM}} \Big)^2 - \Big( \frac{\sigma^{EFT}_{ii}}{\sigma^{SM}}  \Big),
% }
% \end{equation}

% and

% \begin{equation}
% \boxed{
%     K_{i,j}^{k} \equiv \frac{ d {\sigma^{EFT}_{ij}}^{k}}{d {\sigma^{SM}}^{k}} - \frac{\sigma^{EFT}_{i}}{\sigma^{SM}} \frac{ d {\sigma^{EFT}_{j}}^{k}}{d {\sigma^{SM}}^{k}} - \frac{\sigma^{EFT}_{j}}{\sigma^{SM}} \frac{ d {\sigma^{EFT}_{i}}^{k}}{d {\sigma^{SM}}^{k}} + 2 \Big(  \frac{\sigma^{EFT}_{i}}{\sigma^{SM}} \Big) \Big(  \frac{\sigma^{EFT}_{j}}{\sigma^{SM}} \Big)  - \frac{\sigma^{EFT}_{ij}}{\sigma^{SM}}. 
%     }
% \end{equation}


==> Chapters/appendices/top/tables/baseline_fit_names.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[tb]
  \begin{center}
  \centering
  \tiny
   \renewcommand{\arraystretch}{1.5}
   \setlength{\tabcolsep}{5pt}
  \begin{tabular}{l|C{1.5cm}C{1.5cm}C{1.5cm}C{1.5cm}C{1.5cm}C{1.5cm}C{1.5cm}}
  \multirow{2}{*}{\textbf{Fit ID}}    &  \multicolumn{6}{c}{\textbf{Datasets included in fit}}  \\
   & \textbf{No-top baseline, Sect.~\ref{sec:baseline_data}} & \textbf{Incl. $t\bar{t}$, Table~\ref{tab:input_datasets_toppair}} & \textbf{Asymm., Table~\ref{tab:input_datasets_topasymmetries}} & \textbf{Assoc. $t\bar{t}$, Table~\ref{tab:input_datasets2}} & \textbf{Single-$t$, Table~\ref{tab:input_datasets_3}} & \textbf{Assoc. single$-t$, Table~\ref{tab:input_datasets_4}}  \\
    \midrule
    \nnpdfnotop (Baseline) & \checkmark  \\
    A (inclusive $t\bar{t}$) & \checkmark & \checkmark \\
    B (inclusive $t\bar{t}$ and charge asymmetry) & \checkmark & \checkmark & \checkmark \\
    C (single top) & \checkmark & & & & \checkmark \\
    D (all $t\bar{t}$ and single top) & \checkmark & \checkmark & \checkmark & & \checkmark \\
    E (associated $t\bar{t}$) & \checkmark & & & \checkmark & & \\
    F (associated single top) & \checkmark & & & & & \checkmark \\
    G (all associated top) & \checkmark & & & \checkmark & & \checkmark \\
    H (all top data) & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
    \bottomrule
  \end{tabular}
  \vspace{0.3cm}
  \caption{Overview of the SM-PDF fits discussed in this section.
    %
    The baseline fit, \nnpdfnotop, is based on the same dataset as \nnpdf
    with all top quark measurements excluded.
    %
    The fit variants A to G consider the impact of including in this baseline
    various subsets of top data, while in fit H the full set of top quark measurements described in Sect.~\ref{sec:exp} is added to the baseline.
     \label{tab:fit_list}
  }
  \end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> Chapters/appendices/top/tables/chi2_pdfs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
  \begin{center}
  \renewcommand{\arraystretch}{1.20}
%\scriptsize
\tiny
\begin{tabular}{ l | c| C{1.2cm} | C{1.2cm} | C{1.0cm} | C{1.2cm} | C{1.2cm} | C{1.2cm} }
 \toprule
 \multirow{3}{*}{Dataset}    & \multirow{3}{*}{$n_{\rm dat}$}   &  \multicolumn{6}{c}{$\chi^2/n_{\rm dat}$}  \\[1.5ex]
 &   & \multicolumn{3}{c|}{\bf SM-PDF fits} & \multicolumn{2}{c|}{\bf Fixed-PDF EFT fits}   & {\bf SMEFT-PDFs}    \\
  &   & NNPDF4.0 (no top)  & NNPDF4.0 & Fit H & NNPDF4.0 (no top) & Fit H & Joint fit   \\
 \midrule
 \midrule
 SLAC      & 67   & 0.768   & 0.758 & 0.753 & 0.768 & 0.753  & 0.761  \\
 BCDMS   & 581 &  	1.265  & 1.247 & 1.251 & 1.265  & 1.251  & 1.245   \\
 NMC       & 325 & 1.298   & 1.306 & 1.304  & 1.298  & 1.304  & 1.292    \\
 CHORUS  & 832 & 0.899    & 0.900 & 0.901  & 0.899  & 0.901  & 0.898     \\
  NuTeV     & 76  & 0.398 & 0.425  & 0.423 & 0.398  & 0.423  & 0.393    \\
 HERA  & 1208 & 1.204  & 1.203 & 1.204  & 1.204  & 1.204  & 1.200    \\
 \midrule
     {\bf Total DIS}  & {\bf 3089} &  {\bf 1.122 }  & {\bf 1.119 } & {\bf 1.119 } & {\bf 1.122 } & {\bf 1.119 } & {\bf 1.114 } \\
     \midrule
     \midrule
 E886    $\sigma^d_{\rm DY}/\sigma^p_{\rm DY}$ & 15  & 0.527    & 0.524  & 0.536  & 0.527 & 0.536   & 0.544   \\
 E886    $\sigma^p_{\rm DY}$                               & 89  & 1.566  & 1.559  & 1.615  & 1.566 & 1.615  & 1.602   \\
 E605   $\sigma^p_{\rm DY}$                                & 85  & 0.456   & 0.456  & 0.460 & 0.456  & 0.460  & 0.464    \\
 E906   $\sigma^d_{\rm DY}/\sigma^p_{\rm DY}$ &  6  &  0.827   &    0.885  & 0.886   & 0.827 & 0.886  &  0.955    \\
\midrule
{\bf Total fixed-target DY} & {\bf 195} & {\bf 0.981 } & {\bf 0.979 }   & {\bf 1.008 } & {\bf 0.981} & {\bf 1.008 } & {\bf 1.006 }  \\
 \midrule
 \midrule
 CDF    $d\sigma_Z/dy_Z$                                    & 28 &  1.234  & 1.280  &  1.275 & 1.234  & 1.275  & 1.188    \\
 D0     $d\sigma_Z/dy_Z$                                     & 28 &   0.637  & 0.644 &  0.640 & 0.637  & 0.640 & 0.632   \\
 D0    	$W\to \mu \nu$ asy.                       & 9  &   1.958 & 1.929 & 1.905  & 1.958  & 1.905 & 1.641     \\
 \midrule
 ATLAS low-mass DY 7 TeV               & 6 &  0.875  & 0.879 & 0.883  & 0.875  & 0.883 & 0.888    \\
 ATLAS high-mass DY 7 TeV               & 5 & 1.694 & 1.691 & 1.661 & 1.694  & 1.661 & 1.629  \\
 ATLAS $W, Z$ 7 TeV ($\mathcal{L} = 35$ pb${}^{-1}$) & 30   &  1.000 & 0.988 & 1.000 & 1.000 & 1.000  & 0.991    \\
 ATLAS  $W,Z$ 7 TeV ($\mathcal{L} = 4.6$ fb${}^{-1}$) & 61  & 1.689 & 1.686  & 1.685 & 1.685  & 1.685 & 1.599    \\
ATLAS low-mass DY 2D 8 TeV            & 60 & 1.203 &1.216 & 1.225 & 1.203  & 1.225 & 1.207   \\
ATLAS high-mass DY 2D 8 TeV           & 48 & 1.123  & 1.110 & 1.118 & 1.123  & 1.118 & 1.147   \\
ATLAS $\sigma_{W,Z}^{\rm tot}$ 13 TeV    & 3 & 0.727 & 0.778  & 0.706 & 0.727 & 0.706 & 0.471 \\
 \midrule
 CMS $W$ electron asymmetry 7 TeV             & 11 & 0.836 & 0.833 & 0.836 & 0.836 & 0.836 & 0.892   \\
CMS $W$ muon asymmetry 7 TeV              & 11 & 1.728 & 1.714 & 1.733 & 1.728  & 1.733 &  1.699  \\
CMS DY 2D 7 TeV                                        & 110 & 1.367 & 1.361 & 1.353 & 1.367 & 1.353 &  1.339 \\
CMS $W$ rapidity 8 TeV                              & 22 & 1.375 & 1.361 & 1.365 & 1.375  & 1.365 & 1.162  \\
 \midrule
 LHCb $Z \rightarrow ee$ 7 TeV                       & 9  &  1.630  & 1.648 & 1.636 & 1.630 & 1.636 & 1.669 \\
 LHCb $Z \rightarrow ee$ 8 TeV                        & 17  & 1.272   & 1.325 & 1.334 & 1.272 &  1.334 & 1.266 \\
 LHCb  $W,Z \rightarrow \mu$  7 TeV                 & 29  &   2.032 &  1.948 & 1.902 & 2.032 & 1.902 & 1.896   \\
 LHCb  $W,Z \rightarrow \mu$   8 TeV                & 30  & 1.494   & 1.426 & 1.417 & 1.494  & 1.417 & 1.386  \\
  LHCb  $Z \rightarrow ee$   13 TeV                & 15  & 1.701 & 1.726  & 1.717  & 1.701  & 1.717 & 1.640   \\
  LHCb  $Z \rightarrow \mu\mu$   13 TeV                & 16  & 0.970 & 0.993 & 0.978  & 0.970  & 0.978 & 0.928   \\
\midrule
{\bf Total inclusive gauge boson production} & {\bf 548} &  {\bf 1.344}  & {\bf 1.339}  & {\bf 1.335}  & {\bf 1.344}  & {\bf 1.335} & {\bf 1.297}    \\
 \midrule
 \midrule
ATLAS $W^{\pm}+$jet 8 TeV                      & 30 & 0.954 & 0.959 & 0.957  & 0.954  & 0.957 & 0.973 \\
ATLAS $Z$ $p_T$ 8 TeV ($p_T, m_{\ell\ell}$)      & 44 & 0.911 & 0.905 & 0.904 & 0.911 & 0.904 & 0.910 \\
ATLAS $Z$ $p_T$ 8 TeV ($p_T, y_Z$)                 & 48 & 0.909 & 0.898 & 0.896 & 0.909 & 0.896 & 0.924\\
ATLAS incl. jets 8 TeV, $R=0.6$                           & 171 & 0.682 & 0.687 & 0.687 & 0.682  & 0.687 & 0.667  \\
ATLAS dijets 7 TeV, $R=0.6$                               & 90 & 2.184  & 2.149  & 2.125  & 2.184 & 2.125 &. 2.177  \\
ATLAS isolated $\gamma$ prod. 13 TeV             & 53 & 0.811  & 0.763 & 0.753 & 0.811  & 0.753 & 0.813  \\
 \midrule
CMS $Z$ $p_T$ 8 TeV                                 & 28 & 1.447 & 1.401 & 1.407  & 1.447 & 1.407 & 1.473  \\
CMS incl. jets 8 TeV                                     & 185 & 1.140 & 1.183 & 1.200 & 1.140  & 1.200 & 1.118   \\
CMS dijets 7 TeV                                          & 54 & 1.788 & 1.810  & 1.809 & 1.788 & 1.809  & 1.800  \\
 \midrule
     {\bf Total jets, $Z$ $p_T$ and isolated photon}                      & {\bf 703} &  {\bf 1.154}  & {\bf 1.157} & {\bf 1.158}  & {\bf 1.154}  & {\bf 1.158}  & {\bf 1.148}  \\
      \midrule
 \midrule
     {\bf Total non-top data}                      & {\bf 4535} & {\bf 1.148}  &  {\bf 1.145} & {\bf 1.146} & {\bf 1.148} & {\bf 1.146} & {\bf 1.137} \\
 \bottomrule
\end{tabular}
\end{center}
  \caption{\small \label{tab:chi2-baseline} The values of the $\chi^2$ per data point (using the experimental
    definition of Eq.~\eqref{eq:chi2exp}) for key PDF and EFT analyses presented in this work.
    %
    For each dataset, we indicate the number of data points $n_{\rm dat}$
    and the the $\chi^2$ values for {\it i)} three SM-PDF fits:
    \nnpdfnotop, \nnpdf,
    and Fit H in Table~\ref{tab:fit_list} (full top quark dataset);
    {\it ii)} two fixed-PDF EFT fits: one based on \nnpdfnotop as input,
    and the other using Fit H as input; and finally  {\it iii)} the outcome
    of the simultaneous SMEFT-PDF determination.
    %
    Here we restrict ourselves to the non-top datasets considered in this
    analysis, the corresponding results for the top quark observables
    are provided in Tables~\ref{tab:chi2-top} and~\ref{tab:chi2-single-top}.
    %
    We also provide the total $\chi^2$ for separate groups of processes as well
    as for the full non-top dataset.
    %
    The $\chi^2$ values for the \nnpdfnotop fit
    and for the fixed-PDF EFT fit based on \nnpdfnotop are identical,
    since the latter uses only top data as input.
    %
    For the same reason, the entries in the columns for the SM-PDF Fit H
    and the fixed-PDF EFT fits based on Fit H are the same.
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Chapters/appendices/top/tables/chi2_pdfs_single_top.tex <==
\begin{table}[htbp]
  \begin{center}
  \renewcommand{\arraystretch}{1.50}
%\scriptsize
    \tiny
\begin{tabular}{ l | c| C{1.2cm} | C{1.2cm} | C{1.0cm} | C{1.2cm} | C{1.2cm} | C{1.5cm} }
 \toprule
 \multirow{3}{*}{Dataset}    & \multirow{3}{*}{$n_{\rm dat}$}   &  \multicolumn{6}{c}{$\chi^2/n_{\rm dat}$}  \\[1.5ex]
 &   & \multicolumn{3}{c|}{\bf SM-PDF fits} & \multicolumn{2}{c|}{\bf Fixed-PDF EFT fits}   & {\bf SMEFT-PDFs}    \\
  &   & NNPDF4.0 (no top)  & NNPDF4.0 & Fit H & NNPDF4.0 (no top) & Fit H & Joint fit   \\
 \midrule
 \midrule
     ATLAS $t$-channel $\sigma(t)$, 7 TeV & 1 & \textit{0.785} & \textit{0.756} & 0.757 & 0.179 & 0.135 & 0.155  \\
    ATLAS $t$-channel $\sigma(\bar{t})$, 7 TeV & 1 & \textit{0.304}  & \textit{0.296} & 0.282 & 0.003 & 0.005 & 0.004  \\
    ATLAS $t$-channel $1/\sigma d\sigma(tq)/dy_t$, 7 TeV & 3 & \textit{0.909} & 0.959 & 0.971 & 0.885 & 0.946 & 0.900  \\
     ATLAS $t$-channel $1/\sigma d\sigma(\bar{t}q)/dy_{\bar{t}}$, 7 TeV & 3 & \textit{0.061}  & 0.062 & 0.062 & 0.061 & 0.063 & 0.062  \\
     ATLAS $t$-channel $\sigma(t)$, 8 TeV & 1 & \textit{0.795}  & \textit{0.739} & 0.739 & 0.000 & 0.017 & 0.007 \\
     ATLAS $t$-channel $\sigma(\bar{t})$, 8 TeV & 1 & \textit{2.314} & \textit{2.277}  & 2.221 & 0.379 & 0.337 & 0.356  \\
    ATLAS $t$-channel $1/\sigma d\sigma(tq)/dy_t$, 8 TeV & 3 & \textit{0.288} & 0.246 & 0.241 & 0.290 & 0.245 & 0.283  \\
     ATLAS $t$-channel $1/\sigma d\sigma(\bar{t}q)/dy_{\bar{t}}$, 8 TeV & 3 & \textit{0.196} & 0.190 & 0.187 & 0.198 & 0.189 & 0.192  \\
     ATLAS $s$-channel $\sigma(t + \bar{t})$, 8 TeV & 1 & \textit{0.211} & \textit{0.203} & 0.216 & 0.000 & 0.000 & 0.000  \\
    ATLAS $t$-channel $\sigma(t)$, 13 TeV & 1 & \textit{0.738} & \textit{0.722} & 0.720 & 0.261 & 0.224 & 0.235  \\
    ATLAS $t$-channel $\sigma(\bar{t})$, 13 TeV & 1 & \textit{0.400} & \textit{0.393} & 0.384 & 0.057 & 0.050 & 0.051  \\
     ATLAS $s$-channel $\sigma(t + \bar{t})$, 13 TeV & 1 & \textit{0.700} & \textit{0.688} & 0.703 & 0.127 & 0.138 & 0.118  \\
    \midrule
    CMS $t$-channel $\sigma(t) + \sigma(\bar{t})$, 7 TeV & 1 & \textit{0.765}  & 0.729  & 0.719 & 0.010 & 0.001 & 0.004  \\
    CMS $t$-channel $\sigma(t)$, 8 TeV & 1 & \textit{0.010} & \textit{0.006} & 0.005 & 0.487 & 0.628 & 0.566  \\
    CMS $t$-channel $\sigma(\bar{t})$, 8 TeV & 1 & \textit{0.079} & \textit{0.084} & 0.092 & 0.886 & 0.934  & 0.911 \\
    CMS $s$-channel $\sigma(t + \bar{t})$, 8 TeV & 1 & \textit{1.108}  & \textit{1.112} & 1.105 & 1.348 & 1.338 & 1.350 \\
    CMS $t$-channel $\sigma(t)$, 13 TeV & 1 & \textit{0.904} & \textit{0.883} & 0.880 & 0.281 & 0.235 & 0.248  \\
    CMS $t$-channel $\sigma(\bar{t})$, 13 TeV & 1 & \textit{0.136} & \textit{0.132} & 0.125 & 0.010 & 0.014 & 0.013 \\
   CMS $t$-channel $1/\sigma d\sigma/d|y^{(t)}|$, 13 TeV & 4 & \textit{0.412} & \textit{0.387} & 0.383 & 0.405 & 0.378 & 0.396  \\
       \midrule
   {\bf Total single top}  & {\bf 30}  & {\bf 0.509 }  &  {\bf 0.498 } & {\bf 0.495 } & {\bf 0.332 } & {\bf 0.330 } & {\bf 0.331 }  \\
     \midrule
     \midrule
    ATLAS $\sigma(tW)$, dilepton, 8 TeV & 1 & \textit{0.510} & \textit{0.529} & 0.538 & 0.144  & 0.168 & 0.167 \\
    ATLAS $\sigma(tW)$, single-lepton, 8 TeV & 1 & \textit{0.695} & \textit{0.708} & 0.713 & 0.428 & 0.449 & 0.448  \\
    ATLAS $\sigma(tW)$, dilepton, 13 TeV & 1 & \textit{1.150} & \textit{1.149} & 1.148 & 0.840 & 0.847 & 0.849  \\
    ATLAS $\sigma_{\text{fid}}(tZj)$, dilepton, 13 TeV & 1 & \textit{0.115} & \textit{0.115} & \textit{0.115} & 0.871 & 0.611 & 0.795  \\
    \midrule
    CMS $\sigma(tW)$, dilepton, 8 TeV & 1 & \textit{0.359} & \textit{0.371} & 0.376 & 0.134 & 0.150 & 0.149 \\
    CMS $\sigma(tW)$, dilepton, 13 TeV & 1 & \textit{0.434} & \textit{0.437} & 0.438 & 1.612 & 1.573 & 1.563 \\
    CMS $\sigma_{\text{fid}}(tZj)$, dilepton, 13 TeV & 1 & \textit{1.041} & \textit{1.041} & \textit{1.041} & 0.279 & 0.427 & 0.316  \\
    CMS $d\sigma_{\text{fid}}(tZj)/dp_T^{t}$, dilepton, 13 TeV & 3 & \textit{0.362} & \textit{0.362} & \textit{0.362} & 0.130 & 0.156 & 0.134  \\
   CMS $\sigma(tW)$, single-lepton, 13 TeV & 1 & \textit{2.837} & \textit{2.833} & 2.832 & 1.817 & 1.839 & 1.846  \\
    \midrule
   {\bf Total associated single top}  & {\bf 11}  & {\bf 0.748 }  & {\bf 0.752 } &  {\bf 0.753 }  & {\bf 0.592 } & {\bf 0.594 } & {\bf 0.594 } \\
     \midrule
     \midrule
   {\bf Total top}  & {\bf 175}  & {\bf 1.370}   & {\bf 1.139} & {\bf 1.102} & {\bf 0.868} & {\bf 0.839} & {\bf 0.848}    \\
     \midrule
     \midrule
     {\bf Total dataset}   &  {\bf 4710} & {\bf 1.156}  & {\bf 1.145} & {\bf 1.144} & {\bf 1.138} & {\bf 1.135} & {\bf 1.126}  \\
 \bottomrule
\end{tabular}
\end{center}
  \caption{\small \label{tab:chi2-single-top}
     Same as Table~\ref{tab:chi2-top} now
    for the  inclusive and associated single-top production datasets.
    %
    Values in italics indicate datasets 
    that do not enter the corresponding fits: for those processes,
    we evaluate a posteriori the physical observables and the associated
    $\chi^2$ values using the resulting PDFs from the fit.
    %
    The last row indicates the total values adding together the non-top
    and top data contributions to the $\chi^2$,
    and the next-to-last row the total top quark contribution.
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Chapters/appendices/top/tables/chi2_pdfs_top.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
  \begin{center}
  \renewcommand{\arraystretch}{1.30}
%\scriptsize
  \tiny
\begin{tabular}{ l | c| C{1.2cm} | C{1.2cm} | C{0.8cm} | C{1.2cm} | C{1.0cm} | C{1.2cm} }
 \toprule
 \multirow{3}{*}{Dataset}    & \multirow{3}{*}{$n_{\rm dat}$}   &  \multicolumn{6}{c}{$\chi^2/n_{\rm dat}$}  \\[1.5ex]
 &   & \multicolumn{3}{c|}{\bf SM-PDF fits} & \multicolumn{2}{c|}{\bf Fixed-PDF EFT fits}   & {\bf SMEFT-PDFs}    \\
  &   & NNPDF4.0 (no top)  & NNPDF4.0 & Fit H & NNPDF4.0 (no top) & Fit H & Joint fit   \\
 \midrule
 \midrule
    ATLAS $\sigma(t\bar{t})$, dilepton, 7 TeV    & 1    &   \textit{4.100}  & 4.540 & 4.599 & 1.733 & 1.824 & 1.974     \\
    ATLAS $\sigma(t\bar{t})$, dilepton, 8 TeV & 1 & \textit{0.005} & 0.021 & 0.023 & 0.405 & 0.382 & 0.307 \\
    ATLAS $1/\sigma d\sigma/dm_{t\bar{t}}$, dilepton, 8 TeV & 5 & \textit{0.262} & \textit{0.284} & 0.291 & 0.305 & 0.309 & 0.310  \\
    ATLAS $\sigma(t\bar{t})$, $\ell+$jets, 8 TeV & 1 & \textit{0.218} & \textit{0.270} & 0.277 & 0.002 & 0.001  & 0.000  \\
    ATLAS $1/\sigma d\sigma/d|y_t|$, $\ell+$jets, 8 TeV & 4 & \textit{6.266} & 3.219 & 2.827 & 1.178 & 1.021 & 1.144 \\
    ATLAS $1/\sigma d\sigma/d|y_{t\bar{t}}|$, $\ell+$jets, 8 TeV & 4 & \textit{7.978} & 3.725 & 3.332 & 2.883 & 2.105 & 2.646  \\
    ATLAS $\sigma(t\bar{t})$, dilepton, 13 TeV           & 1    &  \textit{1.388}  & \textit{1.397}  & 1.374 & 0.004 & 0.004 & 0.002    \\
    ATLAS $\sigma(t\bar{t})$, hadronic, 13 TeV         & 1    & \textit{0.231}   &  \textit{0.231} & 0.230 & 0.082 & 0.082  & 0.092    \\
    ATLAS $1/\sigma d^2\sigma/d|y_{t\bar{t}}|dm_{t\bar{t}}$, hadronic, 13 TeV & 10 & \textit{2.276}  & \textit{2.007}  & 1.928 & 1.915 & 1.824 & 1.857  \\
    ATLAS $\sigma(t\bar{t})$, $\ell+$jets, 13 TeV & 1 & \textit{0.489} & 0.492 & 0.485 & 0.004 & 0.004 & 0.013 \\
    ATLAS $1/\sigma d\sigma/dm_{t\bar{t}}$, $\ell+$jets, 13 TeV & 8 & \textit{1.607} & \textit{1.788}  & 1.835 & 2.087 & 2.072 & 2.090  \\
    \midrule
    CMS $\sigma(t\bar{t})$, combined, 5 TeV & 1 & \textit{0.442}  & 0.542 & 0.555 & 0.211 & 0.236 & 0.239  \\
    CMS $\sigma(t\bar{t})$, combined, 7 TeV & 1 & \textit{0.795} & 1.032 & 1.065 & 0.004 & 0.010 & 0.027  \\
    CMS $\sigma(t\bar{t})$, combined, 8 TeV & 1 & \textit{0.170} & 0.247 & 0.258 & 0.174 & 0.156 & 0.103  \\
    CMS $1/\sigma d^2\sigma/d|y_{t\bar{t}}|dm_{t\bar{t}}$, dilepton, 8 TeV & 16 & \textit{1.094}  & \textit{0.994} & 0.963  & 0.519 & 0.580 & 0.514  \\
    CMS $1/\sigma d\sigma/d|y_{t\bar{t}}|$, $\ell+$jets, 8 TeV & 9 & \textit{2.127} &1.245 & 1.131 & 0.928 & 0.995 & 0.935  \\
    CMS $\sigma(t\bar{t})$, dilepton, 13 TeV & 1 & \textit{0.064}  & 0.063 & 0.066 & 0.680 & 0.680 & 0.600  \\
    CMS $1/\sigma d\sigma/dm_{t\bar{t}}$, dilepton, 13 TeV & 5 & \textit{2.760}  & 2.550 & 2.485 & 2.246 & 2.232 & 2.194  \\
    CMS $\sigma(t\bar{t})$, $\ell+$jets, 13 TeV & 1 & \textit{0.230} & \textit{0.227} & 0.234 & 2.153 & 2.155  & 1.907  \\
    CMS $1/\sigma d\sigma/dm_{t\bar{t}}$, $\ell+$jets, 13 TeV & 14 & \textit{1.829}  & \textit{1.481} & 1.393 & 0.962 & 0.911 & 0.912  \\
    \midrule
    ATLAS charge asymmetry, 8 TeV & 1 & \textit{0.679}  & \textit{0.678} & 0.675 & 0.567 & 0.587 & 0.571 \\
    ATLAS charge asymmetry, 13 TeV & 5 & \textit{1.012} & \textit{0.997} & 0.989 & 0.872 & 0.786 & 0.836 \\
    CMS charge asymmetry, 8 TeV & 3 & \textit{0.052} & \textit{0.052} & 0.053 & 0.072 & 0.069  & 0.071\\
    CMS charge asymmetry, 13 TeV & 3 & \textit{0.277} & \textit{0.283} & 0.286 & 0.443 & 0.510 & 0.451  \\
    ATLAS \& CMS combined charge asy., 8 TeV & 6 & \textit{0.603}  &\textit{0.602} & 0.602 & 0.646 & 0.659 & 0.651  \\
    \midrule
    ATLAS $W$-hel., 13 TeV & 2 & \textit{0.370} & \textit{0.370} & \textit{0.370} & 0.037 & 0.037 & 0.038   \\
    ATLAS \& CMS combined $W$-hel., 8 TeV & 2 & \textit{1.046} & \textit{1.046} & \textit{1.046} & 0.853 & 0.853 & 0.854  \\
       \midrule
   {\bf Total inclusive $t\bar{t}$}  & {\bf 108}  &  {\bf 1.700 } &  {\bf 1.328 } & {\bf 1.271 } & {\bf 1.032 } & {\bf 0.994} & {\bf 1.002 }  \\
     \midrule
     \midrule
    ATLAS $\sigma(t\bar{t}Z)$, 8 TeV & 1 & \textit{0.264}  &   \textit{0.232}  & 0.235 & 1.331 & 1.161 & 1.258 \\
    ATLAS $\sigma(t\bar{t}W)$, 8 TeV & 1 &  \textit{2.461} &  \textit{2.482} & 2.430 & 0.751 & 0.708 & 0.722   \\
    ATLAS $\sigma(t\bar{t}Z)$, 13 TeV & 1 &  \textit{0.702} &  \textit{0.747} & 0.742 & 0.001 & 0.000 & 0.000  \\
    ATLAS $1/\sigma d\sigma(t\bar{t}Z)/dp_T^Z$, 13 TeV & 5 &  \textit{1.961}  &  \textit{1.940} & 1.933 & 1.870 & 1.840 & 1.860  \\
    ATLAS $\sigma(t\bar{t}W)$, 13 TeV & 1 &  \textit{1.436} &  \textit{1.456} & 1.417 & 0.000 & 0.002 & 0.000 \\
    \midrule
    ATLAS $\sigma(t\bar{t}\gamma)$, 8 TeV & 1 & \textit{0.426} & \textit{0.426} & \textit{0.426} & 0.037 & 0.009 & 0.034  \\
    \midrule
    ATLAS $\sigma(t\bar{t}t\bar{t})$, multi-lepton, 13 TeV & 1 & \textit{3.655} & \textit{3.655} & \textit{3.655} & 4.289 & 3.784 & 4.145  \\
    ATLAS $\sigma(t\bar{t}t\bar{t})$, single lepton, 13 TeV & 1 & \textit{0.872} & \textit{0.872} & \textit{0.872} & 0.997 & 0.898 & 0.969  \\
    ATLAS $\sigma(t\bar{t}b\bar{b})$, $\ell+$jets, 13 TeV & 1 & \textit{2.062} & \textit{2.062} & \textit{2.062} & 1.093 & 1.316 & 1.152  \\
       \midrule
    CMS $\sigma(t\bar{t}Z)$, 8 TeV & 1 &  \textit{0.432}  &  \textit{0.470} & 0.466 & 0.005 & 0.020 & 0.010 \\
    CMS $\sigma(t\bar{t}W)$, 8 TeV & 1 &  \textit{2.281}  &  \textit{2.298} & 2.255 & 0.808 & 0.770 & 0.783  \\
    CMS $\sigma(t\bar{t}Z)$, 13 TeV & 1 &  \textit{1.185}  &  \textit{1.238} & 1.233 & 0.085 & 0.113 & 0.110 \\
    CMS $1/\sigma d\sigma(t\bar{t}Z)/dp_T^Z$, 13 TeV & 3 &  \textit{0.628}  &  \textit{0.598} & 0.590 & 0.936 & 0.756 & 0.898 \\
    CMS $\sigma(t\bar{t}W)$, 13 TeV & 1 &  \textit{0.667} &  \textit{0.682} & 0.652 & 0.297 & 0.329 & 0.307  \\
    \midrule
    CMS $\sigma(t\bar{t}\gamma)$, 8 TeV & 1 & \textit{0.508} & \textit{0.508} & \textit{0.508} & 0.022 & 0.045 & 0.024 \\
    \midrule
    CMS $\sigma(t\bar{t}t\bar{t})$, multi-lepton, 13 TeV & 1 & \textit{0.027} & \textit{0.027} & \textit{0.027} & 0.124 & 0.041 & 0.096  \\
    CMS $\sigma(t\bar{t}t\bar{t})$, single lepton, 13 TeV & 1 & \textit{0.231} & \textit{0.231} & \textit{0.231} & 0.262 & 0.238 & 0.255 \\
    CMS $\sigma(t\bar{t}b\bar{b})$, all-jet, 13 TeV & 1 & \textit{1.878} & \textit{1.878} & \textit{1.878} & 1.334 & 1.466 & 1.369  \\
    CMS $\sigma(t\bar{t}b\bar{b})$, dilepton, 13 TeV & 1 & \textit{0.962} & \textit{0.962} & \textit{0.962} & 0.312 & 0.447 & 0.347  \\
    CMS $\sigma(t\bar{t}b\bar{b})$, $\ell+$jets, 13 TeV & 1 & \textit{0.900} & \textit{0.900} & \textit{0.900} & 0.135 & 0.269 & 0.167  \\
    \midrule
   {\bf Total associated $t\bar{t}$}  & {\bf 26}  &  {\bf 1.255 } &  {\bf 1.255 } & {\bf 1.246 } & {\bf 0.925 } & {\bf 0.888 } & {\bf 0.913 } \\
%     \midrule
%     \midrule
%   {\bf Total top}  & {\bf 260}  &   &    \\
%     \midrule
%     \midrule
%     {\bf Grand total across all non-top \& top data}   &  {\bf 4022} & 1.1623  & 1.1627  \\
 \bottomrule
\end{tabular}
\end{center}
  \caption{\small \label{tab:chi2-top}
    Same as Table~\ref{tab:chi2-baseline} now
    for the  inclusive and associated $t\bar{t}$ production datasets.
    %
     Values in italics indicate datasets 
    that do not enter the corresponding SM-PDF fit: for those processes,
    we evaluate a posteriori the physical observables and the associated
    $\chi^2$ values using the resulting PDFs from the fit.
    %
    For instance, top data is removed from the \nnpdfnotop,
    and for some top quark observables like $t\bar{t}t\bar{t}$ their
    PDF dependence is neglected.
    %
      The last row indicates the total values adding together the non-top
    and top data contributions to the $\chi^2$.
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Chapters/appendices/top/tables/table-dataset-selection-CMS.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
{\fontsize{8pt}{8pt}\selectfont
%\begin{table}[t]
  \centering
   \renewcommand{\arraystretch}{2}
   \setlength{\tabcolsep}{5pt}
   \begin{tabularx}{\textwidth}{ccXccccl}
  \toprule
  \textbf{Experiment}
  &\textbf{$\sqrt{s}$ (TeV)}
  &\textbf{Observable}
  & \textbf{$n_{\rm dat}$}
  & $\chi^2_{\rm exp}/n_{\rm dat}$
  & \textbf{$n_\sigma$}
  & $Z$
  & \textbf{flag} \\
    %%%%%%%%%%%%%%% CMS %%%%%%%%%%%%%%%%%%%%%%%
  \midrule
  CMS
  & 5
  & $\sigma_{t\bar{t}}^{\rm tot}$, combination
  & 1
  & 0.56
  & -0.31
  & 1.00
  & no \\
%----------------
  & 7
  & $\sigma_{t\bar{t}}^{\rm tot}$, combination
  & 1
  & 1.08
  & 0.06
  & 1.00
  & no \\
%----------------
  & 
  & $\sigma^{\rm tot}(t) + \sigma^{\rm tot}(\bar{t})$, $t$-channel
  & 1
  & 0.72
  & -0.20
  & 1.00
  & no \\
%----------------
  & 8
  & $\sigma_{t\bar{t}}^{\rm tot}$, combination
  & 1
  & 0.27 
  & -0.52
  & 1.00
  & no \\
   & 
  & $1/\sigma d^2\sigma/dy_{t\bar{t}}dm_{t\bar{t}}$, dilepton 
  & 16
  & 0.98
  & -0.06
  & 2.33
  & no \\
   & 
  & $1/\sigma d\sigma/dy_{t\bar{t}}$, $\ell+$jets 
  & 9
  & 1.15
  & 0.31
  & 1.63
  & no \\
  & 
  & $A_C$, dilepton
  & 3
  & 0.05
  & -1.16
  & 1.16
  & no \\
  & 
  & $\sigma(t\bar{t}Z)$
  & 1
  & 0.47
  & -0.37
  & 1.00
  & no\\
  & 
  & $\sigma(t\bar{t}W)$
  & 1
  & {\bf 2.27}
  & 0.90
  & 1.00
  &  no\\
%----------------
  & 
  & $\sigma^{\rm tot}(t)$, $t$-channel
  & 1
  & 0.01
  & -0.70
  & 1.00
  & no \\
%----------------
  & 
  & $\sigma^{\rm tot}(\bar{t})$, $t$-channel
  & 1
  & 0.09
  & -0.64
  & 1.00
  & no \\
%----------------
  & 
  & $\sigma^{\rm tot}(t + \bar{t})$, $s$-channel
  & 1
  & 1.11 
  & 0.08
  & 1.00
  & no \\
%----------------
  & 
  & $\sigma^{\rm tot}(t W)$, dilepton
  & 1
  & 0.38
  & -0.44
  & 1.00
  & no \\
%---------------
   & 13
  & $\sigma_{t\bar{t}}^{\rm tot}$, dilepton  
  & 1
  & 0.06 
  & -0.66
  & 1.00
  & no \\
   & 
  & $1/\sigma d\sigma/dm_{t\bar{t}}$, dilepton  
  & 5
  & {\bf 2.49}
  & 2.36 
  & 1.61
  & no\\
   & 
  & $\sigma_{t\bar{t}}^{\rm tot}$, $\ell+$jets channel
  & 1
  & 0.22
  & -0.55
  & 1.00
  & no \\
%%%%%%%%%%%%%%%%%
   & 
  & $1/\sigma d\sigma/dm_{t\bar{t}}$, $\ell+$jets
  & 14
  & 1.41 
  & 1.08
  & {\bf 4.57}
  & no \\
  %%%%%%%%%%%%%%%%%
   & 
  & $1/\sigma d\sigma/dm_{t\bar{t}}dy_{t}$, $\ell+$jets
  & 34
  & {\bf 6.43} 
  & 22.4
  & 3.88
  & {\bf yes (excl)} \\
  & 
  & $A_C$, $\ell+$jets
  & 3
  & 0.29
  & -0.87
  & 1.00
  & no \\
  & 
  & $\sigma(t\bar{t}Z)$
  & 1
  & 1.24
  & 0.17
  & 1.00
  &  no \\
  & 
  & $1/\sigma d\sigma(t\bar{t}Z)/dp_T(Z)$
  & 3
  & 0.59
  & -0.50
  & 1.28
  &  no\\
  & 
  & $\sigma(t\bar{t}W)$
  & 1
  & 0.66
  & -0.24
  & 1.00
  &  no \\
% ----------------------
  & 
  & $\sigma^{\rm tot}(t)$, $t$-channel
  & 1
  & 0.88
  & -0.08
  & 1.00
  &  no \\
% ----------------------
  & 
  & $\sigma^{\rm tot}(\bar{t})$, $t$-channel
  & 1
  & 0.13 
  & -0.62
  & 1.00
  &  no \\
% ----------------------
  & 
  & $1/\sigma d\sigma/d|y^{(t)}|$, $t$-channel
  & 4
  & 0.38
  & -0.88
  & 1.70
  &  no \\
% ----------------------
  & 
  & $\sigma^{\rm tot}(tW)$, dilepton
  & 1
  & 0.43  
  & -0.40
  & 1.00
  &  no \\
% ----------------------
  & 
  & $\sigma^{\rm tot}(tW)$, single-lepton
  & 1
  & {\bf 2.84} 
  & 1.30
  & 1.00
  &  no \\
  \midrule
  ATLAS-CMS combination
  & 8
  & $A_C$, $\ell$+jets
  & 6
  & 0.602
  & -0.69
  & 1.65
  & no \\
  \bottomrule
   \end{tabularx}
   \vspace{0.3cm}
  \caption{\small Same as Table \ref{tab:datasets_selection_atlas} for the
    CMS and combined ATLAS-CMS datasets. \textit{Note carefully:} the row
    corresponding to the CMS doubly-differential distribution at 13 TeV in the $\ell+$jets
    channel comes from a separate fit, where the corresponding 1D distribution is replaced
    by this dataset.
   \label{tab:datasets_selection_cms}
}
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> Chapters/appendices/top/tables/table-dataset-selection.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
  \begin{center}
{\fontsize{8pt}{8pt}\selectfont
%\begin{table}[t]
  \centering
   \renewcommand{\arraystretch}{2}
   \setlength{\tabcolsep}{5pt}
   \begin{tabularx}{\textwidth}{ccXccccl}
  \toprule
  \textbf{Experiment}
  &\textbf{$\sqrt{s}$ (TeV)}
  &\textbf{Observable, Channel}
  & \textbf{$n_{\rm dat}$}
  & $\chi^2_{\rm exp}/n_{\rm dat}$
  & \textbf{$n_\sigma$}
  & $Z$
  & \textbf{flag}\\
  \midrule
 %----------------------------
  {\bf ATLAS }
  & 7
  & $\sigma_{t\bar{t}}^{\rm tot}$, dilepton
  & 1
  & {\bf 4.63}  
  & 2.57
  & 1.00
  & no  \\
%---------------------------
  & 
  & $\sigma^{\rm tot}(t)$, $t$-channel
  & 1
  &  0.76 
  & -0.17
  & 1.00
  & no  \\
%---------------------------
  & 
  & $\sigma^{\rm tot}(\bar{t})$, $t$-channel
  & 1
  &  0.29
  & -0.50
  & 1.00
  & no  \\
%---------------------------
  & 
  & $1/\sigma d(tq)/dy_t$, $t$-channel
  & 3
  & 0.97 
  & -0.04
  & 1.28
  & no  \\
%---------------------------
  & 
  & $1/\sigma d(\bar{t}q)/dy_{\bar{t}}$, $t$-channel
  & 3
  & 0.06 
  & -1.15
  & 1.39
  & no  \\ \midrule
 %----------------------------
  & 8
    & $\sigma_{t\bar{t}}^{\rm tot}$, dilepton
  & 1
  & 0.03
  & -0.69
  & 1.00
  & no \\
    &
    & $1/\sigma d\sigma/dm_{t\bar{t}}$, dilepton
  & 5
  & 0.29
  & -1.12
  & 1.61
  & no \\
    &
    & $\sigma_{t\bar{t}}^{\rm tot}$, $\ell+$jets 
  & 1
  & 0.28 
  & -0.51
  & 1.00 
  & no \\
     &
     & $1/\sigma d\sigma/d|y_t|$, $\ell+$jets
  & 4
  & {\bf 2.86} 
  & 2.63 
  & 1.65
  & no \\
  &
     & $1/\sigma d\sigma/d|y_{t\bar{t}}|$, $\ell+$jets 
  & 4
  & {\bf 3.37}
  & {\bf 3.35}
  & 2.19 
  & {\bf yes (kept)} \\
  &
  & $A_C$, dilepton
  & 1
  & 0.67
  & -0.23
  & 1.00
  & no\\
  & 
  & $\sigma(t\bar{t}Z)$
  & 1
  & 0.23
  & -0.54
  & 1.00
  & no \\
  & 
  & $\sigma(t\bar{t}W)$
  & 1
  & {\bf 2.44}
  & 1.01
  & 1.00
  &  no \\
%---------------------------
  & 
  & $\sigma^{\rm tot}(t + \bar{t})$, $s$-channel
  & 1
  & 0.21 
  & -0.56
  & 1.00
  & no  \\
%---------------------------
  & 
  & $\sigma^{\rm tot}(t W)$, dilepton
  & 1
  & 0.54 
  & -0.33
  & 1.00
  & no  \\
%---------------------------
  & 
  & $\sigma^{\rm tot}(t W)$, single-lepton
  & 1
  & 0.71  
  & -0.21
  & 1.00
  & no  \\
  \midrule
%-------------------------
 &13
  & $\sigma_{t\bar{t}}^{\rm tot}$, dilepton
  & 1
  & 1.41
  & 0.29
  & 1.00
  & no \\
     &
     & $\sigma_{t\bar{t}}^{\rm tot}$, hadronic
  & 1
  & 0.23 
  & -0.54
  & 1.000
  & no \\
     &
     & $1/\sigma d^2\sigma/d|y_{t\bar{t}}|dm_{t\bar{t}}$, hadronic 
  & 10
  & 1.95 
  & 2.12
  & 2.33
  & no\\ 
     &
     & $\sigma_{t\bar{t}}^{\rm tot}$, $\ell+$jets 
  & 1
  & 0.50
  & -0.35
  & 1.00 
  & no\\ 
     &
     & $1/\sigma d\sigma/dm_{t\bar{t}}$, $\ell+$jets
  & 8
  & 1.83
  & 1.66
  & {\bf 7.61}
  & no\\
  &
  & $A_C$, $\ell+$jets
  & 5
  & 0.99
  & -0.02
  & 1.41
  & no\\
  & 
  & $\sigma(t\bar{t}Z)$
  & 1
  & 0.75
  & -0.18
  & 1.00
  &  no \\
  &
  & $1/\sigma d\sigma(t\bar{t}Z)/dp_T(Z)$
  & 5
  & 1.93
  & 1.47
  & 2.27 
  & no\\
  &
  & $\sigma(t\bar{t}W)$
  & 1
  & 1.43
  & 0.30
  & 1.00 
  & no\\
%---------------------------
  & 
  & $\sigma^{\rm tot}(t)$, $t$-channel
  & 1
  & 0.72  
  & -0.20
  & 1.00
  & no  \\
%---------------------------
  & 
  & $\sigma^{\rm tot}(\bar{t})$, $t$-channel
  & 1
  & 0.39 
  & -0.43
  & 1.00
  & no  \\
%---------------------------
  & 
  & $\sigma^{\rm tot}(t + \bar{t})$, $s$-channel
  & 1
  & 0.70
  & -0.21
  & 1.00
  & no  \\
%---------------------------
  & 
  & $\sigma^{\rm tot}(t W)$, dilepton
  & 1
  & 1.15
  & 0.36
  & 1.00
  & no  \\
%-------------------------
  \bottomrule
   \end{tabularx}
   \vspace{0.3cm}
   \caption{\small For the ATLAS measurements that we consider in this work,
     we list the outcome of a global SM-PDF fit with all
     measurements listed in
     Tables~\ref{tab:input_datasets_toppair}-\ref{tab:input_datasets_4}
     included.
     %
     We display for each dataset the  number of
data points, the $\chi^2$ per data point (Eq.~\eqref{eq:chi2exp}, the number of
standard deviations $n_\sigma$ (Eq.~\eqref{eq:nsigma}), and the
stability metric $Z$  defined in~\cite{Kassabov:2022pps}.
%
The entries that lie above the corresponding threshold values
are  highlighted in boldface,
%
In the
last column, we indicate whether the dataset is flagged and
is either kept or removed.
%
See text for more details.
%\JM{Note that currently, the final two datasets overlap.}
   \label{tab:datasets_selection_atlas}
}
}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> Chapters/appendices/top/tables/table-input-dataset-top1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h!]
  \begin{center}
{\fontsize{8pt}{8pt}\selectfont
%\begin{table}[t]
  \centering
   \renewcommand{\arraystretch}{1.5}
   \setlength{\tabcolsep}{2pt}
   \begin{tabular}{lcccccc|c|c}
     \toprule \textbf{Exp.}   & $\bf{\sqrt{s}}$ \textbf{(TeV)}    &   \textbf{Channel}
    &  \textbf{Observable} & $\mathcal{L}$ (fb${}^{-1}$) & $\mathbf{n_{\rm dat}}$ & \textbf{Ref.}
     &\textbf{New (PDF fits)}
    &  \textbf{New (SMEFT fits)}\\
    \toprule
    \multirow{1}{*}{
      \bf ATLAS}
      & 7
      & dilepton
      & $\sigma(t\bar{t})$
      & $4.6$
      & 1
      & \cite{ATLAS:2014nxi}
      &
      & ($\checkmark$)\\\midrule
%-------------------------------------------------------------------------------
      & 8
      & dilepton
      & $\sigma(t\bar{t})$
      & $20.3$
      & 1
      & \cite{ATLAS:2014nxi}
      &
      & ($\checkmark$)\\
%-------------------------------------------------------------------------------
      & 
      & 
      & $1/\sigma d\sigma/dm_{t\bar{t}}$
      & $20.2$
      & 5
      & \cite{Aaboud:2016iot}
      & ($y_{t\bar{t}} \rightarrow m_{t\bar{t}}$)
      & (absolute $\rightarrow$ ratio)\\
%-------------------------------------------------------------------------------
      & 
      & $\ell+$jets
      & $\sigma(t\bar{t})$
      & $20.2$
      & 1
      & \cite{ATLAS:2017wvi}
      & $\checkmark$
      & ($\checkmark$)\\
%-------------------------------------------------------------------------------
      & 
      & 
      & $1/\sigma d\sigma/d|y_{t}|$
      & $20.3$
      & 4
      & \cite{Aad:2015mbv}
      &
      & ($m_{t\bar{t}}, p_t^T \rightarrow |y_t|, |y_{t\bar{t}}|$)\\
%-------------------------------------------------------------------------------
      & 
      &
      & $1/\sigma d\sigma/d|y_{t\bar{t}}|$
      & $20.3$
      & 4
      & \cite{Aad:2015mbv}
      &
      & ($m_{t\bar{t}}, p_t^T \rightarrow |y_t|, |y_{t\bar{t}}|$)\\\midrule
%-------------------------------------------------------------------------------
      & 13
      & dilepton
      & $\sigma(t \bar{t})$
      & $36.1$
      & 1
      & \cite{ATLAS:2019hau}
      & $\checkmark$
      & $\checkmark$\\
%-------------------------------------------------------------------------------
      &
      & hadronic
      & $\sigma(t \bar{t})$
      & $36.1$
      & 1
      & \cite{ATLAS:2020ccu}
      & $\checkmark$
      & $\checkmark$\\
%-------------------------------------------------------------------------------
      &
      &
      & $1/\sigma d^2\sigma/d|y_{t\bar{t}}|dm_{t\bar{t}}$
      & $36.1$
      & 10
      & \cite{ATLAS:2020ccu}
      & $\checkmark$
      & $\checkmark$\\
%-------------------------------------------------------------------------------
      & 
      & $\ell+$jets
      & $\sigma(t \bar{t})$
      & $139$
      & 1
      & \cite{ATLAS:2020aln}
      & 
      & ($\checkmark$) \\
%-------------------------------------------------------------------------------
      &
      & 
      & $1/\sigma d\sigma/dm_{t\bar{t}}$
      & $36$
      & 8
      & \cite{Aad:2019ntk}
      & $\checkmark$
      & (absolute $\rightarrow$ ratio)\\
%-------------------------------------------------------------------------------
     \midrule \midrule
       \multirow{1}{*}{\bf CMS}      & 5
      & combination
      & $\sigma(t \bar{t})$
      & 0.027
      & 1
      & \cite{CMS:2017zpm}
      & 
      & $\checkmark$\\ \midrule
%-------------------------------------------------------------------------------
      & 7
      & combination
      & $\sigma(t \bar{t})$
      & $5.0$
      & 1
      & \cite{Spannagel:2016cqt}
      & 
      & $\checkmark$\\\midrule
%-------------------------------------------------------------------------------
      & 8
      & combination
      & $\sigma(t \bar{t})$
      & $19.7$
      & 1
      & \cite{Spannagel:2016cqt}
      & 
      & $\checkmark$\\     
%-------------------------------------------------------------------------------
      &
      & dilepton
      & $1/\sigma d^2\sigma/dy_{t\bar{t}}dm_{t\bar{t}}$
      & $19.7$
      & 16
      & \cite{Sirunyan:2017azo}
      & ($m_{t\bar{t}}, y_t \rightarrow m_{t\bar{t}}, y_{t\bar{t}}$)
      & \\
%-------------------------------------------------------------------------------
      &
      & $\ell+$jets
      & $1/\sigma d\sigma/dy_{t\bar{t}}$
      & $19.7$
      & 9
      & \cite{Khachatryan:2015oqa}
      & 
      & \\\midrule
%-------------------------------------------------------------------------------
	& 13
	& dilepton
	& $\sigma(t \bar{t})$
	& $43$
	  & 1
	  & \cite{CMS:2015yky}
      & 
      & ($\checkmark$)\\
%-------------------------------------------------------------------------------
      &
      &
       & $1/\sigma d\sigma/dm_{t\bar{t}}$
       & $35.9$
      & 5
      & \cite{Sirunyan:2018ucr}
      & % (? - different reference?) MU: clicking on the refs they
        % point to the same .pdf 
      & (absolute $\rightarrow$ ratio)\\   
%-------------------------------------------------------------------------------
	& 
	& $\ell+$jets
	& $\sigma(t \bar{t})$
	& $137$
        & 1
        & \cite{CMS:2021vhb}
        & $\checkmark$
       & $\checkmark$\\
%-------------------------------------------------------------------------------
      &
      & 
      & $1/\sigma  d\sigma/dm_{t\bar{t}}$
      & $137$
      & 14
      & \cite{CMS:2021vhb}
        & $\checkmark$
       & $\checkmark$\\     
%%-------------------------------------------------------------------------------
% This is the double-differential distribution which we elect not to use.
%      &
%      & 
%      & $1/\sigma  d^2\sigma/d|y_{t\bar{t}}|dm_{t\bar{t}}$
%      & 34/35
%      & \cite{CMS:2021vhb}
%        & $\checkmark$
%       & $\checkmark$\\       
\bottomrule
   \end{tabular}
   \vspace{0.3cm}
   \caption{\small
    The inclusive cross-sections and differential distributions
    for top quark pair production from ATLAS
    and CMS that we consider in this analysis.
    %
    For each dataset, we indicate the experiment,
    the centre of mass energy $\sqrt{s}$, the final-state
    channel, the observable(s) used in the fit, the integrated luminosity $\mathcal{L}$ in inverse femtobarns, and the
    number of data points $n_{\rm dat}$, together
    with the corresponding publication reference.
%
    In the last two columns, we indicate
    with a $\checkmark$ the datasets
    that are included for the first time here in a global PDF fit
    and in a SMEFT interpretation, respectively.
  %
    The sets marked with brackets have already been included in
    previous studies but here we account for their constraints
    in different manner (e.g. by changing spectra or normalisation), as indicated in the table and in the
    text description.
    \label{tab:input_datasets_toppair}
}
}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Chapters/appendices/top/tables/table-input-dataset-top1b.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h!]
  \begin{center}
{\fontsize{8pt}{8pt}\selectfont
%\begin{table}[t]
  \centering
   \renewcommand{\arraystretch}{1.5}
   \setlength{\tabcolsep}{2pt}
   \begin{tabular}{lcccccc|c|c}
     \toprule \textbf{Experiment}     & $\bf{\sqrt{s}}$\textbf{(TeV)}
     & \textbf{Channel}  &  \textbf{Observable} & $\mathcal{L}$ (fb${}^{-1}$) & $\mathbf{n_{\rm dat}}$ & \textbf{Ref.}   &\textbf{New (PDF fits)}
    &  \textbf{New (SMEFT fits)} \\
    \toprule
      \multirow{2}{*}{ATLAS}
      & 8
      & dilepton
      & $A_C$
      & $20.3$
      & 1
      & \cite{Aad:2016ove}
      & $\checkmark$                                                                     
      &  \\
%-------------------------------------------------------------------------------
      & 13
      & $\ell+$jets
      & $A_C$
      & $139$
      & 5
      & \cite{ATLAS:2022waa}
      & $\checkmark$                                                                     
      & $\checkmark$   \\
%-------------------------------------------------------------------------------
     \midrule
      \multirow{2}{*}{CMS}
      & 8
      & dilepton
      & $A_C$
      & $19.5$
      & 3
      & \cite{Khachatryan:2016ysn}
      & $\checkmark$                                                                     
      &  \\
%-------------------------------------------------------------------------------
      & 13
      & $\ell+$jets
      & $A_C$
      & $138$
      & 3
      & \cite{CMS-PAS-TOP-21-014}
      & $\checkmark$                                                                     
      &  \\
%-------------------------------------------------------------------------------
\midrule
      ATLAS/CMS comb.
      & 8
      & $\ell+$jets
      & $A_C$
      & $20$
      & 6
      & \cite{Sirunyan:2017lvd}
      & $\checkmark$                                                                     
      &  \\
\bottomrule
   \end{tabular}
   \vspace{0.3cm}
   \caption{\small Same as Table~\ref{tab:input_datasets_toppair} for the $t\bar{t}$
     asymmetry datasets.
   \label{tab:input_datasets_topasymmetries} \label{tab:asymmetries}
}
}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Chapters/appendices/top/tables/table-input-dataset-top1c.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h!]
  \begin{center}
{\fontsize{7pt}{7pt}\selectfont
%\begin{table}[t]
  \centering
   \renewcommand{\arraystretch}{2}
   \setlength{\tabcolsep}{5pt}
   \begin{tabular}{lccccc|c}
     \toprule \textbf{Experiment}     & $\bf{\sqrt{s}}$\textbf{(TeV)}
     &   \textbf{Observable} & $\mathcal{L}$ (fb${}^{-1}$) & $\mathbf{n_{\rm dat}}$ & \textbf{Ref.}   
    &  \textbf{New (SMEFT fits)} \\
     \toprule
           ATLAS \& CMS combination
      & 8
      & $F_0, F_L$
      & $20$
      & 2
      & \cite{Aad:2020jvx}
      &  \\
 \midrule
       ATLAS
      & 13
      & $F_0, F_L$
      & $139$
      & 2
      & \cite{ATLAS:2022bdg}
      & $\checkmark$     \\
\bottomrule
   \end{tabular}
   \vspace{0.3cm}
  \caption{\small Same as Table~\ref{tab:input_datasets_toppair} for
    the $W$-helicity fraction measurements.
    %
    These helicity fractions are PDF-independent and hence
    are only relevant in constraining the EFT coefficients.
    \label{tab:whelicities}
   \label{tab:input_datasets_helicityfractions}
}
}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Chapters/appendices/top/tables/table-input-dataset-top2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h!]
  \begin{center}
{\fontsize{8pt}{8pt}\selectfont
%\begin{table}[t]
  \centering
   \renewcommand{\arraystretch}{2}
   \setlength{\tabcolsep}{5pt}
   \begin{tabular}{lccccc|c|c}
     \toprule \textbf{Exp.}   & $\bf{\sqrt{s}}$ \textbf{(TeV)}    
    &  \textbf{Observable} & $\mathcal{L}$ (fb${}^{-1}$) & $\mathbf{n_{\rm dat}}$ & \textbf{Ref.}
     &\textbf{New (PDF fits)}
    &  \textbf{New (SMEFT fits)}\\
    \toprule
    {\bf ATLAS}
    & 8
    & $\sigma(t\bar{t}Z)$
    & $20.3$
    & 1
    &  \cite{Aad:2015eua}
      & $\checkmark$                                                                     
      &  \\
  %-----------------------------------------------------------------------------------------
    & 
    & $\sigma(t\bar{t}W)$
    & $20.3$
    & 1
    & \cite{Aad:2015eua}
      & $\checkmark$                                                                     
      &  \\\midrule
  %-----------------------------------------------------------------------------------------
    & 13
    & $\sigma(t\bar{t}Z)$
    & $36.1$
    & 1
    &\cite{Aaboud:2019njj}
       & $\checkmark$                                                                     
      &  \\
  %-----------------------------------------------------------------------------------------
    & 
    & $1/\sigma d\sigma(t\bar{t}Z)/dp_T^Z$
    & $139$
    & 6
    &  \cite{ATLAS:2021fzm}
      & $\checkmark$                                                                     
      & $\checkmark$ \\
  %-----------------------------------------------------------------------------------------
    & 
    & $\sigma(t\bar{t}W)$
    & $36.1$
    & 1
    &  \cite{Aaboud:2019njj}
      & $\checkmark$                                                                     
      &  \\
  %-----------------------------------------------------------------------------------------
  \midrule
     {\bf  CMS}
    & 8
    & $\sigma(t\bar{t}Z)$
    & $19.5$
    & 1
    & \cite{Khachatryan:2015sha}
       & $\checkmark$                                                                     
      &  \\
  %-----------------------------------------------------------------------------------------
    & 
    & $\sigma(t\bar{t}W)$
    & $19.5$
    & 1
    & \cite{Khachatryan:2015sha}
      & $\checkmark$                                                                     
      &  \\ \midrule
   %-----------------------------------------------------------------------------------------
    & 13
    & $\sigma(t\bar{t}Z)$
    & $35.9$
    & 1
    & \cite{Sirunyan:2017uzs}
        & $\checkmark$                                                                     
      &  \\
   %-----------------------------------------------------------------------------------------
    & 
    & $1/\sigma d\sigma(t\bar{t}Z)/dp_T(Z)$
    & $77.5$
    & 3
    & \cite{CMS:2019too}
      & $\checkmark$                                                                     
      & (absolute $\rightarrow$ ratio) \\
   %-----------------------------------------------------------------------------------------
    & 
    & $\sigma(t\bar{t}W)$
    & $35.9$
    & 1
    &  \cite{Sirunyan:2017uzs}
       & $\checkmark$                                                                     
      &  \\
\bottomrule
   \end{tabular}
   \vspace{0.3cm}
   \caption{\small Same as Table~\ref{tab:input_datasets_toppair} for the measurements
     of top quark production
     in association with a vector boson.
     \label{tab:input_datasets2}
   }
}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> Chapters/appendices/top/tables/table-input-dataset-top2b.tex <==
\begin{table}[h!]
{\fontsize{8pt}{8pt}\selectfont
%\begin{table}[t]
  \centering
   \renewcommand{\arraystretch}{2}
   \setlength{\tabcolsep}{5pt}
   \begin{tabular}{lccccc|c}
     \toprule \textbf{Experiment}     & $\bf{\sqrt{s}}$\textbf{(TeV)}
     &   \textbf{Observable} & $\mathcal{L}$ (fb${}^{-1}$) & $\mathbf{n_{\rm dat}}$ & \textbf{Ref.}   
    &  \textbf{New (SMEFT fits)} \\
    \toprule
    ATLAS
    & 8
    & $\sigma(t\bar{t}\gamma)$
    & $20.2$
    & 1
    &\cite{Aaboud:2017era}
    & \\
  %-----------------------------------------------------------------------------------------
%    & 13
%    & $d\sigma(t\bar{t}\gamma)/dp_T(\gamma)$
%    & $139$
%    & 11
%    &   \cite{Aad:2020axn}
%    & \\
  %-----------------------------------------------------------------------------------------
  \midrule
      CMS
    & 8
    & $\sigma(t\bar{t}\gamma)$
    & $19.7$
    & 1
    & \cite{Sirunyan:2017iyh}
    & \\
\bottomrule
   \end{tabular}
   \vspace{0.3cm}
  \caption{\small Same as Table~\ref{tab:input_datasets_toppair} for
     $t\bar{t}$ production in association with a photon.
    \label{tab:input_datasets2b}
    %
    Theory predictions for these observables adopt a fixed PDF.
   }
   }
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> Chapters/appendices/top/tables/table-input-dataset-top2c.tex <==
\begin{table}[h!]
  \begin{center}
{\fontsize{8pt}{8pt}\selectfont
%\begin{table}[t]
  \centering
   \renewcommand{\arraystretch}{2.3}
   \setlength{\tabcolsep}{5pt}
   \begin{tabular}{lcccccc|c}
     \toprule \textbf{Experiment}     & $\bf{\sqrt{s}}$\textbf{(TeV)}
     &   \textbf{Channel} & \textbf{Observable} & $\mathcal{L}$ (fb${}^{-1}$) & $\mathbf{n_{\rm dat}}$ & \textbf{Ref.}   
    &  \textbf{New (SMEFT fits)} \\
    \toprule
    ATLAS
    & 13
    & multi-lepton
    & $\sigma_{\text{tot}}(t\bar{t}t\bar{t})$
    & $139$
    & 1
    &\cite{ATLAS:2020hpj}
    & \\
  %-----------------------------------------------------------------------------------------
    & 
    & single-lepton
    & $\sigma_{\text{tot}}(t\bar{t}t\bar{t})$
    & $139$
    & 1
    & \cite{ATLAS:2021kqb}
    & $\checkmark$ \\
  %-----------------------------------------------------------------------------------------
        & 
    & $\ell+$jets
    & $\sigma_{\text{tot}}(t\bar{t}b\bar{b})$
    & $36.1$
    & 1
    & \cite{ATLAS:2018fwl}
    & \\
  %-----------------------------------------------------------------------------------------
  \midrule
      CMS
    % & 8
    % & dilepton
    % & $\sigma_{\text{tot}}(t\bar{t}b\bar{b})$
    % & 1
    % & \cite{CMS:2014yxa}
    % & $\checkmark$ \\
   %-----------------------------------------------------------------------------------------
     & 13
    & multi-lepton
    & $\sigma_{\text{tot}}(t\bar{t}t\bar{t})$
    & $137$
    & 1
    & \cite{CMS:2019rvj}
    &  \\
   %-----------------------------------------------------------------------------------------
     & 
    & single-lepton
    & $\sigma_{\text{tot}}(t\bar{t}t\bar{t})$
    & $35.8$
    & 1
    & \cite{CMS:2019jsc}
    &  \\
   %-----------------------------------------------------------------------------------------
     & 
    & all-jet
    & $\sigma_{\text{tot}}(t\bar{t}b\bar{b})$
    & $35.9$
    & 1
    & \cite{CMS:2019eih}
    &  \\
   %-----------------------------------------------------------------------------------------
     & 
    & dilepton
    & $\sigma_{\text{tot}}(t\bar{t}b\bar{b})$
    & $35.9$
    & 1
    & \cite{CMS:2020grm}
    & \\
   %-----------------------------------------------------------------------------------------
     & 
    & $\ell$+jets
    & $\sigma_{\text{tot}}(t\bar{t}b\bar{b})$
    & $35.9$
    & 1
    & \cite{CMS:2020grm}
    &$\checkmark$ \\
\bottomrule
   \end{tabular}
   \vspace{0.3cm}
  \caption{\small  Same as Table~\ref{tab:input_datasets_toppair} for
    the measurements of $t\bar{t}$ production in association with a heavy quark
    pair.
    %
    Theory predictions for these observables adopt a fixed PDF.
     \label{tab:input_datasets2c}
   }
}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> Chapters/appendices/top/tables/table-input-dataset-top3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!ht]
  \begin{center}
{\fontsize{8pt}{8pt}\selectfont
%\begin{table}[t]
  \centering
   \renewcommand{\arraystretch}{2}
   \setlength{\tabcolsep}{5pt}
   \begin{tabular}{lcccccc|c|c}
     \toprule \textbf{Exp.}   & $\bf{\sqrt{s}}$ \textbf{(TeV)}    &   \textbf{Channel}
    &  \textbf{Observable} & $\mathcal{L}$ (fb${}^{-1}$) & $\mathbf{n_{\rm dat}}$ & \textbf{Ref.}
     &\textbf{New (PDF fits)}
    &  \textbf{New (SMEFT fits)}\\
    \toprule
    {\bf ATLAS}
    & 7
    & $t$-channel
    & $\sigma_\text{tot}(t)$ 
    & $4.59$
    & 1
    & \cite{ATLAS:2014sxe}
      & ($\checkmark$)                                                                    
      &   $\checkmark$     \\
  %-----------------------------------------------------------------------------------------
    & 
    & 
    & $\sigma_\text{tot}(\bar{t})$ 
    & $4.59$
    & 1
    & \cite{ATLAS:2014sxe}
          & ($\checkmark$)                                                                    
      &   $\checkmark$     \\
  %-----------------------------------------------------------------------------------------
    & 
    &
    & $1/\sigma d\sigma(tq)/dy_t$ 
    & $4.59$
    & 3
    & \cite{ATLAS:2014sxe}
     &                                                                  
      & $\checkmark$       \\
  %-----------------------------------------------------------------------------------------
    & 
    &
    & $1/\sigma d\sigma(\bar{t}q)/dy_{\bar{t}}$ 
    & $4.59$
    & 3
    & \cite{ATLAS:2014sxe}
     &                                                                
    &  $\checkmark$      \\
    \midrule
   %-----------------------------------------------------------------------------------------
    & 8
    & $t$-channel
    & $\sigma_{\text{tot}}(t)$
    & $20.2$
    & 1
    & \cite{Aaboud:2017pdi}
      & ($\checkmark$)                                                                    
      &  $\checkmark$      \\
   %-----------------------------------------------------------------------------------------
    & 
    & 
    & $\sigma_{\text{tot}}(\bar{t})$
    & $20.2$
    & 1
    & \cite{Aaboud:2017pdi}
          & ($\checkmark$)                                                                    
      &   $\checkmark$     \\
  %-----------------------------------------------------------------------------------------
    & 
    &
    & $1/\sigma d\sigma(tq)/dy_t$ 
    & $20.2$
    & 3
    & \cite{Aaboud:2017pdi}
     &
       & ($\checkmark$)\\
  %-----------------------------------------------------------------------------------------
    & 
    &
    & $1/\sigma d\sigma(\bar{t}q)/dy_{\bar{t}}$ 
    & $20.2$
    & 3
    & \cite{Aaboud:2017pdi}
     &
       & ($\checkmark$)\\
  %-----------------------------------------------------------------------------------------
    & 
    & $s$-channel
    & $\sigma_{\text{tot}}(t + \bar{t})$
    & $20.3$
    & 1
    & \cite{Aad:2015upn} 
     & $\checkmark$
    & \\
    \midrule
  %-----------------------------------------------------------------------------------------
    & 13
    & $t$-channel
    & $\sigma_{\text{tot}}(t)$
    & $3.2$
    & 1
    & \cite{Aaboud:2016ymp}  
     & ($\checkmark$)
     & \\
  %-----------------------------------------------------------------------------------------
    & 
    &
    & $\sigma_{\text{tot}}(\bar{t})$
    & $3.2$
    & 1
    &  \cite{Aaboud:2016ymp}  
     & ($\checkmark$)
     & \\
  %-----------------------------------------------------------------------------------------
    & 
    & $s$-channel
    & $\sigma_{\text{tot}}(t + \bar{t})$ 
    & $139$
    & 1
    & \cite{ATLAS:2022wfk}
     & $\checkmark$
     & $\checkmark$\\
  %-----------------------------------------------------------------------------------------
    \midrule
    \midrule
      {\bf CMS}
     & 7
    & $t$-channel
    & $\sigma_{\text{tot}}(t) + \sigma_{\text{tot}}(\bar{t})$  
    & $1.17, 1.56$
    & 1
    & \cite{CMS:2012xhh}
     &
      & $\checkmark$\\
      \midrule
  %-----------------------------------------------------------------------------------------
    & 8
    & $t$-channel
    & $\sigma_{\text{tot}}(t)$
    & $19.7$
    & 1
    & \cite{Khachatryan:2014iya}
     & ($\checkmark$)
     & \\
  %-----------------------------------------------------------------------------------------
    & 
    &
    & $\sigma_{\text{tot}}(\bar{t})$
    & $19.7$
    & 1
    & \cite{Khachatryan:2014iya}
     & ($\checkmark$)
     & \\
   %-----------------------------------------------------------------------------------------
    & 
    & $s$-channel
    & $\sigma_{\text{tot}}(t + \bar{t})$
    & $19.7$
    & 1
    & \cite{Khachatryan:2016ewo}  
     & $\checkmark$
      & \\
      \midrule
   %-----------------------------------------------------------------------------------------
    & 13
    & $t$-channel
    & $\sigma_{\text{tot}}(t)$
    & $2.2$
    & 1
    & \cite{Sirunyan:2016cdg} 
        & ($\checkmark$)
     & \\
   %-----------------------------------------------------------------------------------------
    &
    & 
    & $\sigma_{\text{tot}}(\bar{t})$
    & $2.2$
    & 1
    & \cite{Sirunyan:2016cdg} 
      & ($\checkmark$)
     & \\
    %-----------------------------------------------------------------------------------------
    &
    & 
    & $1/\sigma d\sigma/d|y^{(t)}|$
    & $35.9$
    & 4
    & \cite{Sirunyan:2019hqb}
     & $\checkmark$
     & \\
\bottomrule
   \end{tabular}
   \vspace{0.3cm}
  \caption{\small Same as Table~\ref{tab:input_datasets_toppair} for
    the inclusive single-top production datasets.
     \label{tab:input_datasets_3}
   }
}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{table}[htbp]
%\begin{table}[h!]
%  \centering
%  \scriptsize
%    \renewcommand{\arraystretch}{1.0}
%   \setlength{\tabcolsep}{1.0pt}
%  \begin{tabular}{l|c|c|c|c|c|c}
%	  Dataset   &  $\sqrt{s}, \mathcal{L}$ & Info  &  Observables  & $N_{\rm dat}$ & Ref & Comment  \\
%\toprule
%    {\tt CMS\_t\_tch\_8TeV\_inc}  \\ ({\color{orange} APPLgrids available!})
%    & {\bf 8 TeV, 19.7~{\rm \bf fb}$^{-1}$ }
%    & $t$-channel
%    & $\sigma_{\rm tot}(t),\sigma_{\rm tot}(\bar{t})$  & 2
%    & \cite{Khachatryan:2014iya}  
%    & $\ast$ $\star$\\
%%----------------------------------------------------------------------------
%\midrule
%    {\tt CMS\_t\_tch\_8TeV\_dif}
%    & {\bf 8 TeV, 19.7~{\rm \bf fb}$^{-1}$}
%    & $t$-channel
%    & $1/ \sigma d\sigma/d|y^{(t+\bar{t})}|$
%    & 6
%    & \cite{CMS-PAS-TOP-14-004}  
%    & $\ast$ $\star$\\ 
%%--------------------------------------------------------------------------
%\midrule
%    {\tt ATLAS\_t\_tch\_8TeV} \\ ({\color{orange} APPLgrids available!})
%    & {\bf 8 TeV, 20.2~{\rm \bf fb}$^{-1}$}
%    & $t$-channel
%	  & $d\sigma(tq)/dy_{t}$, $d\sigma(\bar{t}q)/dy_{\bar{t}}$
%    & 5+5
%    & \cite{Aaboud:2017pdi}
%    & $\ast$\\
%%-----------------------------------------------------------------------------
%\midrule
%\midrule
%    {\tt CMS\_t\_sch\_8TeV}
%    & {\bf 8 TeV, 19.7~{\rm \bf fb}$^{-1}$}
%    & $s$-channel
%    & $\sigma_{\rm tot}(t+\bar{t})$
%    & 1
%    & \cite{Khachatryan:2016ewo}  
%    & $\ast$ $\star$\\ 
%%------------------------------------------------------------------------------
%\midrule
%    {\tt ATLAS\_t\_sch\_8TeV}
%    & {\bf 8 TeV, 20.3~{\rm \bf fb}$^{-1}$ }
%    & $s$-channel
%    & $\sigma_{\rm tot}(t+\bar{t})$
%    & 1
%    & \cite{Aad:2015upn}  
%    & $\ast$ $\star$ \\ 
%%------------------------------------------------------------------------------
%\midrule
%\midrule
%    {\tt ATLAS\_t\_tch\_13TeV} \\ ({\color{orange} APPLgrids available!})
%    & {\bf 13 TeV, 3.2~{\rm \bf fb}$^{-1}$}
%    & $t$-channel
%    & $\sigma_{\rm tot}(t),\sigma_{\rm tot}(\bar{t})$
%    & 2
%    & \cite{Aaboud:2016ymp}  
%    & $\star$ \\ 
%%------------------------------------------------------------------------------
%    \midrule
%    {\tt CMS\_t\_tch\_13TeV\_inc} \\ ({\color{orange} APPLgrids available!})
%    & {\bf 13 TeV, 2.2~{\rm \bf fb}$^{-1}$}
%    & $t$-channel
%    & $\sigma_{\rm tot}(t),\sigma_{\rm tot}(\bar{t})$
%    & 2
%    & \cite{Sirunyan:2016cdg}  
%     & $\ast$ $\star$\\ 
%%------------------------------------------------------------------------------
%    \midrule
%    {\tt CMS\_t\_tch\_13TeV\_2016} 
%    & {\bf 13 TeV, 35.9~{\rm \bf fb}$^{-1}$}
%    & $t$-channel
%    & $1/\sigma d\sigma/d|y^{(t)}|$
%    & 4
%    & \cite{Sirunyan:2019hqb}  
%     &$\ast$ $\star$ \\ 
%%------------------------------------------------------------------------------
%\bottomrule
%  \end{tabular}
%  \caption{Same as Table~\ref{tab:input_datasets_toppair} for inclusive single top production.
%     \label{tab:input_datasets3}
%  }
%\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Chapters/appendices/top/tables/table-input-dataset-top4.tex <==
\begin{table}[h!]
  \begin{center}
{\fontsize{8pt}{8pt}\selectfont
%\begin{table}[t]
  \centering
   \renewcommand{\arraystretch}{2}
   \setlength{\tabcolsep}{5pt}
   \begin{tabular}{lcccccc|c}
     \toprule \textbf{Experiment}     & $\bf{\sqrt{s}}$\textbf{(TeV)}
     &   \textbf{Channel} & \textbf{Observable} & $\mathcal{L}$ (fb${}^{-1}$) & $\mathbf{n_{\rm dat}}$ & \textbf{Ref.}   
     &  \textbf{New (SMEFT fits)} \\
    \toprule
      {\bf ATLAS}
      & 8
      & dilepton
      & $\sigma_{\text{tot}}(tW)$
      & $20.3$
      & 1
      & \cite{Aad:2015eto}
      & \\
%-------------------------------------------------------------------------------
      & 
      & single-lepton
      & $\sigma_{\text{tot}}(tW)$
      & $20.2$
      & 1
      & \cite{Aad:2020zhd}
      & \\
      \midrule
%-------------------------------------------------------------------------------
      & 13
      & dilepton
      & $\sigma_{\text{tot}}(tW)$
      & $3.2$
      & 1
      & \cite{Aaboud:2016lpj}
     &  \\
     % -------------------------------------------------------------------------------
      & 
      & dilepton
      & $\sigma_{\text{fid}}(tZj)$
      & $139$
      & 1
      & \cite{Aad:2020wog}
      & \\
     \midrule
      {\bf CMS}
      & 8
      & dilepton
      & $\sigma_{\text{tot}}(tW)$
      & $12.2$
      & 1
      & \cite{Chatrchyan:2014tua}
      &   \\
      \midrule
%-------------------------------------------------------------------------------
      & 13
      & dilepton
      & $\sigma_{\text{tot}}(tW)$
      & $35.9$
      & 1
      & \cite{Sirunyan:2018lcp}
      & \\
 %-------------------------------------------------------------------------------
      & 
      & dilepton
      & $\sigma_{\text{fid}}(tZj)$
      & $77.4$
      & 1
      & \cite{Sirunyan:2018zgs}
     & \\
 %-------------------------------------------------------------------------------
      &
      & dilepton
      & $d\sigma_{\text{fid}}(tZj)/dp_T^t$
      & $138$
      & 3
      & \cite{CMS:2021rvz}
      & $\checkmark$\\
%-------------------------------------------------------------------------------
      & 
      & single-lepton
      & $\sigma_{\text{tot}}(tW)$
      & $36$
      & 1
      & \cite{CMS:2021vqm}
      & $\checkmark$\\
\bottomrule
   \end{tabular}
   \vspace{0.3cm}
  \caption{\small Same as Table~\ref{tab:input_datasets_toppair} for
    single-top production in association with an electroweak bosons.
}
   \label{tab:input_datasets_4}
}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Chapters/appendices/top/tables/table-input-dataset-top4b.tex <==
\begin{table}[h!]
{\fontsize{7pt}{7pt}\selectfont
%\begin{table}[t]
  \centering
   \renewcommand{\arraystretch}{2}
   \setlength{\tabcolsep}{5pt}
   \begin{tabular}{lcccc|c}
     \toprule \textbf{Experiment}     & $\bf{\sqrt{s}}$\textbf{(TeV)}
     &  \textbf{Observable} & $\mathbf{n_{\rm dat}}$ & \textbf{Ref.}   
    &  \textbf{New (SMEFT fits)} \\
    \toprule
      ATLAS
      & 13
      & $\sigma_{\text{fid}}(tl^+l^-q)$
      & 1
      & \cite{Aad:2020wog}
      & \\
%-------------------------------------------------------------------------------
     \midrule
      CMS
      & 13
      & $\sigma_{\text{fid}}(tl^+l^-q)$
      & 1
      & \cite{Sirunyan:2018zgs}
      & \\
%-------------------------------------------------------------------------------
      & 
      & $d\sigma_{\text{fid}}(tZq)/dp_T(Z)$ or $d\sigma_{\text{fid}}(tZq)/dp_T(t)$
      & 4 or 3
      & \cite{CMS:2021rvz}
      & $\checkmark$\\
\bottomrule
  \end{tabular}
  \caption{\small Same as Table~\ref{tab:input_datasets_toppair} for all the single-top production in association with a $Z$-boson included in this analysis.
     \label{tab:input_datasets_4b}
}
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Samples/clean/01Preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Some custom packages
%%
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{xspace}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Fonts (like different typewriter fonts etc.)
%%
%\RequirePackage[scaled=.87]{couriers}
%\RequirePackage[T1]{fontenc}
%\renewcommand\rmdefault{psb}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Style (Changing the visual style of chapter headings and stuff.)
%%
\RequirePackage{titlesec}
% [Fixes issue #34 (see https://github.com/cambridge/thesis/issues/34). Solution from: http://tex.stackexchange.com/questions/299969/titlesec-loss-of-section-numbering-with-the-new-update-2016-03-15
\RequirePackage{etoolbox}
\makeatletter
\patchcmd{\ttlh@hang}{\parindent\z@}{\parindent\z@\leavevmode}{}{}
\patchcmd{\ttlh@hang}{\noindent}{}{}{}
\makeatother
% end of issue #34 fix]
\newcommand{\PreContentTitleFormat}{\titleformat{\chapter}[display]{\scshape\Large}
{\Large\filleft\MakeUppercase{\chaptertitlename} \Huge\thechapter}
{1ex}
{}
[\vspace{1ex}\titlerule]}
\newcommand{\ContentTitleFormat}{\titleformat{\chapter}[display]{\scshape\huge}
{\Large\filleft\MakeUppercase{\chaptertitlename} \Huge\thechapter}
{1ex}
{\titlerule\vspace{1ex}\filright}
[\vspace{1ex}\titlerule]}
\newcommand{\PostContentTitleFormat}{\PreContentTitleFormat}
\PreContentTitleFormat




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% References (special style etc.)
%%
\RequirePackage[numbers,sort&compress]{natbib}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Theorems, definitions, and examples
%%
\RequirePackage{amsthm}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[chapter]
%% Support for `Examples` (provides a counter for examples, the possibility to
%% label and reference them etc.)
%%
\newtheorem{example}{Example}[chapter]




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Captions: This makes captions of figures use a boldfaced small font. 
%%
\RequirePackage[small,bf]{caption}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Subfigure (note: this must be included after the `caption` package). 
%%
\RequirePackage{subfig}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Graphics (we set the central folder for all included graphics to
%% `./Figures/`)
%%
\graphicspath{{./Figures/}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Content commands
%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Glossary entries
%%
\newglossaryentry{pi}{
    name={\ensuremath{\pi}},
    sort={pi},
    description={ratio of the circumference of a circle to the diameter}
}


==> Samples/clean/02ThesisInfo.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Thesis Meta-Information
%%

%% The title of the thesis:
\title{My thesis title\\
spanning two lines}

%% The full name of the author (e.g.: James Smith):
\author{My Full Name}

%% College affiliation:
\college{My College}

%% College shield (optional):
% \collegeshield{CollegeShields/Clare}
% \collegeshield{CollegeShields/Fitzwilliam}
% \collegeshield{CollegeShields/FitzwilliamRed}
% \collegeshield{CollegeShields/StJohns}
% \collegeshield{CollegeShields/Trinity}
\collegeshield{CollegeShields/Queens}

%% Submission date (optional):
\submissiondate{November, 2042}

%% You can redefine the submission notice:
% \submissionnotice{A badass thesis submitted on time for the Degree of PhD}

%% Declaration date:
\date{Month, Year}

%% PDF meta-info:
\subjectline{Computer Science}
\keywords{one two three}


==> Samples/clean/03Abstract.tex <==
\abstract{%
  My abstract ...
}

==> Samples/clean/04Acknowledgments.tex <==
\acknowledgements{%
  My acknowledgements ...
}

==> Samples/clean/15ResultsEvaluation.tex <==
\chapter{Results and evaluation}


==> Samples/clean/16RelatedWork.tex <==
\chapter{Related work}


==> Samples/clean/17FutureWork.tex <==
\chapter{Future work}


==> Samples/clean/18Conclusion.tex <==
\chapter{Conclusion}


==> Samples/clean/22Index.tex <==
\cleardoublepage
\phantomsection
\addcontentsline{toc}{chapter}{Index}
\printindex
